Approximation Algorithms for ROUND-UFP and ROUND-SAP

We study ROUND-UFP and ROUND-SAP, two generalizations of the classical BIN PACKING problem that correspond to the unsplittable flow problem on a path (UFP) and the storage allocation problem (SAP), respectively. We are given a path with capacities on its edges and a set of tasks where for each task we are given a demand and a subpath. In ROUND-UFP, the goal is to find a packing of all tasks into a minimum number of copies (rounds) of the given path such that for each copy, the total demand of tasks on any edge does not exceed the capacity of the respective edge. In ROUND-SAP, the tasks are considered to be rectangles and the goal is to find a non-overlapping packing of these rectangles into a minimum number of rounds such that all rectangles lie completely below the capacity profile of the edges. We show that in contrast to BIN PACKING, both the problems do not admit an asymptotic polynomial-time approximation scheme (APTAS), even when all edge capacities are equal. However, for this setting, we obtain asymptotic $(2+\varepsilon)$-approximations for both problems. For the general case, we obtain an $O(\log\log n)$-approximation algorithm and an $O(\log\log\frac{1}{\delta})$-approximation under $(1+\delta)$-resource augmentation for both problems. For the intermediate setting of the no bottleneck assumption (i.e., the maximum task demand is at most the minimum edge capacity), we obtain absolute $12$- and asymptotic $(16+\varepsilon)$-approximation algorithms for ROUND-UFP and ROUND-SAP, respectively.

==> Arxiv submission/NBA.tex <==
\section{Algorithms for the no-bottleneck-assumption}
\label{sec:roundsapandufpwithnba}

In this section, we present a $(16+\eps)$-approximation algorithm
for \rsap\  and a $12$-approximation
 for \rufp, both under the no-bottleneck-assumption (NBA).  

\subsection{Algorithm for \rsap}

For our algorithm for \rsap\ under NBA, we first
scale down all job demands and edge capacities so that $c_{\min}:=\min_{e\in E}c_{e}=1$.
Since the NBA holds, this implies that $d_{\js}\le1$ for each job
$\js\in J$. Then, we scale down all edge capacities to the nearest
power of 2, i.e., for each edge $e\in E$ we define a new rounded
capacity $c'_{e}:=2^{\left\lfloor \log c_{e}\right\rfloor }$. We
introduce horizontal lines whose $y$-coordinates are integral powers
of 2 (in contrast to the lines with uniform spacing that we used in Section~\ref{sec:Uniform_capacity}). Formally,
we define a set of lines $\mathcal{L}:=\{\ell_{2^k}|k\in\mathbb{N}\}$.
Let $OPT'_{SAP}$ denote the optimal solution for the rounded down capacities
$(c'_{e})_{e\in E}$ under the additional constraint that there must be no job
whose rectangle intersects a line in $\mathcal{L}$. 

%We show that rounding the edge capacities and the latter constraint lose at most a factor of 4 in our approximation ratio.

We now show that given a valid \rsap\ packing $\Ps$ of a set of jobs $J'$ for the
edge capacities $(c_{e})_{e\in E}$, there exists a valid packing
of $J'$ into 4 rounds $\Rs^{1},\Rs^{2},\Rs^{3},\Rs^{4},$ under profile
$(c'_{e})_{e\in E}$ such that no job is sliced by a line in $\mathcal{L}$ (see \Cref{closedcor2_newnew} in \Cref{sec:figforrsap}). Let $J^{(i)}$ be the set of jobs with bottleneck capacity in  $[2^i,2^{i+1})$. For $i\ge 1$, we pack $J^{(i)}$ as follows:
\begin{enumerate}
\item Place each job $\js$ lying completely below $\ell_{2^{i}}$ into
$\Rs^{1}$ at height $h'_{\js}:=h_{\js}$.
(Note that here $h_{\js}$ denotes the height of the bottom edge
of $\js$ in $\Ps$.) 
\item Place each job $\js$ lying completely between $\ell_{2^{i}}$ and
$\ell_{3\cdot2^{i-1}}$ into $\Rs^{2}$ with $h'_{\js}:=h_{\js}-2^{i-1}$. 
\item Place each job $\js$ lying completely between $\ell_{3\cdot2^{i-1}}$
and $\ell_{2^{i+1}}$ into $\Rs^{3}$ with $h'_{\js}:=h_{\js}-2^{i}$. 
\item Place each job $\js$ sliced by $\ell_{2^{i}}$ into $\Rs^{4}$ with
$h'_{\js}:=2^{i}-d_{\js}$; and place each job $\js$ sliced by $\ell_{3\cdot2^{i-1}}$ into $\Rs^{4}$
with $h'_{\js}:=3\cdot2^{i-2}-d_{\js}$ for $i\ge2$ and $h'_{\js}:=1-d_{\js}$
for $i=1$.
\end{enumerate}
\noindent Finally, we pack $J^{(0)}$ as follows:
\begin{enumerate}
\item Place each job $\js$ lying completely below $\ell_{1}$ into $\Rs^{1}$
with $h'_{\js}:=h_{\js}$. 
\item Place each job $\js$ lying completely between $\ell_{1}$ and $\ell_{2}$
into $\Rs^{2}$ with $h'_{\js}:=h_{\js}-1$. 
\item Place each job $\js$ sliced by $\ell_{1}$ into $\Rs^{3}$ with $h'_{\js}:=1-d_{\js}$. 
\end{enumerate}
It can be checked easily that the above algorithm yields a feasible packing of $J'$ in which no job is sliced by a line in $\mathcal{L}$. Thus by losing at most a factor of 4 in our approximation ratio, we can convert any valid \rsap\ packing to a packing under the profile $(c'_{e})_{e\in E}$ that satisfies the latter constraint as well.

\begin{lemma} \label{lemma:factor4} We have that $OPT'_{SAP}\le4\cdot OPT_{SAP}$
\end{lemma} 

\iffalse
\begin{proof}
Given a valid \rsap\ packing $\Ps$ of a set of jobs $T$ for the
given edge capacities $(c_{e})_{e\in E}$, we construct a valid packing
of $T$ into 4 rounds $\Rs^{1},\Rs^{2},\Rs^{3},\Rs^{4},$ under profile
$(c'_{e})_{e\in E}$ such that no job is sliced by $\mathcal{L}$.
Let $T^{(i)}:=\{\js\in T\mid2^{i}\le\mathfrak{b}_{\js}<2^{i+1}\}$,
$\forall i\in\{0,1,\ldots,\lfloor\log c_{\max}\rfloor\}$. Note that
jobs in $T^{(i)}$ will have bottleneck capacity equal to $2^{i}$ in
$(c'_{e})_{e\in E}$. For $i\in\{1,\ldots,\lfloor\log c_{\max}\rfloor\}$,
we pack $T^{(i)}$ as follows: 
\begin{itemize}
\item Place each job $\js$ lying completely below $\ell_{2^{i}}$ into
$\Rs^{1}$ at height $h'_{\js}:=h_{\js}$.
(Note that here $h_{\js}$ denotes the height of the bottom edge
of $\js$ in $\Ps$.) 
\item Place each job $\js$ lying completely between $\ell_{2^{i}}$ and
$\ell_{3\cdot2^{i-1}}$ into $\Rs^{2}$ with $h'_{\js}:=h_{\js}-2^{i-1}$. 
\item Place each job $\js$ lying completely between $\ell_{3\cdot2^{i-1}}$
and $\ell_{2^{i+1}}$ into $\Rs^{3}$ with $h'_{\js}:=h_{\js}-2^{i}$. 
\item Place each job $\js$ sliced by $\ell_{2^{i}}$ into $\Rs^{4}$ with
$h'_{\js}:=2^{i}-d_{\js}$. 
\item Place each job $\js$ sliced by $\ell_{3\cdot2^{i-1}}$ into $\Rs^{4}$
with $h'_{\js}:=3\cdot2^{i-2}-d_{\js}$ for $i\ge2$ and $h'_{\js}:=1-d_{\js}$
for $i=1$. 
\end{itemize}
Note that the jobs allocated to $\Rs^{1}$ are placed at the same
vertical height as in $\Ps$. For $\Rs^{2}$, we have maintained the
invariant that all jobs placed between $\ell_{2^{i-1}}$ and $\ell_{2^{i}}$
lied completely between $\ell_{2^{i}}$ and $\ell_{3.2^{i-1}}$ and
had bottleneck capacity in the interval $[2^{i},2^{i+1})$ in $\Ps$.
Similarly for $\Rs_{3}$, jobs placed between $\ell_{2^{i-1}}$ and
$\ell_{2^{i}}$ lied completely between $\ell_{3.2^{i-1}}$ and $\ell_{2^{i+1}}$
and had bottleneck capacity in the interval $[2^{i},2^{i+1})$ in
$\Ps$. Observe that the region below $\ell_{1}$ is currently empty
in both $\Rs^{2}$ and $\Rs^{3}$ (this will be utilized for packing
jobs in $T_{0}$). Finally, $\Rs^{4}$ contains the jobs sliced by
$\ell_{2^{i}}$ and $\ell_{3\cdot2^{i-1}}$.

As we have ensured that jobs from $T^{(i)}$ have been placed only in
the region between the slicing lines $\ell_{2^{i-1}}$ and $\ell_{2^{i}}$
in $\Rs^{2}$ and $\Rs^{3}$, there is no overlap between jobs from
different $T^{(i)}$'s in $\Rs^{2}$ and $\Rs^{3}$. Also since the
demand of each job is at most 1, there is no overlapping of jobs from
different $T^{(i)}$'s inside $\Rs^{4}$. Now we pack the jobs in $T_{0}$
(jobs with bottleneck capacity less than 2), as follows: 
\begin{itemize}
\item Place each job $\js$ lying completely below $\ell_{1}$ into $\Rs^{1}$
with $h'_{\js}:=h_{\js}$. 
\item Place each job $\js$ lying completely between $\ell_{1}$ and $\ell_{2}$
into $\Rs^{2}$ with $h'_{\js}:=h_{\js}-1$. 
\item Place each job $\js$ sliced by $\ell_{1}$ into $\Rs^{3}$ with $h'_{\js}:=1-d_{\js}$. 
\end{itemize}
We continue to maintain the same invariant for $\Rs^{1}$. For $\Rs^{2}$
and $\Rs^{3}$, we used the empty region below $\ell_{1}$ to pack
jobs from $T^{(0)}$. Note that no job is sliced by $\Ls$ in the packing
obtained. Hence the lemma holds. 
\end{proof}
\fi


\iffalse 
\begin{figure}
\centering \captionsetup{justification=centering} \begin{tikzpicture}
\node[inner sep=0pt] (figc) at (0,0)
    {\includegraphics[width=.33\textwidth]{figc.png}};
    
\node[inner sep=0pt] (figd) at (4.6,0)
    {\includegraphics[width=.33\textwidth]{figd.png}}; 
    
\node[inner sep=0pt] (fige) at (9.2,0)
    {\includegraphics[width=.33\textwidth]{fige.png}};      
    
\node[inner sep=0pt] (figa) at (1.1,3.695)
    {\includegraphics[width=.33\textwidth]{figa.png}};     
    
\node[inner sep=0pt] (figb) at (7.1,3)
    {\includegraphics[width=.33\textwidth]{figb.png}}; 

\draw[thick, color = yellow, pattern=north east lines, pattern color = yellow] (9.4,5.2) rectangle (9.9,5.4);
\draw[thick] (10.6,5.3) node {\tiny Jobs in $T_0$};
   
\draw[thick, color = green, pattern=north east lines, pattern color = green] (9.4,4.9) rectangle (9.9,5.1);
\draw[thick] (10.6,5) node {\tiny Jobs in $T_1$};

\draw[thick, color = pink, pattern=north east lines, pattern color = pink] (9.4,4.6) rectangle (9.9,4.8);
\draw[thick] (10.6,4.7) node {\tiny Jobs in $T_2$};    
    
\draw[thick] (7.1,1.8) node {\scriptsize \textbf{(b)} Round $\Rs^1$};
\draw[thick] (1.1,1.8) node {\scriptsize \textbf{(a)} Packing $\Ps$};
%\draw[thick] (1.2,1.2) node {\scriptsize represent the demands)};       

%\draw[thick] (0,-0.75) node {\scriptsize \textbf{(i)}};
%\draw[thick] (4.5,-0.75) node {\scriptsize \textbf{(ii)}};
\draw[thick] (0,-1.1) node {\scriptsize \textbf{(c)} Round $\Rs^2$};
\draw[thick] (4.6,-1.1) node {\scriptsize \textbf{(d)} Round $\Rs^3$};
\draw[thick] (9.2,-1.1) node {\scriptsize \textbf{(e)} Round $\Rs^4$};
%\draw[thick] (9,-1.1) node {\scriptsize using only 1 round};
\end{tikzpicture} \caption{Figure for \Cref{lemma:factor4}}
\label{fig:lemma9} 
\end{figure}

\fi



We shall now obtain a valid packing of $J$ for the edge capacities
$(c'_{e})_{e\in E}$. Let $c'_{\max}:=\max_{e\in E}c'_{e}$ and for
each $i\in\{0,1,\ldots,\log c'_{\max}\}$ let $J^{(i)}\subseteq J$
denote the set of jobs with bottleneck capacity $2^{i}$ according
to $(c'_{e})_{e\in E}$. For each set $J^{(i)}$ we create a new (artificial)
instance with uniform edge capacities: in the instance for $J^{(0)}$
all edges have capacity 1, and for each $i\in\{1,2,\ldots,\log c'_{\max}\}$
in the instance for $J^{(i)}$ all edges have capacity $2^{i-1}$. For
each $i\in\{0,1,2,\ldots,\log c'_{\max}\}$ denote by $OPT^{(i)}$ the
number of rounds needed in the optimal solution to the instance for
$J^{(i)}$. Since in the solution $OPT'_{SAP}$ no rectangle is intersected
by a line in $\mathcal{L}$, for each set $J^{(i)}$ we can easily rearrange
the jobs in $J^{(i)}$ in $OPT'_{SAP}$ such that we obtain a solution
for $J^{(i)}$ with at most $2\cdot OPT'_{SAP}$ rounds.

\begin{lemma} \label{lemma:factor2loss} For each $i\in\{0,1,2,\ldots,\log c'_{\max}\}$
it holds that $OPT^{(i)}\le2\cdot OPT'_{SAP}$. \end{lemma}

For each set $J^{(i)}$ we invoke our asymptotic $(2+\eps)$-approximation
algorithm for \rsap\ for uniform edge capacities (see Section~\ref{sec:Uniform_capacity})
and obtain a solution $\Gamma^{(i)}$ which hence uses $\Gamma^{(i)}\le (2+\eps)\cdot OPT^{(i)}+O(1)\le (2+\eps)\cdot OPT'_{SAP}+O(1)$
rounds. Finally, we combine the solutions $\Gamma^{(i)}$ for all $i\in\{0,1,2,\ldots,\log c'_{\max}\}$
to one global solution of $J$. The key insight for this is that if
some edge $e$ has a (rounded) capacity of $c'_{e}=2^{k}$, then in
one round we can place the solution of one round of each of the solutions
$\Gamma^{(0)},\Gamma^{(1)},...,\Gamma^{(k-1)}$. 
\begin{lemma}
\label{lemma:mainpackinglemma}Given a solution $\Gamma^{(i)}$ for
the set $J^{(i)}$ for each $i\in\{0,1,2,\ldots,\log c'_{\max}\}$, in polynomial time we can construct a solution for $J$ and the edge
capacities $(c'_{e})_{e\in E}$ with at most $\max^{(i)}\{\Gamma^{(i)}\}$
many rounds.
\end{lemma}

\iffalse
\begin{algorithm}
Apply \Cref{theorem:twoasymptoticapprox} to obtain a solution to $J^{(0)}$, assuming all edges have capacity 1,

Apply \Cref{theorem:twoasymptoticapprox} to obtain a solution to $J^{(i)}$ for each $i\in\{1,2,\ldots,\log c'_{\max}\}$, assuming that
all edges have capacity $2^{i-1}$,

Use \Cref{lemma:mainpackinglemma} to combine the packings and obtain
a valid packing of $J$ for the profile $(c'_{e})_{e\in E}$. \caption{}
\label{algo:UniformRoundSap1arbitrary}
\end{algorithm}
\fi

Using the asymptotic $(2+\eps)$- (resp. absolute 3-) approximation for \rsap under uniform edge capacities (from Theorems \ref{theorem:twoasymptoticapprox} and \ref{thm:unisapabs}),  this yields the following theorem.
%an asymptotic $(16+\eps)$- (resp. abs. 24-) approximation  for \rsap\ under the~NBA.

\begin{theorem} \label{theorem:16approxroundsap} For any $\eps>0$,
there exists an asymptotic $(16+\eps)$-approximation and an absolute 24-approximation algorithm for
\rsap under the NBA. \end{theorem}
%\arir{added 24-approx.}

\subsection{Algorithm for \rufp}

\label{sec:generalroundufp} In this section, we present a 12-approximation
for \rufp\ under NBA. In \rufp, it is not clear how to bootstrap
the algorithm for the uniform case as we did for \rsap, since in
the optimal solution it might not be possible to draw the jobs as non-overlapping
rectangles. Instead, our algorithm refines combinatorial properties
from \cite{ElbassioniGGKN12} to obtain an improved approximation
ratio. We will use the following algorithm due to~\cite{NomikosPZ01}
as a subroutine. 
\begin{theorem}[\cite{NomikosPZ01}]
\label{theorem:nomikostheorem}Given an instance of \rufp\ in which
all job demands are equal to 1 and all edge capacities are integral.
Then $OPT_{UFP}=r$ and in polynomial time we can compute a packing
into $OPT_{UFP}$ many rounds.
\end{theorem}

\noindent Via scaling, we assume that $c_{\min}=1$ and the demand of each
job is at most 1. Let $J_{\mathrm{large}}:=\{\js\in J\mid d_{\js}>1/2\}$
and  $J_{\mathrm{small}}:=J\setminus J_{\mathrm{large}}$. For
each job $\js\in J_{\mathrm{small}}$ we round up its demand to the
next larger power of $1/2$, i.e., we define its rounded demand $d'_{\js}:=2^{\left\lceil \log d_{\js}\right\rceil }$.
For each $i\in\mathbb{N}$, let $J^{(i)}$ denote the set of jobs whose
demands after rounding equal $\frac{1}{2^{i}}$, i.e., $J^{(i)}=\{\js\in J|d'_{\js}=\frac{1}{2^{i}}\}$.
For each edge $e$ and each $i\in\mathbb{N}$, we count how many jobs
in $J^{(i)}$ use $e$ and we define $n_{e,i}:=|\{\js\in J^{(i)}\mid e\in P_{\js}\}|$.
We partition each set $J^{(i)}$ into the sets $J'^{(i)}=\{\js\in J^{(i)}\mid\exists e\in P_{\js}:n_{e,i}<2r\}$
and $J''^{(i)}=J\setminus J'^{(i)}$. Let $n'_{e,i}:=|\{\js\in J'^{(i)}\mid e\in P_{\js}\}|$
and $n''_{e,i}:=|\{\js\in J''^{(i)}\mid e\in P_{\js}\}|$. Clearly, $n'_{e,i}<4r$ for each edge $e$ and each $i$.

First, we compute a packing for $J_{\mathrm{small}}$. For the (small)
jobs in the sets $J'^{(i)}$, we use a packing method that ensures
that inside each round we have at most one job from each set $J'^{(i)}$. 
Since $n'_{e,i}<4r$ for each edge $e$ and each $i$, this needs at most $4r$ rounds.  
Moreover, by a geometric sum argument this yields a valid packing inside each round (the job demands sum up to at most $1=c_{\min}$). For the
jobs in $J''^{(i)}$, we partition the available capacity inside each
round among the sets $J''^{(i)}$ and then invoke the algorithm due to
Theorem~\ref{theorem:nomikostheorem} for each set $J''^{(i)}$ separately, which also needs at most $4r$ rounds, and thus at most $8r$ rounds in total.

\begin{lemma} For the jobs in $J_{\mathrm{small}}$ we can find a packing into at most $8r$ rounds. \end{lemma} 
\begin{proof}
For packing jobs in $\bigcup_{i}J'^{(i)}$, we introduce a set
$\Ts$ of $4r$ rounds. For each $i$, we consider the jobs in $J'^{(i)}$
in non-decreasing order of their left endpoints and assign a job to
the first round in $\Ts$ where it does not overlap with any job from
$J'^{(i)}$ that have been assigned till now. Since $n'_{e,i}\le4r$,
such an assignment is always possible. Thus over any edge $e$ inside
any round of $\Ts$, at most 1 job from each set $J^{(i)}$ can be present.
Thus the load on edge $e$ is at most $\sum\limits_{i}\frac{1}{2^{i}}\le1\le c_{e}$, 
and hence this is a valid packing.

For packing the jobs in $\bigcup_{i}J''^{(i)}$, we introduce
a set $\Ss$ of $4r$ rounds. Consider a set $J''^{(i)}$. Inside each
of these rounds, to each edge $e$ we assign a capacity of $\frac{1}{2^{i}}\cdot\lfloor\frac{n_{e,i}}{2r}\rfloor$
to $J''^{(i)}$. The resulting congestion of any edge having non-zero
capacity is $\frac{\frac{1}{2^{i}}n''_{e,i}}{\frac{1}{2^{i}}\lfloor\frac{n_{e,i}}{2r}\rfloor}\le\frac{\frac{n_{e,i}}{2r}}{\lfloor\frac{n_{e,i}}{2r}\rfloor}\cdot2r\le4r$.
Also since each job in $J''^{(i)}$ has demand equal to $\frac{1}{2^{i}}$,
the assigned capacity of each edge is an integral multiple of the
demand. Thus using \Cref{theorem:nomikostheorem}, jobs in $J''^{(i)}$
can be packed into at most $4r$ rounds with these capacities. When
we do this procedure for each set $J''^{(i)}$, we obtain that the total
load on each edge $e$ inside any round is at most $\sum\limits_{i}\frac{1}{2^{i}}\lfloor\frac{n_{e,i}}{2r}\rfloor\le\sum\limits_{i}\frac{1}{2^{i+1}}\frac{n_{e,i}}{r}\le\frac{1}{r}\sum\limits _{\js\colon e\in P_{j}}d_{j}\le c_{e}$.
Thus this is a valid packing.

Therefore, we pack all jobs in $J_{\mathrm{small}}$ into $8r$ rounds. 
\end{proof}
For the jobs in $J_{\mathrm{large}}$ we round up their demands to
1 and the edge capacities to the respective nearest integer. This increases the congestion $r$
by at most a factor of 4. Then we invoke Theorem~\ref{theorem:nomikostheorem}.

\begin{lemma} 
\label{lem:ufp4r}
The jobs in $J_{\mathrm{large}}$ can be packed into
$4r$ rounds. \end{lemma} 
%\arir{shifted proof to appendix}
%
Overall, this yields a 12-approximation algorithm for \rufp\ under
the NBA.

\begin{theorem} \label{theorem:16approxroundufp-1}There is a polynomial
time 12-approximation algorithm for \rufp\ under the NBA. \end{theorem}

\begin{comment}
---------------------------------------

Now we state a crucial lemma, which enables us to improve the approximation
ratio. Intuitively, it does the following: suppose that we are given
some jobs whose demands are all in the range $[\frac{1}{\eta_{1}}c_{\min},\frac{1}{\eta_{2}}c_{\min}]$.
We scale up the demand of each job to $\frac{1}{\eta_{2}}c_{\min}$
and we scale down the capacity of each edge to the nearest integral
multiple of $\frac{1}{\eta_{2}}c_{\min}$. The resulting instance
is equivalent to an instance in which the edge capacities are integral
and all job demands are equal to 1. For such instances it is known
that the optimal number of needed rounds equals the congestion and
we can compute such a packing in polynomial time~\cite{NomikosPZ01}.
Some calculations show that this yields a packing with less than $\frac{\eta_{1}(\eta_{2}+1)}{\eta_{2}^{2}}r+1$
rounds in our setting.

\begin{lemma} \label{lemma:cruciallemma} Let $H:=\{\js\in J\mid\frac{1}{\eta_{1}}c_{\min}<d_{\js}\le\frac{1}{\eta_{2}}c_{\min}\}$,
for some $\eta_{1}>\eta_{2}\ge1$. Then there exists a valid \rufp\ packing
of $H$ using less than $\frac{\eta_{1}(\eta_{2}+1)}{\eta_{2}^{2}}r+1$
rounds. \end{lemma} 
\begin{proof}
Scale up the demand of each job in $H$ to $\frac{1}{\eta_{2}}c_{\min}$
and scale down the capacity of each edge in $E$ to the nearest integral
multiple of $\frac{1}{\eta_{2}}c_{\min}$. Let $H'$ denote the new
set of identical demand (of $\frac{1}{\eta_{2}}c_{\min}$) jobs and
let $I':=(c'_{e_{1}},c'_{e_{2}},\ldots,c'_{e_{m}})$ denote the new
profile. For $e\in E$, let $l_{e}^{H}$ and $r_{e}^{H}$ denote the
original load and congestion of edge $e$ due to the jobs in $H$
and let $l_{e}^{H'}$ and $r_{e}^{H'}$ denote the new load and congestion,
respectively. Then $l_{e}^{H'}<\frac{\eta_{1}}{\eta_{2}}l_{e}^{H}$
and $c'_{e}\ge\frac{\eta_{2}}{\eta_{2}+1}c_{e}$. Thus $r_{e}^{H'}=\Big\lceil\frac{l_{e}^{H'}}{c'_{e}}\Big\rceil\le\Big\lceil\frac{\frac{\eta_{1}}{\eta_{2}}l_{e}^{H}}{\frac{\eta_{2}}{\eta_{2}+1}c_{e}}\Big\rceil<\frac{\eta_{1}(\eta_{2}+1)}{\eta_{2}^{2}}\frac{l_{e}^{H}}{c_{e}}+1\le\frac{\eta_{1}(\eta_{2}+1)}{\eta_{2}^{2}}r_{e}^{H}+1$.

Finally, we scale all demands and edge capacities by $\frac{1}{\eta_{2}}c_{\min}$
so that now all jobs have unit demands and all capacities are integers.
Applying \Cref{theorem:nomikostheorem}, we obtain the number of
rounds required $:=\max\limits _{e}r_{e}^{H'}<\max\limits _{e}\frac{\eta_{1}(\eta_{2}+1)}{\eta_{2}^{2}}r_{e}^{H}+1\le\frac{\eta_{1}(\eta_{2}+1)}{\eta_{2}^{2}}r+1$. 
\end{proof}
Let $J_{\mathrm{large}}:=\{\js\in J\mid d_{\js}>\aw{c_{\min}}/9\}$
and let $J_{\mathrm{small}}:=J\setminus J_{\mathrm{large}}$. We compute
a packing for $J_{\mathrm{large}}$ with at most $10r$ rounds: we
partition it into jobs $\js$ with $d_{\js}\le\frac{1}{3}c_{\min}$
and jobs with $d_{\js}>\frac{1}{3}c_{\min}$ and apply \Cref{lemma:cruciallemma}
to each of them. 

\begin{lemma} \label{lemma:10approxforsmalljobs} The jobs in $J_{\mathrm{large}}$
can be packed into at most $10r$ rounds. \end{lemma} 
\begin{proof}
Let $Q_{\mathrm{medium}}:=\{\js\in J_{\mathrm{large}}\mid\frac{1}{9}c_{\min}<d_{\js}\le\frac{1}{3}c_{\min}\}$
and $Q_{\mathrm{large}}:=J_{\mathrm{large}}\setminus Q_{\mathrm{medium}}$.
Apply \Cref{lemma:cruciallemma} to $Q_{\mathrm{medium}}$ with
$\eta_{1}=9$ and $\eta_{2}=3$ and to $Q_{\mathrm{large}}$ with
$\eta_{1}=3$ and $\eta_{2}=1$. This gives packings of $Q_{\mathrm{medium}}$
and $Q_{\mathrm{large}}$ using less than $4r+1$ and $6r+1$ rounds,
respectively. Since the number of rounds must be an integer, at most
$4r$ and $6r$ rounds are used, respectively, which yields at most
$10r$ rounds in total. 
\end{proof}
\begin{lemma} \label{lemma:badjobs} The jobs in $J_{\mathrm{small}}$
can be packed into at most $6r$ rounds. \end{lemma} 
\begin{proof}
Our algorithm is similar to that of Elbassioni et al.~\cite{ElbassioniGGKN12}.
The \textit{class} of edge $e\in E$ is defined as cl$(e):=\lfloor\log c_{e}\rfloor$.
The \textit{critical edge} of a job $\js$, denoted by crit$(\js)$,
is the leftmost edge having the minimum class among all edges in $P_{\js}$.

We maintain $6r$ different rounds, $\Rs^{1},\Rs^{2},\ldots,\Rs^{6r}$.
We consider the jobs in $J_{\mathrm{small}}$ in non-decreasing order
of $s_{\js}$ and assign $\js$ to a round $\Rs$ such that the sum
of the demands of the jobs which have previously been assigned to
$\Rs$ and passes through crit$(\js)$ is at most $c_{\text{crit}(\js)}/6$.
Such a round must exist, otherwise $r_{\text{crit}(\js)}>\frac{6r\cdot({c_{\text{crit}(\js)}}/{6})}{c_{\text{crit}(\js)}}=r$,
a contradiction. Now we show that this produces a valid packing.

Consider any round $\Rs$ and any edge $e\in E$. Let $S_{e}^{\Rs}$
denote the set of jobs assigned to $\Rs$ that passes through $e$
and let $\js_{\text{left}}$ be the last job in $S_{e}^{\Rs}$ whose
critical edge is either $e$ or lies to the left of $e$. Note that
$\text{cl}(\text{crit}(\js_{\text{left}}))\le\text{cl}(e)$. Thus
all jobs in $S_{e}^{\Rs}$ allocated before $\js_{\text{left}}$ must
pass through $\text{crit}(\js_{\text{left}})$. Hence, the sum of
demands of all these jobs (excluding $\js_{\text{left}}$) is at most
$c_{\text{crit}(\js_{\text{left}})}/6$, otherwise we would not have
assigned $\js_{\text{left}}$ to $\Rs$. Thus the total sum of demands
of jobs in $S_{e}^{\Rs}$ whose critical edge is either $e$ or lies
to the left of $e$ is at most $\frac{c_{\text{crit}(\js_{\text{left}})}}{6}+\frac{c_{e}}{9}\le\frac{2^{\text{cl}(e)+1}}{6}+\frac{c_{e}}{9}\le\frac{c_{e}}{3}+\frac{c_{e}}{9}\le\frac{4}{9}c_{e}$.

Now consider the jobs whose critical edges lie to the right of $e$.
Let $\js$ be such a job, then clearly cl(crit$(\js))<\text{cl}(e)$.
Also if $\text{cl(crit}(\js))=i$, then $d_{\js}\le\mathfrak{b}_{\js}/9\le2^{i+1}/9$.
Thus the total sum of demands of all such jobs is at most $\sum_{i=0}^{\text{cl}(e)-1}\Big(\frac{2^{i+1}}{6}+\frac{2^{i+1}}{9}\Big)\le\frac{5}{18}\cdot2^{\text{cl}(e)+1}\le\frac{5}{9}c_{e}$.

Hence, the total sum of demands of all jobs in $S_{e}^{\Rs}$ is at
most $c_{e}$. 
\end{proof}
Combining \Cref{lemma:10approxforsmalljobs} and \Cref{lemma:badjobs},
we have the following theorem.

\begin{theorem} \label{theorem:16approxroundufp} \rufp\ admits
a polynomial time 16-approximation algorithm. \end{theorem}

A careful parameter optimization can improve the approximation ratio
of 16 to 15.696. It seems unlikely that more substantial improvements
are possible using the current techniques.
\end{comment}

\section{Algorithms for \rtree}
%\arir{added this section}
Extending the results for \rufp, using results on path coloring \cite{erlebach2001complexity}
and multicommodity demand flow \cite{ChekuriMS07}, we obtain the
following results for \rtree~(see App. \ref{sec:roundufpontree}).

\begin{theorem} \label{thm:rtreetheorem} For \rtree, there exists
a polynomial-time asymptotic (resp. absolute) 5.1- (resp. 5.5-) approximation algorithm for uniform edge capacities
and an asymptotic (resp. absolute) 49- (resp. 55-) approximation algorithm for the general case under the NBA. \end{theorem}

% See Appendix \ref{sec:roundufpontree} for the proof of Theorem \ref{thm:rtreetheorem}. 




==> Arxiv submission/constantdemand.tex <==
\section{Uniform Capacity and Constant Job Demands}
\label{sec:Constant_Job_Heights}
In this section, we prove Theorem \ref{theorem:APTASforconstant}.

\begin{theorem}
(Restatement of Theorem \ref{theorem:APTASforconstant})
There exist APTASes for \ursap\ and \urufp\ when the maximum demand $d_{\max}$ is constant.
\end{theorem}
%\arir{constant demand can be confused with same demand.}
%\arir{c is a poor notation as we already use it for capacity function as well.}
The proof is divided into two cases, depending on the value of $d_{\max}$.

\subsection{Case 1: $d_{\max}\ge \eps \cs$.}
\label{subsec:allconstant}
Intuitively, in this case $\cs$ is also a constant and thus we can use a dynamic program to find the optimal packing in polynomial-time. First, we consider \ursap. 
Consider a valid \ursap\ packing of a subset of $J$ inside one round of the uniform capacity profile of height $\cs$. We assume w.l.o.g.~that $h_{\js}$ is an integer, for all jobs $\js$ in the packing. This can be achieved by applying "gravity" to the packing, i.e., we consider the jobs in the non-decreasing order of $h_{\js}$'s and move them downwards till they touch the top of some other job or reach the $x$-axis. We define an encoding of the sequence of jobs present over any edge. The \textit{configuration} of edge $e$ is defined as an ordered $\cs$-tuple $(\zeta_1,\zeta_2,\dots,\zeta_{\cs})$. For all $i \in \{1,2,\ldots,\cs\}$, define $\zeta_i = 0$, if no job is present between the slicing lines $\ell_{i-1}$ and $\ell_i$ over $e$; and otherwise, define $\zeta_i = d_{\js}$, where $\js$ is the job present between $\ell_{i-1}$ and $\ell_i$. Thus each $\zeta_i$ can take $d_{\max}+1$ many values. Hence the number of possible configurations of an edge is $\nu := (d_{\max}+1)^{\cs} = O_{\eps}(1)$, since $d_{\max}$ is a constant and $\cs \le d_{\max}/\eps$.

Now consider any valid \ursap\ packing of $J$ using $\lambda$ rounds $\Rs^1, \Rs^2,\ldots,\Rs^\lambda$. The \textit{joint configuration} of an edge $e$ is defined as an \textbf{unordered} $\lambda$-tuple $(C^{e}_{1},C^{e}_{2},\ldots, C^{e}_{\lambda})$, where $C^{e}_i$ denotes the configuration of $e$ in round $\Rs^i$, $\forall i \in \{1,2,\dots,\lambda\}$. Since there are $\lambda$ rounds, such a joint configuration is said to be a $\lambda$-\textit{dimensional} joint configuration. Thus the number of possible $\lambda$-dimensional joint configurations of an edge is at most $\lambda^{\nu} = \lambda^{O_{\eps}(1)}$.

We define a procedure called \checkcomp\ (see \Cref{algo:Checkcompatibility}) that takes input a valid \ursap\ packing $\Ps$ of $J^{e_{i-1}}$ using $\lambda$ rounds and a $\lambda$-dimensional joint configuration $\Cs^{e_i}$, for some $i \in \{2, 3, \dots, m\}$. \checkcomp\  returns \textbf{false} if $\Ps$ and $\Cs^{e_i}$ cannot be feasibly packed together, otherwise, it returns the feasible packing. Let the $\lambda$ rounds in $\Ps$ be $\Rs^1$, $\Rs^2$,\ldots,$\Rs^\lambda$ and let $\Cs^{e_i} = (C^{e_i}_{1},C^{e_i}_{2},\ldots, C^{e_i}_{\lambda})$. 

\begin{algorithm}[H]
For each round $\Rs^j$, create a node $u_j$, and for each configuration $C^{e_i}_{k}$, create a node $v_k$, $1\le j,k \le \lambda$.\\
Add an edge between $u_j$ and $v_k$ if configuration $C^{e_i}_{k}$ can be feasibly placed with the packing inside the round $\Rs^j$, $\forall 1\le j,k \le \lambda$. Let $\Gs$ denote the resulting bipartite graph.\\   
%Create a bipartite graph $G=L\cup R$ where $L$ consists of the $k$ rounds in $\Ps$ and $R$ consists of the $k$ configurations in $C_e$.\\
%$\forall (l,r)\in L\cup R$, add an edge between $l$ and $r$ if configuration $r$ can be feasibly packed inside round $l$.\\
Compute the maximum matching $N$ in $\Gs$.\\
If $N$ is a perfect matching, return the packing corresponding to $N$, else return \textbf{false}.
\caption{\checkcomp$(\Ps,\Cs^{e_i})$}
\label{algo:Checkcompatibility}
\end{algorithm}

Equipped with the above procedure, we now propose a dynamic programming based algorithm. First, guess the value of $\opt_{URS}$ as $\kappa$ where $1\le \kappa \le n$. A DP cell consists of 
\begin{itemize}
\item an edge $e\in E$.
\item a $\kappa$-dimensional joint configuration $\Cs^e$ of $e$.
\end{itemize}

We define DP($e,\Cs^e$)=1 if and only if there exists a valid \ursap\ packing $\Ps$ of $J^e$ such that the joint configuration of $e$ in $\Ps$ is exactly $\Cs^e$. If DP($e,\Cs^e$)=1, we also store the corresponding packing $\Ps$ in another table $\Upsilon$ in the table entry $\Upsilon(e,\Cs^e)$. For all $i \in \{2,3,\ldots, m\}$,  the recurrence for the dynamic program is given by: DP($e_i,\Cs^{e_i}$)=1 if there exists a $\Cs^{e_{i-1}}$ such that DP($e_{i-1},\Cs^{e_{i-1}}$)=1 and \checkcomp$(\Upsilon(e_{i-1},\Cs^{e_{i-1}}),\Cs^{e_i})$ returns a valid packing; otherwise, DP($e_i,\Cs^{e_i}$)=0. Clearly, the number of DP cells is polynomially bounded and each DP entry can be computed in polynomial time. 

For \urufp\, the positions of jobs inside a round do not matter. Hence the configuration of an edge $e$ can simply be encoded as a $d_{\max}$-tuple $(\zeta_1,\zeta_2,\ldots,\zeta_{d_{\max}})$, where $\forall i \in \{1,2,\ldots, d_{\max}\}$, $\zeta_i$ denotes the number of jobs having demand $i$, present over $e$ inside a round of a valid packing. Clearly, each $\zeta_i \le \cs$ and therefore the number of possible edge configurations is bounded by ${\cs}^{d_{\max}} \le O_{\eps}(1)$. The definition of a joint configuration remains the same. Procedure \checkcomp\ and the dynamic program also stay the same. Thus we have the following theorem:

\begin{theorem}
\label{theorem:optimalsolnforrsap}
For any $\eps >0$, if $d_{\max}$ is constant, and $d_{\max}\ge \eps \cs$, then the optimal number of rounds required to pack $J$ can be computed in $n^{O_{\eps}(1)}$ time.
\end{theorem}

\subsection{Case 2: $d_{\max}<\eps \cs$.}
\label{subsubsec:someconstants}
We first show the following results.

\begin{lemma}
\label{corollary:maincorollary_new}
\ursap\ and \urufp\ can be solved optimally in polynomial time if $L$ is a constant.
\end{lemma}
\begin{proof}
If $\cs > 3L$, apply \Cref{theorem:dynamicProgramming} to obtain a DSA packing with makespan at most $3L < \cs$. Thus all jobs can be packed inside one round of the uniform capacity profile and hence $\opt_{URS} = \opt_{URU} = 1$. 

Suppose now that $\cs \le 3L$. Consider \ursap\ first. Apply \Cref{lemma:maindynamicprogramming} to $J$. Since all demands are integers, at most $L$ jobs pass through any edge. Thus $\omega = L$. Also for any job $\js$, $h_{\js}$ can take at most $\cs \le 3L$ distinct values and therefore $U = 3L$. Thus the running time of the dynamic program is bounded by $(n\cdot 3L)^{O(L)}$, which is polynomial in $n$.

Similarly for \urufp\, we apply \Cref{lemma:corollaryofdp} with $\omega = L$ as before. The running time is bounded by $n^{O(L)}$.
\end{proof}

\begin{lemma}
\label{lemma:abcdef}
There exists an algorithm that 
\begin{enumerate}[(i)]
\item if $L=O_{\eps}(1)$, returns the optimal \ursap\ or \urufp\ solution,
\item else, returns a DSA packing of makespan at most $(1+15\eps )L$.
\end{enumerate}
\end{lemma}
\begin{proof}
Our algorithm is very similar to the algorithm in section 4 in \cite{BuchsbaumKKRT03}. If $L \le C\frac{1}{\eps^4}\log ^2\frac{1}{\eps}$, we apply \Cref{corollary:maincorollary_new} to get the optimal \ursap\ or \urufp\ solution. Otherwise steps 2,3,4 of the algorithm generate a DSA packing of makespan at most $(1+15\eps )L$, as proved by the authors in Theorem 4.1.
\end{proof}

Now we present our main algorithm in \Cref{algo:UniformRoundSap1}.

\begin{algorithm}[H]
%\textbf{If} $d_{\max} \ge \eps c$, apply \Cref{theorem:constantHeights} with $H = c$. Pack the jobs lying between consecutive slicing lines of $\Ls_{c}$ into separate rounds, and halt.\\
%\textbf{Else} apply \Cref{theorem:constantHeights} with $H = d_{\max}\lceil1/\eps\rceil$ to generate a DSA packing $\Ps_1$.\\
%Pack jobs in $J \setminus J^{\Ps_1}_{\Ls_{c}}$ lying between consecutive slicing lines into separate rounds.\\
%Apply \Cref{theorem:dynamicProgramming} to $J^{\Ps_1}_{\Ls_{c}}$. Let $\Ps_2$ be the packing generated.\\
%Pack jobs in $J^{\Ps_1}_{\Ls_{c}} \setminus J^{\Ps_2}_{\Ls_{c}}$ lying between consecutive slicing lines in $\Ps_2$ into separate rounds.\\
%For each slicing line $\ell \in \Ls_{c}$, pack the jobs in $J^{\Ps_2}_{\Ls_{c}}$ sliced by $\ell$ in $\Ps_2$ into separate rounds.\\
Apply \Cref{lemma:abcdef} to $J$. If it returns an optimal solution (i.e. halts in step (i)), halt.\\
Else let $\Ps$ be the DSA packing returned. Apply \Cref{lemma:sidelemma} to $\Ps$ with parameters $\delta = \eps$ and $\vartheta=\cs$.    
\caption{}
\label{algo:UniformRoundSap1}
\end{algorithm}

\textbf{Analysis:} If the algorithm halts in step 1, we get an optimal solution for \ursap\ or \urufp. Otherwise, from \Cref{lemma:abcdef}, the makespan of $\Ps$ is at most $(1+15\eps)L$. Thus \Cref{lemma:sidelemma} implies the number of rounds used in step 2 is bounded by $(1+O(\eps))r+2$. Note that any valid \ursap\ packing is also a valid \urufp\ packing. Since $r$ is a lower bound for both $\opt_{URS}$ and $\opt_{URU}$, \Cref{theorem:APTASforconstant} holds.  





==> Arxiv submission/general.tex <==
\section{General case}

We present our $O(\log\log n)$-approximation algorithms for the general cases of \rufp and \rsap.

We consider \rufp\ first and describe later how to extend our algorithm
to \rsap. We split the input jobs into large and small
jobs. We define $J_{\mathrm{large}}:=\{\js\in J|d_{\js}>b_{\js}/4\}$
and $J_{\mathrm{small}}:=\{\js\in J|d_{\js}\le b_{\js}/4\}$.
For the small jobs, we invoke a result by Elbassioni et al. \cite{ElbassioniGGKN12}
that yields a 16-approximation.
\begin{theorem}[\cite{ElbassioniGGKN12}]
\label{thm:Elbassioni-small} Given an instance of \rufp\ with
a set of jobs $J'$ such that $d_{\js}\le\frac{1}{4}b_{\js}$ for
each job $\js\in J'$. There is a polynomial time algorithm that computes
a 16-approximate solution to $J'$. 
\end{theorem}

Now consider the large jobs $J_{\mathrm{large}}$. For each job $\js\in J_{\mathrm{large}}$, 
we define a rectangle $R_{\js}=(s_{\js},b_{\js}-d_{\js})\times(t_{\js},b_{\js})$.
Note that $R_{\js}$ corresponds to the rectangle for $\js$ in \rsap
if we assign $\js$ the maximum possible height $h_{\js}$ (which is $h_{\js}:=b_{\js}-d_{\js}$). We say
that a set of jobs $J'\subseteq J_{\mathrm{large}}$ is \emph{top-drawn}
(underneath the capacity profile), if their rectangles are pairwise
non-overlapping, i.e., if $R_{\js}\cap R_{\js'}=\emptyset$ for any
$\js,\js'\in R_{\js}$. If a set of jobs $J'$ is top-drawn, then
it clearly forms a feasible round in \rufp. 
However, not every feasible round of \rufp is top-drawn. Nevertheless, we look for a solution to \rufp in which the
jobs in each round are top-drawn. The following lemma implies that
this costs only a factor of 8 in our approximation ratio.

\begin{lemma}[\cite{BonsmaSW11}] \label{lemma:itspacking}  Let $J'$ 
be the set of jobs packed in  a feasible round for a given instance of \rufp. Then $J'$ can
be partitioned into at most 8 sets such that each of them is top-drawn.\end{lemma}

Let $\R_{\mathrm{large}}:=\{R_{\js}|\js\in J_{\mathrm{large}}\}$
denote the rectangles corresponding to the large jobs and let $\omega_{\mathrm{large}}$ be 
their clique number, i.e., the size of the largest set $\R'\subseteq\R_{\mathrm{large}}$
such that all rectangles in $\R'$ pairwise overlap. It is known that
for such a set of rectangles $\R'$ there must be a point in which all rectangles
in $\R'$ overlap\footnote{\ari{This is a simple consequence of Helly's theorem. See \cite{helly22} for details.}}. Note that we need at least $\omega_{\mathrm{large}}$
rounds since we seek a solution with only top-drawn jobs in
each round. Our strategy is to invoke the following theorem on $\R_{\mathrm{large}}$. 

\begin{theorem}[\cite{parinbar}] \label{thm:parinyathm}  Given a
set of rectangles $\R'$ with clique number $\omega$. In polynomial
time, we can compute a coloring of the rectangles using $O(\omega\log\omega)$
colors such that no two rectangles of the same color intersect. \end{theorem}

Thus, if $\omega_{\mathrm{large}}=O(\log n)$ then we obtain an $O(\log\log n)$-approximation
as desired. However, it might be that $\omega_{\mathrm{large}}$ is
larger. In that case, we partition $\R_{\mathrm{large}}$ into $\omega_{\mathrm{large}}/\log n$
sets, such that each of them has a clique size of $O(\log n)$.
\begin{lemma}
There is a randomized polynomial time algorithm that w.h.p.~computes
a partition $\R_{\mathrm{large}}=\R_{1}\dot{\cup}...\dot{\cup}\R_{\omega_{\mathrm{large}}/\log m}$
such that for each set $\R_{i}$, the corresponding clique size is
at most $O(\log n)$.
\end{lemma}
\arir{removed log m claim, adapted to log n. Please check.}
\begin{proof}
We split the rectangles $\R_{\mathrm{large}}$ uniformly at random
into $\omega/\log n$ sets $\R_{1},\ldots,\R_{\omega/\log n}$. Thus
the expected clique size in each set $\R_{i}$ at any point $p$ under
the profile is at most $\log n$. Using the Chernoff bound, the probability
that the clique size at $p$ is more than $6\log n$ is at most $2^{-6\log n}=1/n^{6}$.
For each vertex $v_{i}$, let $p_{v_{i}}$ denote the point $(v_{i},\min(c_{i-1},c_{i}))$.
We draw a horizontal and vertical line passing through $p_{v_{i}}$
inside the capacity profile. \deb{This divides the region below the capacity
profile into $m^2 \le 4 n^{2}$ rectangular regions. Inside any such region, the clique size is maximized at the top edge of the rectangular region (since the rectangles are top-drawn).} Thus the probability that there exists a point $p$ under the capacity
profile where the clique size is more than $6\log n$ is at most $4n^{2}/n^{6}\le1/n^{3}$.
Hence using union bound, probability that clique size is more than
$6\log n$ at some point in some set $\R_{i}$ is at most $1/n^{2}$.
\end{proof}
We apply Theorem~\ref{thm:parinyathm} to each set $\R_{i}$
separately and thus obtain a coloring with $O(\log n\log\log n)$
colors. Thus, for all sets $\R_{i}$ together we use at most $\frac{\omega_{\mathrm{large}}}{\log n}O(\log n\log\log n)=O(\omega_{\mathrm{large}}\log\log n)$
colors. We pack the jobs from each color class to a separate round
for our solution to \rufp. Due to Lemma~\ref{lemma:itspacking},
we have that $\omega_{\mathrm{large}}$ is  $O(\opt_{UFP})$, which thus yields
an $O(\log\log n)$-approximation for \rufp, together with Theorem~\ref{thm:Elbassioni-small}. 

\begin{theorem} There exists a randomized $O(\log\log n)$-approximation
algorithm for \rufp\ for general edge capacities. \end{theorem}

%Since $m\le 2n-1$, this also yields an $O(\log \log n)$-approximate algorithm.

In order to obtain an algorithm for \rsap, we invoke the following
lemma due to \cite{MomkeW15} to each round of the computed solution
to \rufp.
\begin{lemma}[\cite{MomkeW15}]
\label{lem:UFP2SAP}Let $J'$ be the set of jobs packed in a feasible round for a given instance
of \rufp. Then in polynomial time we can partition $J'$ into  $O(1)$ sets and compute a height $h_{\js}$ for each job $\js\in J'$
such that each set yields a feasible round of \rsap.
\end{lemma}

This yields a solution to \rsap~with only $O(OPT_{SAP}\log\log n)$
rounds.

\begin{theorem} There exists a randomized $O(\log\log n)$-approximation
algorithm for \rsap\ for general edge capacities.\end{theorem}

\begin{comment}
\begin{lemma} \label{lem:constantforsmalljobs-1} There exist $O(1)$-approximation
algorithms for \rufp\ and \rsap\ for packing jobs in $S$. \end{lemma} 
\begin{proof}
For \rufp, Elbassioni et al. \cite{ElbassioniGGKN12} gave a 16-approximation
algorithm for packing jobs in $S$. For \rsap, our algorithm in \Cref{sec:generalRoundSap}
gives an asymptiotic $(16+\eps)$-approximation algorithm. 
\end{proof}
\begin{lemma} \label{lem:loglognforlargejobs-1} There exists a randomized
$O(\log\log m)$-approximation for \rufp\ and \rsap\ for packing
jobs in $T$. \end{lemma} 
\begin{proof}
Let $OPT'$ denote the optimal number of rounds required to pack all
jobs in $T$ as top-drawn sets. Then from \Cref{thm:itspacking},
we have $OPT'\le8OPT_{RU}\le8OPT_{RS}$.

We draw all the jobs as rectangles in a top-drawn fashion inside one
bin, i.e each job $\js$ is placed in the region $R_{\js}$ (thus
the top edge of the rectangle touches the capacity profile over its
bottleneck edge). Let $\omega$ denote the clique size, i.e the maximum
number of rectangles that overlap at any point. Thus $\omega\le OPT'$.

If $\omega<\log n$, we apply \Cref{thm:parinyathm} to get a coloring
using at most $\omega O(\log\log n)$ colors. Otherwise 

We apply \Cref{thm:parinyathm} to each set $J_{i}$. Thus with
probability at least $1-\frac{1}{n^{2}}$, each set can be colored
using $O(\log n\log\log n)$ colors. Thus total number of colors used
is $\frac{\omega}{\log n}O(\log n\log\log n)\le\omega O(\log\log n)$.
We pack all rectangles having the same color inside one bin. Thus
the total number of bins used is at most $O(\log\log n)OPT'\le O(\log\log n)OPT_{RU}\le O(\log\log n)OPT_{RS}$
(since $OPT'\le8OPT_{RU}\le8OPT_{RS}$). 
\end{proof}
Note that the above algorithm works even if $n$ is replaced by $m$
everywhere. With probability at least $1-\frac{1}{m^{2}}$, we would
get a packing using at most $O(\log\log m)OPT_{RS}$ bins. Combining
\Cref{lem:constantforsmalljobs} and \Cref{lem:loglognforlargejobs},
we have the following theorem.

\begin{theorem} There exists a randomized $\min(O(\log\log n,\log\log m))$-approximation
algorithm for \rufp\ and \rsap\ without NBA. \end{theorem}
\end{comment}



==> Arxiv submission/general_new.tex <==
\section{General Case}
In this section, present our algorithms for the general cases of \rufp and \rsap. We begin with 
our $O(\log\log \min\{n,m\})$-approximation algorithms where we 
consider \rufp\ first and describe later how to extend our algorithm
to \rsap. We split the input jobs into large and small
jobs. We define $J_{\mathrm{large}}:=\{\js\in J|d_{\js}>\mathfrak{b}_{\js}/4\}$
and $J_{\mathrm{small}}:=\{\js\in J|d_{\js}\le \mathfrak{b}_{\js}/4\}$.
For the small jobs, we invoke a result by Elbassioni et al. \cite{ElbassioniGGKN12}
that yields a 16-approximation.
\begin{theorem}[\cite{ElbassioniGGKN12}]
\label{thm:Elbassioni-small} We are given an instance of \rufp\ with
a set of jobs $J'$ such that $d_{\js}\le\frac{1}{4}\mathfrak{b}_{\js}$ for
each job $\js\in J'$. Then there is a polynomial time algorithm that computes
a 16-approximate solution to $J'$. 
\end{theorem}

Now consider the large jobs $J_{\mathrm{large}}$. For each job $\js\in J_{\mathrm{large}}$, 
we define a rectangle $R_{\js}=(s_{\js},\mathfrak{b}_{\js}-d_{\js})\times(t_{\js},\mathfrak{b}_{\js})$.
Note that $R_{\js}$ corresponds to the rectangle for $\js$ in \rsap
if we assign $\js$ the maximum possible height $h_{\js}$ (which is $h_{\js}:=\mathfrak{b}_{\js}-d_{\js}$). We say
that a set of jobs $J'\subseteq J_{\mathrm{large}}$ is \emph{top-drawn}
(underneath the capacity profile), if their rectangles are pairwise
non-overlapping, i.e., if $R_{\js}\cap R_{\js'}=\emptyset$ for any
$\js,\js'\in R_{\js}$. If a set of jobs $J'$ is top-drawn, then
it clearly forms a feasible round in \rufp. 
However, not every feasible round of \rufp is top-drawn. Nevertheless, we look for a solution to \rufp in which the
jobs in each round are top-drawn. The following lemma implies that
this costs only a factor of 8 in our approximation ratio.

\begin{lemma}[\cite{BonsmaSW11}] \label{lemma:itspacking}  Let $J' \subseteq J_{\mathrm{large}}$ 
be a set of jobs packed in  a feasible round for a given instance of \rufp. Then $J'$ can
be partitioned into at most 8 sets such that each of them is top-drawn.\end{lemma}

Let $\R_{\mathrm{large}}:=\{R_{\js}|\js\in J_{\mathrm{large}}\}$
denote the rectangles corresponding to the large jobs and let $\omega_{\mathrm{large}}$ be 
their clique number, i.e., the size of the largest set $\R'\subseteq\R_{\mathrm{large}}$
such that all rectangles in $\R'$ pairwise overlap. As a consequence of Helly's theorem (see \cite{helly22} for details), 
 for such a set of axis-parallel rectangles $\R'$ there must be a point in which all rectangles
in $\R'$ overlap. Note that we need at least $\omega_{\mathrm{large}}$
rounds since we seek a solution with only top-drawn jobs in
each round. 

We first reduce the original instance to the case where there are only $O(m^2)$ many distinct job demands. For each $i \in \{1,\ldots,m\}$, let $p_{i}$ denote the point $(i,c_{e_i})$. We draw a horizontal and a vertical line segment passing through $p_i$ and lying completely under the capacity profile (see \Cref{processingtopdrawn}(a)). This divides the region underneath the capacity profile into at most $m^2$ regions. Let $\Hs$ denote the set of horizontal lines and $\Vs$ denote the set of vertical lines drawn. Thus, the top edge of any rectangle corresponding to a large job must touch a line in $\Hs$. Now consider any rectangle $R_{\js}$ corresponding to a job $\js$. Let $h\in \Hs$ be the horizontal line segment lying just below the bottom edge of $R_{\js}$. We increase the value of $d_{\js}$ so that the the bottom edge of $R_{\js}$ now touches the line segment $h$ (see \Cref{processingtopdrawn}(b)). Since the rectangles were top-drawn, the clique number of this new set of large rectangles (denoted by $\R'_{\mathrm{large}}$) does not change. Also any feasible packing of $\R'_{\mathrm{large}}$ is a feasible packing of $\R_{\mathrm{large}}$.

\begin{figure}
\captionsetup{justification=centering} \captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{.5\textwidth}
\centering \resizebox{4.4cm}{1.3cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick] (1,0) -- (1,2.5) -- (3,2.5) -- (3,0.5) -- (4,0.5) -- (4,1.5) -- (5,1.5) -- (5,2.5) -- (6,2.5) -- (6,2) -- (7,2) -- (7,2.5) -- (8,2.5) -- (8,1.5) -- (9,1.5) -- (9,2) -- (10,2) -- (10,1.5) -- (11,1.5) -- (11,2.5) -- (13,2.5) -- (13,0);
			
			\draw[dashed] (1,0.5) -- (13,0.5);
			\draw[dashed] (4,1.5) -- (13,1.5); 
			\draw[dashed] (5,2) -- (8,2);
			\draw[dashed] (3,0) -- (3,0.5);			
			\draw[dashed] (4,0) -- (4,0.5);
			\draw[dashed] (5,0) -- (5,1.5);
			\draw[dashed] (6,0) -- (6,2);
			\draw[dashed] (7,0) -- (7,2);
			\draw[dashed] (8,0) -- (8,1.5);
			\draw[dashed] (9,0) -- (9,2);
			\draw[dashed] (10,0) -- (10,2);
			\draw[dashed] (11,0) -- (11,2);
			
			\draw[thick, color=blue, pattern=north east lines, pattern color = blue] (1,1.5) rectangle (3,2.5);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (7,1) rectangle (11,1.5);
			\draw[thick, color=green, pattern=north east lines, pattern color = green] (11,1) rectangle (13,2.5);
			\draw[thick, color=yellow, pattern=north east lines, pattern color = yellow] (5,1.5) rectangle (6,2.5);
			\draw[thick, color=violet, pattern=north east lines, pattern color = violet] (4,1) rectangle (6,1.5);
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
\centering \resizebox{4.4cm}{1.3cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick] (1,0) -- (1,2.5) -- (3,2.5) -- (3,0.5) -- (4,0.5) -- (4,1.5) -- (5,1.5) -- (5,2.5) -- (6,2.5) -- (6,2) -- (7,2) -- (7,2.5) -- (8,2.5) -- (8,1.5) -- (9,1.5) -- (9,2) -- (10,2) -- (10,1.5) -- (11,1.5) -- (11,2.5) -- (13,2.5) -- (13,0);
			
			\draw[dashed] (1,0.5) -- (13,0.5);
			\draw[dashed] (4,1.5) -- (13,1.5); 
			\draw[dashed] (5,2) -- (8,2);
			\draw[dashed] (3,0) -- (3,0.5);			
			\draw[dashed] (4,0) -- (4,0.5);
			\draw[dashed] (5,0) -- (5,1.5);
			\draw[dashed] (6,0) -- (6,2);
			\draw[dashed] (7,0) -- (7,2);
			\draw[dashed] (8,0) -- (8,1.5);
			\draw[dashed] (9,0) -- (9,2);
			\draw[dashed] (10,0) -- (10,2);
			\draw[dashed] (11,0) -- (11,2);
			
			\draw[thick, color=blue, pattern=north east lines, pattern color = blue] (1,0.5) rectangle (3,2.5);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (7,0.5) rectangle (11,1.5);
			\draw[thick, color=green, pattern=north east lines, pattern color = green] (11,0.5) rectangle (13,2.5);
			\draw[thick, color=yellow, pattern=north east lines, pattern color = yellow] (5,1.5) rectangle (6,2.5);
			\draw[thick, color=violet, pattern=north east lines, pattern color = violet] (4,0.5) rectangle (6,1.5);
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure}

 \caption{\textbf{(a)} The capacity profile along with the sets of lines $\Hs$ and $\Vs$ and some top-drawn jobs; \textbf{(b)} The jobs after processing; \protect \\
 }
\label{processingtopdrawn} 
\end{figure}






Note that $\R'_{\mathrm{large}}$ contains at most $m^4$ distinct types of jobs: the endpoints $s_{\js}$ and $t_{\js}$ can be chosen in ${m+1 \choose 2}\le m^2$ ways and the top and bottom edges of $R_{\js}$ must coincide with two lines from $\Hs$, which can be again chosen in ${m \choose 2}\le m^2$ ways. Let $U$ denote the number of types of job of the given instance and
let $\R'_{\mathrm{large}} = J_1\cup J_2 \cup \ldots \cup J_U$ be the decomposition of $\R'_{\mathrm{large}}$ into the $U$ distinct job types. 

We now formulate the configuration LP for this instance. Let $\Cs$ denote the set of all possible configurations of a round containing jobs from $\R'_{\mathrm{large}}$, drawn as top-drawn sets. For each $C \in \Cs$, we introduce a variable $x_C$, which stands for the number of rounds having configuration $C\in \Cs$. We write $J_k \triangleleft C$ if configuration $C$ contains a job from $J_k$ (note that $C$ can contain at most one job from $J_k$). Then the relaxed configuration LP and its dual (which contains a variable $y_k$ for each set $J_k$) are as follows.


\begin{align*}
\text{minimize} \quad \sum_{C\in \Cs} x_{C}&
&\text{maximize} \quad \sum_{k=1}^{U} |J_k|y_k& \\
\text{subject to} \quad \sum_{C:J_{k} \triangleleft C} x_C &\geq |J_k|, \quad k = 1,\ldots,U
&\text{subject to } \quad \sum_{k:J_{k} \triangleleft C} y_k &\leq 1, \quad C\in \Cs \\
x_{C} & \geq 0, \quad\, C\in \Cs
&y_k & \geq 0, \quad\, k =1, \dots, U
\end{align*}

\iffalse
\begin{alignat*}{2}
  & \text{minimize: } & & \sum_{C\in \Cs} x_{C} \\
   & \text{subject to: }& \quad & \sum_{\mathclap{{C:J_{k} \aw{\triangleleft} C}}}\begin{aligned}[t]
                    x_{C} & \geq |J_k|,& k & =1, \dots, U\\[3ex]
                  x_{C} & \geq 0, & \quad \quad C\in \Cs
                \end{aligned}
\end{alignat*}
The dual of the above LP  contains a variable $y_k$ for each set $J_k$ and is as follows.
\begin{alignat*}{2}
  & \text{maximize: } & & \sum_{k=1}^{U} |J_k|y_k \\
   & \text{subject to: }& \quad & \sum_{\mathclap{{k:J_{k} \aw{\triangleleft} C}}}\begin{aligned}[t]
                    y_{k} & \le 1,& \quad C\in \Cs\\[3ex]
                  y_{k} & \geq 0, & k & =1, \dots, U
                \end{aligned}
\end{alignat*}
\fi

The dual LP can be solved via the ellipsoid method with a suitable separation oracle. We interpret $y_k$ as the weight of each job in $J_k$. Given $(y_k)_{k\in \{1,\ldots,U\}}$, the separation problem asks whether there exists a configuration where jobs are drawn as top-drawn sets and the total weight of all the jobs in the configuration exceeds 1. For this, we invoke the following result of Bonsma et al.~\cite{BonsmaSW11}.

\begin{theorem} [\cite{BonsmaSW11}] \label{thm:dynamicprogramforufp} 
Given an instance of UFP with a set of jobs $J'$, the maximum-weight top-drawn subset of $J'$ can be computed in $O(nm^3)$ time.
\end{theorem}

Let $(x^*_C)_{C\in \Cs}$ be an optimal basic solution of the primal LP. 
By the rank lemma, there are at most
% Now since the ellipsoid algorithm returns a \textit{basic solution}, 
at most $U$ configurations $C$ for which $x^*_C$ is non-zero. 
For each non-zero $x^*_C$, we introduce $\lfloor x^*_C \rfloor$ rounds with configuration $C$, thus creating at most $8\cdot\opt_{UFP}$ rounds (due to \Cref{lemma:itspacking}). Now let $\R''_{\mathrm{large}}\subseteq \R'_{\mathrm{large}}$ be the large jobs that are yet to be packed and let $\omega''_{\mathrm{large}}$ be their clique number (and note that $\omega''_{\mathrm{large}}\le 8\cdot\opt_{UFP}$). In particular, a feasible solution to the configuration LP for the rectangles in $\R''_{\mathrm{large}}$ is to select one more round for each configuration $C$ with $x^*_C>0$. Therefore, we conclude that 
$\omega''_{\mathrm{large}} \le U \le m^4$ since there are at most $U$ configurations $C$ with $x^*_C>0$  and 
for each point, each configuration contains at most one rectangle covering this point.

Our strategy is to invoke the following theorem on $\R''_{\mathrm{large}}$.

\begin{theorem}[\cite{parinbar}] \label{thm:parinyathm}  Given a
set of rectangles with clique number $\omega$, in polynomial
time, we can compute a coloring of the rectangles using $O(\omega\log\omega)$
colors such that no two rectangles of the same color intersect. \end{theorem}

Thus, if $\omega''_{\mathrm{large}}=O(\log m)$ then we obtain an $O(\log\log m)$-approximation
as desired. However, it might be that $\omega''_{\mathrm{large}}$ is
larger. In that case, we partition $\R''_{\mathrm{large}}$ into $\omega''_{\mathrm{large}}/\log m$
sets, such that each of them has a clique size of $O(\log m)$.
\begin{lemma}
There is a randomized polynomial time algorithm that w.h.p.~computes
a partition $\R''_{\mathrm{large}}=\R_{1}\dot{\cup}...\dot{\cup}\R_{\omega''_{\mathrm{large}}/\log m}$
such that for each set $\R_{i}$, the corresponding clique size is
at most $O(\log m)$.
\end{lemma}
%\arir{removed log m claim, adapted to log n. Please check.}
\begin{proof}
We split the rectangles $\R''_{\mathrm{large}}$ uniformly at random
into $\omega''_{\mathrm{large}}/\log m$ sets $\R_{1},\ldots,\R_{\omega''_{\mathrm{large}}/\log m}$. Thus
the expected clique size in each set $\R_{i}$ at any point $p$ under
the profile is at most $\log m$. Using the Chernoff bound, the probability
that the clique size at $p$ is more than $8\log m$ is at most $2^{-8\log m}=1/m^{8}$. As before, we draw the set of horizontal and vertical lines $\Hs$ and $\Vs$, respectively,  under the capacity profile, dividing the region underneath the profile into at most $m^2$ regions. Clearly, the clique number must be the same at all points inside any such region. Thus the probability that there exists a point $p$ under the capacity profile where the clique size is more than $8\log m$ is at most $m^{2}/m^{8}\le1/m^{6}$.
Hence using union bound, probability that clique size is more than
$8\log m$ at some point in some set $\R_{i}$ is at most $1/m^{2}$ (since $\omega''_{\mathrm{large}}\le m^4$).
\end{proof}
We apply Theorem~\ref{thm:parinyathm} to each set $\R_{i}$
separately and thus obtain a coloring with $O(\log m\log\log m)$
colors. Thus, for all sets $\R_{i}$ together we use at most $\frac{\omega''_{\mathrm{large}}}{\log m}O(\log m\log\log m)=O(\omega''_{\mathrm{large}}\log\log m)$
colors. We pack the jobs from each color class to a separate round
for our solution to \rufp. This yields
an $O(\log\log m)$-approximation, together with Theorem~\ref{thm:Elbassioni-small}. 
Since $m\le 2n-1$ after our preprocessing, our algorithms are also $O(\log \log n)$-approximation algorithms.

\begin{theorem} There exists a randomized $O(\log\log \min\{n,m\})$-approximation
algorithm for \rufp\ for general edge capacities. \end{theorem}

%Since $m\le 2n-1$, this also yields an $O(\log \log n)$-approximate algorithm.

In order to obtain an algorithm for \rsap, we invoke the following
lemma due to \cite{MomkeW15} to each round of the computed solution
to \rufp.
\begin{lemma}[\cite{MomkeW15}]
\label{lem:UFP2SAP}Let $J'$ be the set of jobs packed in a feasible round for a given instance
of \rufp. Then in polynomial time we can partition $J'$ into  $O(1)$ sets and compute a height $h_{\js}$ for each job $\js\in J'$
such that each set yields a feasible round of \rsap.
\end{lemma}

This yields a solution to \rsap~with only $O(OPT_{UFP}\log\log m) \le O(OPT_{SAP}\log\log m)$
many rounds.

\begin{theorem} There exists a randomized $O(\log\log \min\{n,m\})$-approximation
algorithm for \rsap\ for general edge capacities.\end{theorem}


\subsection{An $O(\log \log \frac{1}{\delta})$-approximation algorithm with $(1+\delta)$-resource augmentation}

We show that if we are allowed a resource augmentation of a factor of $1+\delta$ for some $\delta>0$, we can get an $O(\log \log \frac{1}{\delta})$-approximation for both \rsap\ and \rufp. 
Consider \rufp\ first.

%\arir{add proof in appendix}
\begin{lemma}
\label{lem:Jpack}
Let $J^{(i)} := \{\js \in J  \mid \mathfrak{b}_{\js}\in [1/\delta^i,1/\delta^{i+1})\}$.  For packing jobs in $J^{(i)}$, it can be assumed that the capacity of each edge lies in the range $[1/\delta^i,2/\delta^{i+1})$.
\end{lemma}
Hence using the following theorem, we get a $O(\log \log \frac{1}{\delta})$-approximate solutions for each $J^{(i)}$,
which in particular uses at most $O(\opt_{UFP}\log\log\frac{1}{\delta})$ rounds.

\begin{theorem} [\cite{JahanjouKR17}]
There is a polynomial time $O(\log \log \frac{c_{\max}}{c_{\min}})$-approximation algorithm for \rufp.
\end{theorem}

Next we argue that we can combine the rounds computed for the sets $J^{(i)}$.
More precisely, we show that if we take one round from each set $J^{(0)},J^{(2)},J^{(4)},...$
and form their union, then they form a feasible round for the given
instance under $(1+\delta)$-resource augmentation. The same holds
if we take one round from each set $J^{(1)},J^{(3)},J^{(5)}, \dots$.

\begin{lemma}
\label{lem:combine}Take one computed round for each set $J^{(2k)}$
with $k\in\mathbb{N}$ or one computed round from each set $J^{(2k+1)}$
with $k\in\mathbb{N}$, and let $J'$ be their union. Then $J'$ is
a feasible round for the given instance of \rufp\ under $(1+\delta)$-resource
augmentation.
\end{lemma}

% For each set $J^{(i)}$ we computed a solution with at most $O(\opt_{UFP}\log\log\frac{1}{\delta})$
% rounds. 
Thus, due to Lemma~\ref{lem:combine} we obtain a solution
with at most $O(\opt_{UFP}\log\log\frac{1}{\delta})$ rounds for the overall
instance. As earlier, we  take the given \rufp~solution 
 and apply Lemma~\ref{lem:UFP2SAP} to it, which yields a solution
to \rsap\ with at most $O(\opt_{SAP}\log\log\frac{1}{\delta})$ rounds.

\begin{theorem}
\label{thm:loglogapproxwithresourceaugmentation}
There exists an $O(\log\log\frac{1}{\delta})$-approximation algorithm
for \rsap\ and \rufp\ for general edge capacities and $(1+\delta)$-resource
augmentation. 
\end{theorem}


\begin{comment}
\subsection{An $O(\log\log\frac{1}{\delta})$-approximation with $1+\delta$
resource augmentation}

Suppose now that we are given $(1+\delta)$-resource augmentation,
i.e., we can increase the capacity of each edge by a factor $1+\delta$,
while the compared optimal solution does not have this privilege.
Again, we start with \rufp. 

We divide the jobs based on their bottleneck capacities: for each
$i\in\mathbb{N}$ let $J^{(i)}:=\{\js\in J_{\mathrm{}}|b_{\js}\in[{1}/{\delta^{i}},{1}/{\delta^{i+1}})\}$.
First, we construct an $O(\log\log\frac{1}{\delta})$-approximate solution 
 under resource augmentation for each such set. Then, we
argue that we can combine the computed rounds for the sets using resource
augmentation.

Consider a set $J^{(i)}$. By definition no job in $J^{(i)}$ uses
an edge whose capacity is less than $1/\delta^{i}$. Also,
we can assume that the capacity of each edge is at most $2/\delta^{i+1}$
since for each edge $e$ with a capacity of more than $1/\delta^{i+1}$,
each jobs using it must also use the closest edge on the left or on
the right of $e$ with a capacity of at most $1/\delta^{i+1}$.
Thus, in a feasible round, $e$ is used by jobs from $J^{(i)}$ with a total
demand of at most $2/\delta^{i+1}$.
Thus, via scaling we can assume that the edge capacities are in the
range $[1,2/\delta)$. On the resulting instance, we invoke the algorithm
due to~\cite{JahanjouKR17}, 
% where $c_{\min}:=\min_{e}c_{e}$ and
% $c_{\max}:=\max_{e}c_{e}$, 
which hence in our case yields a $O(\log\log\frac{1}{\delta})$-approximation for each set $J^{(i)}$.
\begin{theorem}[\cite{JahanjouKR17}]
There is a polynomial time $O(\log\log\frac{c_{\text{max}}}{c_{\min}})$-approximation
algorithm for \rufp.
\end{theorem}

We argue that we can combine the rounds computed for the sets $J^{(i)}$.
More precisely, we show that if we take one round from each set $J^{(0)},J^{(2)},J^{(4)},...$
and form their union, then they form a feasible round for the given
instance under $(1+\delta)$-resource augmentation. The same holds
if we take one round from each set $J^{(1)},J^{(3)},J^{(5)}, \dots$.
\begin{lemma}
\label{lem:combine}Take one computed round for each set $J^{(2k)}$
with $k\in\mathbb{N}$ or one computed round from each set $J^{(2k+1)}$
with $k\in\mathbb{N}$, and let $J'$ be their union. Then $J'$ is
a feasible round for the given instance of \rufp\ under $(1+\delta)$-resource
augmentation.
\end{lemma}
\arir{add proof in appendix}

For each set $J^{(i)}$ we computed a solution with at most $O(\opt_{UFP}\log\log\frac{1}{\delta})$
rounds. Thus, due to Lemma~\ref{lem:combine} we obtain a solution
with at most $O(\opt_{UFP}\log\log\frac{1}{\delta})$ rounds for the overall
instance. Similarly like earlier, we can take the given solution to
\rufp and apply Lemma~\ref{lem:UFP2SAP} to it, which yields a solution
to \rsap.
\begin{theorem}
There exists an $O(\log\log\frac{1}{\delta})$-approximation algorithm
for \rsap\ and \rufp\ for general edge capacities and $(1+\delta)$-resource
augmentation. 
\end{theorem}


the combined jobs form a feasible 

Suppose we have a valid packing of $J_{i}$ using $x_{i}$ rounds.
Using resource augmentation, we can combine the packings of $J_{i}$
in the following way.

\begin{lemma} Let $\Rs^{i}$ be a round containing only jobs from
the set $J_{i}$. Then all jobs inside the rounds $\Rs^{0},\Rs^{2},\ldots$
can be packed inside one round $\Rs$ of the resource-augmented profile.
\end{lemma} 
\begin{proof}
Suppose we are allowed a resource augmentation of $1+\gamma$, for
some $\gamma>0$. Now since the bottleneck capacity of any job in
$J_{i}$ is at least $\frac{1}{\delta^{i}}$, on resource augmentation,
the capacity of any such edge would increase by at least $\frac{\gamma}{\delta^{i}}$.
Given the packing inside round $\Rs^{i}$, we shift up the position
of each job by $\frac{\gamma}{\delta^{i}}$ and place it in $\Rs$.

Now the jobs from $J_{i-2}$ do not go above $\frac{1}{\delta^{i-1}}+\frac{\gamma}{\delta^{i-2}}$.
We choose $\gamma$ such that $\frac{\gamma}{\delta^{i}}\ge\frac{1}{\delta^{i-1}}+\frac{\gamma}{\delta^{i-2}}$,
from which we get $\gamma=\frac{\delta}{1-\delta^{2}}=O(\delta)$. 
\end{proof}
Hence the total number of rounds used is $\max(x_{0},x_{2},\ldots)+\max(x_{1},x_{3},\ldots)$.
We now show that each $x_{i}$ is at most $O(\log\log\frac{1}{\delta})OPT$.
By scaling, we may assume all edges have capacity in the range $(1,1/\delta)$.
For 1/4-small jobs, we already have 16-approximation algorithms for
\rsap\ and \rufp. For 1/4-large jobs, Jahanjou et al. \cite{JahanjouKR17}
gave an $O(\log\log c_{\text{max}})$-approximation algorithm. Since
$c_{\text{max}}\le1/\delta$ for our case, this yields an $O(\log\log\frac{1}{\delta})$-approximation
algorithm. Hence we have the following result.

\iffalse We now show that each $x_{i}$ is at most $O(\frac{1}{\delta})OPT$.
By scaling, we may assume all edges have capacity in the range $(1,1/\delta)$.
For 1/4-small jobs, we already have 16-approximation algorithms for
\rsap\ and \rufp. So consider the 1/4-large jobs. We sort the jobs
in $J_{i}$ in non-decreasing order of their left endpoints and apply
the FF interval coloring algorithm. Hence in each round, at most 1
job is placed over each edge.

\begin{lemma} $x_{i}\le\frac{4}{\delta}OPT$. \end{lemma} 
\begin{proof}
Since the jobs are 1/4-large and the edge capacity is at most $1/\delta$,
there are at most $4/\delta$ jobs over any edge inside any round
of the optimal packing. Thus again by FF interval coloring, these
can be split into at most $\frac{4}{\delta}$ sets such that each
edge has at most 1 job over it. Thus the number of rounds used by
our algorithm to pack $J_{i}$ is at most $\frac{4}{\delta}OPT$. 
\end{proof}
\fi
\end{comment}



==> Arxiv submission/hardness_new.tex <==
\section{Lower Bounds}

\label{section:lowerboundnew} A simple reduction from the \textsc{Partition}
problem shows that it is NP-hard to obtain a better approximation ratio 
than $3/2$
for the classical \textsc{Bin Packing} problem. However, in the resulting
instances, the optimal solutions use only two or three bins. On the
other hand, \textsc{Bin Packing} admits an APTAS~\cite{de1981bin} and thus, 
for any $\eps>0$, a $(1+\eps)$-approximation algorithm for
instances in which $OPT$ is sufficiently large. % (compared to $1/\epsilon$).
Since \rsap\ and \rufp\ are generalizations of \textsc{Bin Packing} (even if $G$ has only a single edge),
the lower bound of $3/2$ continues to hold. However, maybe surprisingly,
we show that unlike \textsc{Bin Packing}, \rsap\ and \rufp\ do
not admit APTASes, even in the case of  uniform edge capacities. More
precisely, we provide a lower bound of $(1+1/1398)$ on the asymptotic
approximation ratio for \rsap\ and \rufp\ via a reduction from
the \textsc{2-Bounded Occurrence Maximum 3-Dimensional Matching} (\sbmdm)
problem. 

In \sbmdm, we are given as input three pairwise disjoint sets $X:=\{x_{1},x_{2},\dots,x_{q}\}$,
$Y:=\{y_{1},y_{2},\dots,y_{q}\}$, and $Z:=\{z_{1},z_{2},\dots,z_{q}\}$
and a set of triplets $\Ts\subseteq X\times Y\times Z$ such that
each element of $X\cup Y\cup Z$ occurs in exactly two triplets in
$\Ts$. Note that $|X|=|Y|=|Z|=q$ and $|\Ts|=2q$. A {\em matching}
is a subset $M\subseteq\Ts$ such that no two triplets in $M$ agree
in any coordinate. The goal is to find a matching of maximum cardinality
(denoted by $OPT_{3DM}$). Chlebik and Chlebikova \cite{chlebik2006complexity}
gave the following hardness result. 

\begin{theorem} [\cite{chlebik2006complexity}]\label{theorem:chlebikhardness_new}
For \sbmdm~there exists a family of instances such that for each
instance $K$ of the family, either $OPT_{3DM}(K)<\alpha(q):=\lfloor0.9690082645q\rfloor$
or $OPT_{3DM}(K)\ge\beta(q):=\lceil0.979338843q\rceil$, and it is
NP-hard to distinguish these two cases. 

\end{theorem}

Hardness of \sbmdm~has been useful in inapproximability results
for various (multidimensional) packing, covering, and scheduling problems,
e.g. vector packing \cite{woeginger1997there}, geometric bin packing
\cite{bansal2006bin}, geometric bin covering \cite{chlebik2009hardness},
generalized assignment problem \cite{chekuri2005polynomial}, etc.
Similar to these results, we also use gadgets based on a reduction
from \sbmdm\ to the 4-Partition problem. %, using which the hardness of a non-numeric problem is used to show hardness for a problem involving numeric data.
However, the previous techniques are not directly transferable to
our problem due to the inherent differences between these problems.
%For example, in both \vbp\ and \bp, vectors/rectangles can be translated both horizontally and vertically, unlike \rsap\ and \rufp\ where we can translate only vertically. 
Therefore, we first use the technique from \cite{woeginger1997there}
to associate certain integers with the elements of $X\cup Y\cup Z$
and $\Ts$ and then adapt the numeric data in a different way to obtain
the hard instances. % for \rsap\ and \rufp. 

Let $\rho=32q$ and let $\Vs$ be the set of $5q$ integers defined
as follows: $x'_{i}=i\rho+1\text{, for }1\le i\le|X|$, $y'_{j}=j\rho^{2}+2\text{, for }1\le j\le|Y|$,
$z'_{k}=k\rho^{3}+4\text{, for }1\le k\le|Z|,$ $\tau'_{l}=\rho^{4}-k\rho^{3}-j\rho^{2}-i\rho+8\text{, for each triplet }\tau_{l}=(x_{i},y_{j},z_{k})\in\Ts.$
Define $\gamma=\rho^{4}+15$. The following result is due to Woeginger
\cite{woeginger1997there}.

\begin{lemma} [\cite{woeginger1997there}]\label{lemma:woegingerlemma}
Four integers in $\Vs$ sum up to the value $\gamma$ if and only
if (i) one of them corresponds to some element $x_{i}\in X$, one
to some element $y_{j}\in Y$, one to an element $z_{k}\in Z$, and
one to some triplet $\tau_{l}\in\Ts$, and if (ii) $\tau_{l}=(x_{i},y_{j},z_{k})$
holds for these four elements. \end{lemma}

Now, we create a hard instance, tailor-made for our problems. We define
that our path $G=(V,E)$ has $40000\gamma$ vertices
that we identify with the numbers $0,1,...,40000\gamma$. For each
$x_{i}\in X$ (respectively $y_{j}\in Y$, $z_{k}\in Z$), we specify
two jobs $a_{X,i}$ and $a'_{X,i}$ (respectively $a_{Y,j}$, $a'_{Y,j}$
and $a_{Z,k}$, $a'_{Z,k}$), which will be called \textit{peers}
of each other. Each job $\js$ is specified by a triplet $(s_{\js},t_{\js},d_{\js})$.
We define
\begin{itemize}
\item $a_{X,i}=(0,20000\gamma-4x'_{i},999\gamma+4x'_{i})\text{ and }a'_{X,i}=(20000\gamma-4x'_{i},40000\gamma,1001\gamma-4x'_{i})$,
\item $a_{Y,j}=(0,20000\gamma-4y'_{j},999\gamma+4y'_{j})\text{ and }a'_{Y,j}=(20000\gamma-4y'_{j},40000\gamma,1001\gamma-4y'_{j})$,
and 
\item $a_{Z,k}=(0,20000\gamma-4z'_{k},999\gamma+4z'_{k})\text{ and }a'_{Z,k}=(20000\gamma-4z'_{k},40000\gamma,1001\gamma-4z'_{k})$. 
\end{itemize}
For each $\tau_{l}\in\Ts$, we define two jobs $b_{l}$ and $b'_{l}$
(also \textit{peers}) by: 
\begin{itemize}
\item $b_{l}=(0,19001\gamma-4\tau'_{l},999\gamma+4\tau'_{l})\text{ and }b'_{l}=(19001\gamma-4\tau'_{l},40000\gamma,1001\gamma-4\tau'_{l})$. 
\end{itemize}
Finally let $D$ be a set of $5q-4\beta(q)$ \emph{dummy} jobs each
specified by $(0,40000\gamma,2997\gamma)$. We define that each edge
$e\in E$ has a capacity of $c_{e}:=\cs:=4000\gamma$. This completes
the reduction. For any job $\js=(s_{\js},t_{\js},d_{\js})$ we define
its \emph{width} $w_{\js}:=t_{\js}-s_{\js}$. 

Let $A_{X}:=\{a_{X,i}\mid1\le i\le q\}$ and $A'_{X}:=\{a'_{X,i}\mid1\le i\le q\}$.
The sets $A_{Y}$, $A'_{Y}$, $A_{Z}$, $A'_{Z}$ are defined analogously.
Let $A:=A_{X}\cup A_{Y}\cup A_{Z}$ and $A':=A'_{X}\cup A'_{Y}\cup A'_{Z}$.
Finally let $B:=\{b_{l}\mid1\le l\le2q\}$ and $B':=\{b'_{l}\mid1\le l\le2q\}$. 

To provide some intuition, we first give an upper bound on the number
of jobs that can be packed in a round. All following lemmas, statements,
and constructions hold for both \rsap\ and \rufp. 
\begin{lemma}
\label{lem:maxnumberofjobs}
In any feasible solution any round can contain at most 8 jobs. 
\end{lemma}

We say that a round is \emph{nice }if it contains exactly 8 jobs.
It turns out that such a round corresponds exactly to one element
$\tau_{l}=(x_{i},y_{j},z_{k})\in\Ts$. We say that the jobs $a_{X,i},a'_{X,i},a_{Y,j},a'_{Y,j},a_{Z,k},a'_{Z,k},b_{l},$
and $b'_{l}$ \emph{correspond }to $\tau_{l}=(x_{i},y_{j},z_{k})$. 
\begin{lemma}
\label{lem:propertyofnicerounds}
We have that a round is nice if and only if there is an element $\tau_{l}=(x_{i},y_{j},z_{k})\in\Ts$
such that the round contains exactly the jobs that correspond to $\tau_{l}=(x_{i},y_{j},z_{k})$. 
\end{lemma}

Given an optimal solution $OPT_{3DM}$ to \sbmdm~ with $|OPT_{3DM}|\ge\beta(q)$, 
we construct a solution as follows:
\begin{enumerate}
\item Let $\Ms$ be any subset of $OPT_{3DM}$ with $|\Ms|=\beta(q)$. Create $\beta(q)$ \textit{\emph{nice}}\textit{ }rounds corresponding
to the elements in $\Ms$, i.e., for each element $\tau_{l}=(x_{i},y_{j},z_{k})\in \Ms$,
create a round containing the jobs that correspond to $\tau_{l}=(x_{i},y_{j},z_{k})$. 
\item For each $\tau_{l}\in\Ts\setminus \Ms$ create a round containing $b_l$ and $b'_l$ along with a dummy job. 
\item For each $x_{i}\in X$ (respectively $y_{j}\in Y$, $z_{k}\in Z$)
not covered by $\Ms$, pack $a_{X,i}$ and $a'_{X,i}$ (respectively
$a_{Y,j}$, $a'_{Y,j}$ and $a_{Z,k}$, $a'_{Z,k}$) together with
one dummy job in one round. 
\end{enumerate}
\begin{lemma}
\label{lem:reduction-1}If $|OPT_{3DM}|\ge\beta(q)$ then the constructed
solution is feasible and it uses at most $5q-3\beta(q)$ rounds.
\end{lemma}

\begin{proof}
One can easily check that all constructed rounds are feasible. In
step (1) we construct exactly $\beta(q)$ rounds. In step (2), we
construct $|\Ts|-\beta(q) = 2q-\beta(q)$ rounds, since
$|\Ts|=2q$. In step (3), we construct $3|\Ts\setminus \Ms|=3q-3|OPT_{3DM}|$
rounds. Hence, overall we construct at most $5q-3|OPT_{3DM}|\le5q-3\beta(q)$
rounds.
\end{proof}
Conversely, assume that $|OPT_{3DM}| < \alpha(q)$ and that we are
given any feasible solution to our constructed instance. We want to
show that it uses at least $5q-3\beta(q)+\frac{1}{7}(\beta(q)-\alpha(q))$
rounds. For this, a key property of our construction is given in the
following lemma.
\begin{lemma}
\label{lem:propertyofdummyrounds}
If a round contains a dummy job, then it can have at most three jobs:
at most one dummy job, at most one job from $A\cup B$, and at most one job from $A'\cup B'$. 
\end{lemma}

Let $n_{g}$ denote the number of nice rounds in our solution, $n_{d}$
the number of rounds with a dummy job, and $n_{b}$ the number of
remaining rounds. Note that each of the latter rounds can contain
at most 7 jobs each. Since all jobs in $A\cup A' \cup B \cup B'$ need to be assigned to a round,
we have that $8n_{g}+7n_{b}+2n_{d}\ge6q+2|\Ts|=10q$. Since the nice rounds correspond to a matching of the given instance
of~\sbmdm, we have that $n_{g}\le\alpha(q)$. Using this, we lower-bound
the number of used rounds in the following lemma.
\begin{lemma}
\label{lem:reduction-2}If $|OPT_{3DM}|< \alpha(q)$ then the number
of rounds in our solution is $n_{d}+n_{g}+n_{b}\ge(5q-3\beta(q))+\frac{1}{7}(\beta(q)-\alpha(q))$.
\end{lemma}

\begin{proof}
Since $8n_{g}+7n_{b}+2n_{d}\ge6q+2|\Ts|=10q$ and $n_{d}=5q-4\beta(q)$,
we obtain that $8n_{g}+7n_{b}\ge8\beta(q)$. Thus $n_{g}+n_{b}\ge\frac{8}{7}\beta(q)-\frac{1}{7}n_{g}$.
Since $n_{g}\le\alpha(q)$ the number of rounds is at least $n_{d}+n_{g}+n_{b}\ge5q-4\beta(q)+\frac{8}{7}\beta(q)-\frac{1}{7}\alpha(q)=(5q-3\beta(q))+\frac{1}{7}(\beta(q)-\alpha(q))$.
\end{proof}
Now Lemmas~\ref{lem:reduction-1} and \ref{lem:reduction-2} yield
our main theorem.

\begin{theorem} \label{theorem:hardnessproofnew-1} There exists
a constant $\delta_{0}>1/1398$, such that it is NP-hard to approximate
\rufp~and \rsap~in the case of uniform edge capacities with an
asymptotic approximation ratio less than $1+\delta_{0}$. \end{theorem} 
%\arir{Proof of theorem added in appendix}

\begin{comment}
, we get $8n_{g}+7n_{b}\ge8\beta(q)$. %\begin{equation}
%\label{eq: 2new}
%8n_g + 7n_b \ge 8\beta (q)
%\end{equation}
Thus $n_{g}+n_{b}\ge\frac{8}{7}\beta(q)-\frac{1}{7}n_{g}$. Since,
the nice rounds correspond to a matching for $K_{2}$, we have $n_{g}\le OPT_{3DM}(K_{2})\le\alpha(q)$.
Thus $OPT_{URS}(\Is_{K_{2}})=$.

For each $\tau_{l}=(x_{i},y_{j},z_{k})\in\Ts$ there are 8 jobs corresponding
to $\tau_{l}$: $a_{X,i},a'_{X,i},a_{Y,j},a'_{Y,j},a_{Z,k},a'_{Z,k}b_{l},$
and $b'_{l}$. One can easily check that they can be packed together
in one round, see Figure \ref{fig:Awellpackedbin_new} in Appendix
\ref{sec:appfig}. We say that such a round is \emph{neatly-packed}. 

Observe that the 8 jobs corresponding to a triplet $\tau_{l}=(x_{i},y_{j},z_{k})\in\Ts$
(4 from $A\cup B$ and their peers) can be packed together inside
one round as shown in Figure \ref{fig:Awellpackedbin_new} in Appendix
\ref{sec:appfig}. Such a round is said to be a \textit{neatly-packed}
round.

Our chosen instance ensures that the jobs satisfy following properties.
The omitted proofs are given in Appendix \ref{sec:applowb}.
\begin{lemma}
\label{lemma:lemma1new} The following conditions hold: 
\begin{enumerate}
\item $w_{a}+d_{a}=20999\gamma$, $\forall a\in A$, 
\item $w_{a'}+d_{a'}=21001\gamma$, $\forall a'\in A'$, 
\item $w_{b}+d_{b}=20000\gamma$, $\forall b\in B$, and 
\item $w_{b'}+d_{b'}=22000\gamma$, $\forall b'\in B'$. %\begin{proof}
%Can be verified easily.
%\end{proof}
\end{enumerate}
\end{lemma}

\begin{lemma} \label{lemma:lemma2new} The following statements hold:\\
 (i) the demands of four jobs in $A\cup B$ (or $A'\cup B'$) sum
to $4000\gamma$ iff they correspond to a triplet. (ii) the widths
of two jobs in $A\cup A'\cup B\cup B'$ sum to $40000\gamma$ iff
they are peers. \end{lemma}

\begin{lemma} \label{lemma:inequalities} The following inequalities
hold:\\
 (i) $d_{a}>999\gamma$, $\forall a\in A$, (ii) $d_{b}>1001\gamma$,
$\forall b\in B$, \\
 (iii) $d_{a'}>1000\gamma$, $\forall a'\in A'$, (iv) $d_{b'}>997\gamma$,
$\forall b'\in B'$. \end{lemma}

\begin{lemma} \label{lemma:twolemmas} The following statements hold:\\
 (i) if a round contains a dummy job, then it can have at most 1 job
each from $A\cup B$ and $A'\cup B'$, (ii) any round contains at
most 8 jobs. \end{lemma}

\begin{lemma} \label{lemma:startingandending} $s_{b'}<t_{a}$, $\forall a\in A$,
$b'\in B'$. \end{lemma}

We call a round containing exactly 8 jobs, a \textit{nice} round.
Observe that the 8 jobs corresponding to a triplet $\tau_{l}=(x_{i},y_{j},z_{k})\in\Ts$
(4 from $A\cup B$ and their peers) can be packed together inside
one round as shown in Figure \ref{fig:Awellpackedbin_new} in Appendix
\ref{sec:appfig}. Such a round is said to be a \textit{neatly-packed}
round. We now prove the following lemma.

\begin{lemma} \label{lemma:niceround} A round is nice if and only
if it is neatly-packed. \end{lemma} 
\begin{proof}
The if part follows from definition since any neatly-packed round
contains 8 jobs.

Now we show nice rounds are neatly-packed. From the proof of \Cref{lemma:twolemmas}(ii),
a nice round must have 4 jobs each from $A\cup B$ and $A'\cup B'$.
Since any \rsap\ packing is also a valid \rufp\ packing, it suffices
to prove the result for \rufp\ packings.

We begin by showing that such a round can contain at most 1 job from
$B$. Suppose at least 2 jobs from $B$ are present. From \Cref{lemma:inequalities}(i)
and (ii), the sum of demands of all the 4 jobs from $A\cup B$ is
then $>2\cdot1001\gamma+2\cdot999\gamma=4000\gamma$, a contradiction.
Now we show that at least one job from $B$ must be present. Suppose
not, then there are 4 jobs from $A$. \Cref{lemma:startingandending}
then implies that no job from $B'$ can be present. Thus there must
be 4 jobs from $A'$. But from \Cref{lemma:inequalities}(iii),
the sum of demands of these jobs from $A'$ would be $>4\cdot1000\gamma=4000\gamma$,
a contradiction. Hence, the round must have exactly 1 job from $B$
and thus 3 jobs from $A$.

As shown above, the round cannot contain 4 jobs from $A'$ and thus
must have at least 1 job from $B'$. We now show that exactly 1 job
from $B'$ must be present. \Cref{lemma:startingandending} implies
any job in $B'$ must share at least one edge with any job in $A$.
Let $e$ be such a common edge. Therefore, if at least 2 jobs from
$B'$ are present, sum of demands of all jobs over $e$ would be $>3\cdot999\gamma+2\cdot997\gamma>4000\gamma$
(from \Cref{lemma:inequalities}), a contradiction. Thus the round
has exactly 1 job from $B'$ and thus 3 jobs from $A'$.

Consider the leftmost edge $e_{1}$. Let the 4 jobs from $A\cup B$
lying over $e_{1}$, from top to bottom, be $\js_{1},\js_{2},\js_{3},\js_{4}$.
Similarly let the 4 jobs from $A'\cup B'$ lying over the rightmost
edge $e_{m}$ be $\js_{5},\js_{6},\js_{7},\js_{8}$ from top to bottom.
Then the following inequalities must hold: 
\begin{align}
\sum_{i=1}^{4}d_{\js_{i}}\le4000\gamma,\qquad\sum_{i=5}^{8}d_{\js_{i}}\le4000\gamma,\qquad\sum_{i=1}^{8}w_{\js_{i}}\le4\cdot40000\gamma=160000\gamma\label{eq: 200}
\end{align}

Adding the three inequalities, we get $\sum_{i=1}^{8}(d_{\js_{i}}+w_{\js_{i}})\le168000\gamma$.
Also \Cref{lemma:lemma1new} implies that $\sum_{i=1}^{8}(d_{\js_{i}}+w_{\js_{i}})=3\cdot20999\gamma+3\cdot21001\gamma+1\cdot20000\gamma+1\cdot22000\gamma=168000\gamma$.
Thus \eqref{eq: 200} must be satisfied with equality. \Cref{lemma:lemma2new}(i)
then implies that the four jobs from $A\cup B$ must correspond to
a triplet. Also since equality holds in \eqref{eq: 200}, \Cref{lemma:lemma2new}(ii)
implies that their corresponding peers must be present. Thus the round
is neatly-packed. 
\end{proof}
Now we state the main result of this section. For ease of presentation,
we work only with \ursap. The same proof also works for \urufp.
\begin{theorem} \label{theorem:hardnessproofnew} There exists a
constant $\sigma>1+1/1398$, such that it is NP-hard to approximate
\ursap\ with an asymptotic approximation ratio less than $\sigma$.
\end{theorem} 
\begin{proof}
Let $\Is_{K}$ be the \ursap\ instance generated by the above reduction
on a \sbmdm~instance $K$. First, consider an instance $K_{1}$
of \sbmdm~such that $OPT_{3DM}(K_{1})\ge\beta(q)$. We claim that
$OPT_{URS}(\Is_{K_{1}})\le5q-3\beta(q)$. Consider any set $\Ms$
of $\beta(q)$ triplets in the maximum matching. Create $\beta(q)$
\textit{neatly-packed} rounds corresponding to these triplets. For
each $\tau_{l}\in\Ts\setminus\Ms$, pack $B_{l}$ and $B'_{l}$ along
with a dummy job in a round, thus creating $2q-\beta(q)$ rounds.
Finally, for each $x_{i}\in X$ (respectively $y_{j}\in Y$, $z_{k}\in Z$)
not covered by $\Ms$, pack $A_{X,i}$ and $A'_{X,i}$ (respectively
$A_{Y,j}$, $A'_{Y,j}$ and $A_{Z,k}$, $A'_{Z,k}$) along with one
dummy job in a round. Thus all jobs are packed and total number of
rounds used is $5q-3\beta(q)$.

Now consider an instance $K_{2}$ such that $OPT_{3DM}(K_{2})<\alpha(q)$.
We will now lower bound $OPT_{URS}(\Is_{K_{2}})$. Consider the optimal
packing. Let $n_{d}=5q-4\beta(q)$ denote the number of rounds containing
dummy jobs, $n_{g}$ denote the number of \textit{nice} rounds and
$n_{b}$ denote the number of remaining rounds. Clearly, each of the
$n_{b}$ rounds contain at most 7 jobs. %Since all jobs in $A \cup B$ are packed and each of the $n_d$ rounds can contain at most 1 job from $A \cup B$, we have $4n_g + 4n_b + n_d \ge 3q + |\Ts| = 5q$. 
%As  $n_d = 5q - 4\beta (q)$, we get 
%\begin{equation}
%\label{eq: 1new}
%n_g + n_b \ge \beta (q)
%\end{equation}  
Since all jobs in $A\cup A'\cup B\cup B'$ need to be packed, we have
$8n_{g}+7n_{b}+2n_{d}\ge6q+2|\Ts|=10q$. As $n_{d}=5q-4\beta(q)$,
we get $8n_{g}+7n_{b}\ge8\beta(q)$. %\begin{equation}
%\label{eq: 2new}
%8n_g + 7n_b \ge 8\beta (q)
%\end{equation}
Thus $n_{g}+n_{b}\ge\frac{8}{7}\beta(q)-\frac{1}{7}n_{g}$. Since,
the nice rounds correspond to a matching for $K_{2}$, we have $n_{g}\le OPT_{3DM}(K_{2})\le\alpha(q)$.
Thus $OPT_{URS}(\Is_{K_{2}})=n_{d}+n_{g}+n_{b}\ge5q-4\beta(q)+\frac{8}{7}\beta(q)-\frac{1}{7}\alpha(q)=(5q-3\beta(q))+\frac{1}{7}(\beta(q)-\alpha(q))$.

Thus, we may choose $\sigma=1+\frac{1}{7}\frac{\beta(q)-\alpha(q)}{5q-3\beta(q)}$
and the result follows using \Cref{theorem:chlebikhardnessnew}. 
\end{proof}
For $\alpha(q)=\lfloor0.9690082645q\rfloor$ and $\beta(q)=\lceil0.979338843q\rceil$,
a simple calculation will show $\sigma>1+1/1398$. In particular,
this proves that these problems do not admit APTAS.
\end{comment}



==> Arxiv submission/improvements.tex <==
\section{Improvements}
\subsection{\rufp\ with NBA}
We assume that $c_{\min}=1$ and the demand of each job is at most 1. Let $S$ be the set of jobs whose demands are $\le 1/2$ and $T=J\setminus S$. Consider any job $\js\in S$ and let $i$ be such that $\frac{1}{2^{i+1}}< d_{\js} \le \frac{1}{2^i}$. We round up the demand of $\js$ to $\frac{1}{2^i}$. Let $J_i$ denote the set of jobs whose demands after rounding is $\frac{1}{2^i}$ and let $n_{e,i}=|\{\js \in J_i \mid e\in P_{\js}\}|$. Let $U_{e,i}=\{e\in E\mid n_{e,i}<2r\}$ and $J'_i = \{\js \in J_i\mid \exists e\in U_{e,i} \text{ such that } e\in P_{\js}\}$. Let $J''_i = J\setminus J'_i$. Let $n'_{e,i}=|\{\js \in J'_i \mid e\in P_{\js}\}|$ and $n''_{e,i}=|\{\js \in J''_i \mid e\in P_{\js}\}|$. Clearly $n'_{e,i} < 4r$.

\begin{lemma}
The jobs in $S$ can be packed into at most $8r$ bins.
\end{lemma}
\begin{proof}
For packing jobs in $\bigcup\limits_i J''_i$, we introduce a set $\Ss$ of $4r$ bins. Inside each of these bins, we create a profile $I_i$, such that the capacity of edge $e$ in $I_i$ equals $\frac{1}{2^i} \lfloor \frac{n_{e,i}}{2r} \rfloor$. Jobs in $J''_i$ shall be packed under these profiles $I_i$. The congestion of any edge having non-zero capacity in $I_i$ is $\frac{\frac{1}{2^i}n''_{e,i}}{\frac{1}{2^i}\lfloor \frac{n_{e,i}}{2r} \rfloor} \le \frac{\frac{n_{e,i}}{2r}}{\lfloor \frac{n_{e,i}}{2r} \rfloor}\cdot 2r \le 4r$. Also since each job in $J''_i$ has demand equal to $\frac{1}{2^i}$, the capacity of each edge in $I_i$ is an integral multiple of the demand. Thus using \Cref{theorem:nomikostheorem}, jobs in $J''_i$ can be packed under the $4r$ profiles $I_i$. The load on edge $e$ inside any bin is at most $\sum\limits_i \frac{1}{2^i} \lfloor \frac{n_{e,i}}{2r} \rfloor \le \sum\limits_i \frac{1}{2^{i+1}}\frac{n_{e,i}}{r} \le \frac{1}{r} \sum\limits_{\js \colon e\in P_j} d_j \le c_e$. Thus this is a valid packing.

For packing jobs in $\bigcup\limits_i J'_i$, we introduce a set $\Ts$ of $4r$ bins. For each $i$, we consider the jobs in $J'_i$ in non-decreasing order of their left endpoints and assign a job to the first bin in $\Ts$ where it does not overlap with any job from $J'_i$ that have been assigned till now. Since $n'_{e,i}\le 4r$, such an assignment is always possible. Thus over any edge $e$ inside any bin of $\Ts$, at most 1 job from each $J_i$ can be present. Thus the load on edge $e$ is at most $\sum\limits_i \frac{1}{2^i} \le 1 \le c_e$ and this is a valid packing. 

Hence all jobs in $S$ can be packed into $8r$ bins.
\end{proof}

\begin{lemma}
The jobs in $T$ can be packed into $4r$ bins.
\end{lemma}
\begin{proof}
We round up the demand of each job in $T$ to $1$ and round down the capacity of each edge to the nearest integer. Thus the congestion increases by at most a factor of 4. Hence by applying \Cref{theorem:nomikostheorem}, jobs in $T$ can be packed into at most $4r$ bins.
\end{proof}

Thus we get a packing of $J$ using at most $12r$ bins.

\subsection{Without NBA}
A set of jobs is said to form a top-drawn set if each job is placed in the rectangular region $R_{\js}=(s_{\js},b_{\js}-d_{\js})\times (t_{\js},b_{\js})$ under the capacity profile such that $R_{\js}\cap R_{\js'}=\phi$ for any two jobs $\js$ and $\js'$. We use the following results.

\begin{theorem}
\label{thm:itspacking}
\cite{BonsmaSW11} Let $F$ be a feasible UFPP packing of $1/k$-large jobs inside 1 bin. Then $F$ can be split into $2k$ top-drawn sets.
\end{theorem}

\begin{theorem}
\label{thm:parinyathm}
\cite{parinbar} Given a set of rectangles with clique number $\omega$, a coloring of the rectangles using $O(\omega \log \omega)$ colors such that no two rectangles of the same color intersect, can be computed in polynomial time.
\end{theorem}

Let $S=\{\js \in J\mid d_{\js}\le \frac{1}{4}b_{\js}\}$ and $T=J\setminus S$.

\begin{lemma}
\label{lem:constantforsmalljobs}
There exist $O(1)$-approximation algorithms for \rufp\ and \rsap\ for packing jobs in $S$.
\end{lemma}
\begin{proof}
For \rufp, Elbassioni et al. \cite{ElbassioniGGKN12} gave a 16-approximation algorithm for packing jobs in $S$. For \rsap, our algorithm in \Cref{sec:generalRoundSap} gives an asymptiotic $(16+\eps)$-approximation algorithm.
\end{proof}



\begin{lemma}
\label{lem:loglognforlargejobs}
There exists a randomized $O(\log \log n)$-approximation for \rufp\ and \rsap\ for packing jobs in $T$.
\end{lemma}
\begin{proof}
Let $OPT'$ denote the optimal number of rounds required to pack all jobs in $T$ as top-drawn sets. Then from \Cref{thm:itspacking}, we have $OPT' \le 8 OPT_{RU} \le 8 OPT_{RS}$. 

We draw all the jobs as rectangles in a top-drawn fashion inside one bin, i.e each job $\js$ is placed in the region $R_{\js}$ (thus the top edge of the rectangle touches the capacity profile over its bottleneck edge). Let $\omega$ denote the clique size, i.e the maximum number of rectangles that overlap at any point. Thus $\omega \le OPT'$. 

If $\omega < \log n$, we apply \Cref{thm:parinyathm} to get a coloring using at most $\omega O(\log \log n)$ colors. Otherwise we split the set of jobs uniformly at random into $\omega/\log n$ sets $J_1,\ldots,J_{\omega/\log n}$. Thus the expected clique size in each set $J_i$ at any point $p$ under the profile is $\le \log n$. Using Chernoff bound, the probability that the clique size at $p$ is more than $6\log n$ is at most $2^{-6\log n}=1/n^6$. For each vertex $v_i$, let $p_{v_i}$ denote the point $(v_i,\min (c_{i-1},c_i))$. We draw a horizontal and vertical line passing through $p_{v_i}$ inside the capacity profile. This divides the region below the capacity profile into $m^2\le 4n^2$ regions. Clearly inside each region, the clique size must be the same, since all rectangles are top-drawn. Thus the probability that there exists a point $p$ under the capacity profile where the clique size is more than $6\log n$ is at most $4n^2/n^6 \le 1/n^3$. Hence using union bound, probability that clique size is more than $6\log n$ at some point in some set $J_i$ is at most $1/n^2$. 

We apply \Cref{thm:parinyathm} to each set $J_i$. Thus with probability at least $1-\frac{1}{n^2}$, each set can be colored using $O(\log n\log \log n)$ colors. Thus total number of colors used is $\frac{\omega}{\log n}O(\log n\log \log n) \le \omega O(\log \log n)$. We pack all rectangles having the same color inside one bin. Thus the total number of bins used is at most $O(\log\log n)OPT'\le O(\log \log n)OPT_{RU}\le O(\log\log n)OPT_{RS}$ (since $OPT'\le 8OPT_{RU}\le 8OPT_{RS}$). 
\end{proof}

Note that the above algorithm works even if $n$ is replaced by $m$ everywhere. With probability at least $1-\frac{1}{m^2}$, we would get a packing using at most $O(\log\log m)OPT_{RS}$ bins. Combining \Cref{lem:constantforsmalljobs} and \Cref{lem:loglognforlargejobs}, we have the following theorem.

\begin{theorem}
There exists a randomized $\min (O(\log \log n, \log \log m))$-approximation algorithm for \rufp\ and \rsap\ without NBA.
\end{theorem}


\subsection{An $O(\log \log \frac{1}{\delta})$-approximation without NBA with $1+\delta$ resource augmentation}
We divide the jobs based on their bottleneck capacities: let $J_i$ be the set of jobs with bottleneck capacity in the range $(\frac{1}{\delta^i},\frac{1}{\delta^{i+1}})$, $i\ge 0$. Suppose we have a valid packing of $J_i$ using $x_i$ rounds. Using resource augmentation, we can combine the packings of $J_i$ in the following way. 

\begin{lemma}
Let $\Rs^i$ be a round containing only jobs from the set $J_i$. Then all jobs inside the rounds $\Rs^0,\Rs^2,\ldots$ can be packed inside one round $\Rs$ of the resource-augmented profile.
\end{lemma}
\begin{proof}
Suppose we are allowed a resource augmentation of $1+\gamma$, for some $\gamma > 0$. Now since the bottleneck capacity of any job in $J_i$ is at least $\frac{1}{\delta^i}$, on resource augmentation, the capacity of any such edge would increase by at least $\frac{\gamma}{\delta^i}$. Given the packing inside round $\Rs^i$, we shift up the position of each job by $\frac{\gamma}{\delta^i}$ and place it in $\Rs$.

Now the jobs from $J_{i-2}$ do not go above $\frac{1}{\delta^{i-1}}+\frac{\gamma}{\delta^{i-2}}$. We choose $\gamma$ such that $\frac{\gamma}{\delta^i} \ge \frac{1}{\delta^{i-1}}+\frac{\gamma}{\delta^{i-2}}$, from which we get $\gamma = \frac{\delta}{1-\delta^2}=O(\delta)$.
\end{proof}

Hence the total number of rounds used is $\max (x_0,x_2,\ldots) + \max (x_1,x_3,\ldots)$. We now show that each $x_i$ is at most $O(\log \log \frac{1}{\delta})OPT$. By scaling, we may assume all edges have capacity in the range $(1,1/\delta)$. For 1/4-small jobs, we already have 16-approximation algorithms for \rsap\ and \rufp. For 1/4-large jobs, Jahanjou et al. \cite{JahanjouKR17} gave an $O(\log \log c_{\text{max}})$-approximation algorithm. Since $c_{\text{max}}\le 1/\delta$ for our case, this yields an $O(\log \log \frac{1}{\delta})$-approximation algorithm. Hence we have the following result.






\iffalse
We now show that each $x_i$ is at most $O(\frac{1}{\delta})OPT$. By scaling, we may assume all edges have capacity in the range $(1,1/\delta)$. For 1/4-small jobs, we already have 16-approximation algorithms for \rsap\ and \rufp. So consider the 1/4-large jobs. We sort the jobs in $J_i$ in non-decreasing order of their left endpoints and apply the FF interval coloring algorithm. Hence in each round, at most 1 job is placed over each edge. 

\begin{lemma}
$x_i \le \frac{4}{\delta}OPT$.
\end{lemma}
\begin{proof}
Since the jobs are 1/4-large and the edge capacity is at most $1/\delta$, there are at most $4/\delta$ jobs over any edge inside any round of the optimal packing. Thus again by FF interval coloring, these can be split into at most $\frac{4}{\delta}$ sets such that each edge has at most 1 job over it. Thus the number of rounds used by our algorithm to pack $J_i$ is at most $\frac{4}{\delta}OPT$.
\end{proof}
\fi

\begin{corollary}
There exists an $O(\log \log \frac{1}{\delta})$-approximation algorithm for \rsap\ and \rufp\ without NBA when the edge capacities can be augmented by a factor $1+\delta$.
\end{corollary}




==> Arxiv submission/prelim.tex <==
\section{Introduction}

\label{sec:intro} %Scheduling and routing problems are well-studied in combinatorial optimization. 
The unsplittable flow on a path problem (UFP) %\cite{bansal2014logarithmic},
and the storage allocation problem~(SAP) %~\cite{MomkeW20} 
are two
well-studied problems in combinatorial optimization. In this paper,
we study \rufp~and \rsap, which are two related natural problems
that also generalize the classical {\sc Bin Packing} problem. % \cite{karmarkar1982efficient}.

%In  both \rsap~and \rufp, we are given a path graph $G:=(V,E)$ and a set of jobs $J$ with $|J|=n$. Each job $\js \in J$ has demand $d_{\js} \in \mathbb{N}$, source $s_{\js} \in V$, and sink $t_{\js} \in V$. Job $\js$ spans  $P_{\js}$: the $(s_{\js}, t_{\js})$-path. 
%which we call the start and end vertex of job $j$, respectively. 
%Every edge $e \in E$ has an integral capacity $c_e$. The set $I := \{c_e \mid e \in E\}$ is called the \cpro. 

In both \rufp and \rsap, we are given as input a path $G=(V,E)$
and a set of $n$ jobs $J$. We assume that $\{v_{0},v_{1},\dots,v_{m}\}$
are the vertices in $V$ from left to right and then for each $i \in \{1,...,m\}$ there is an
edge $e_{i}:=\{v_{i-1},v_{i}\}$.
Each job $\js\in J$ has integral demand $d_{\js}\in\mathbb{N}$,
a source $v_{s_{j}}\in V$, and a sink $v_{t_{j}}\in V$. We say that
each job $\js$ spans the path $P_{\js}$ which we define to be the path between
$v_{s_{\js}}$ and $v_{t_{\js}}$. For every edge $e\in E$, we are
given an integral capacity $c_{e}$. A useful geometric interpretation
of the input path and the edge capacities is the following (see Figure~\ref{closedcor2}):
consider the interval $[0,m)$ on the $x$-axis and a function $c\colon[0,m)\to\mathbb{N}$.
Each edge $e_{k}$ corresponds to the interval $[k-1,k)$ and each
vertex $v_{i}$ corresponds to the point $i$. For edge $e_{k}$, we
define $c(x)=c_{e_{k}}$ for each $x\in[k-1,k)$.

In the \rufp~problem, the objective is to partition the jobs $J$
into a minimum number of sets $J_{1},...,J_{k}$ (that we will denote
by \emph{rounds}) such that the jobs in each set $J_{i}$ form a \emph{valid
packing, }i.e., they obey the edge capacities, meaning that $\sum_{\js\in J_{i}:e\in P_{\js}}d_{\js}\le c_{e}$
for each $e\in E$. In the \rsap~problem, we require to compute
additionally for each set $J_{i}$ a non-overlapping set of rectangles
underneath the capacity profile, corresponding to the jobs in $J_{i}$
(see Figure~\ref{closedcor2}). Formally, we require for each job $\js\in J_{i}$
to determine a height $h_{\js}$ with $h_{\js}+d_{\js}\le c_{e}$
for each edge $e\in P_{\js}$, yielding a rectangle $R_{\js}=(s_{\js},t_{\js})\times(h_{\js},h_{\js}+d_{\js})$,
such that for any two jobs $\js,\js'\in J_{i}$ we have that $R_{\js}\cap R_{{\js}'}=\emptyset$.
Again, the objective is to minimize the number of rounds.

Note that unlike \rsap, in \rufp\ we do not need to pack the jobs
as contiguous rectangles. Hence, intuitively in \rufp\ we can slice the rectangles
vertically and place different slices at different heights. See Figure~\ref{closedcor2}
for the differences between the problems. % between packings in \rsap\ and \rufp. Note also that in both problems, the horizontal positions of the jobs are fixed, i.e. job $\js$ must be placed between $s_{\js}$ and $t_{\js}$.
\iffalse 
\begin{figure}
\centering \captionsetup{justification=centering} \begin{tikzpicture}
\node[inner sep=0pt] (figthree) at (0,0)
    {\includegraphics[width=.33\textwidth]{fig3.png}};
    
\node[inner sep=0pt] (figfour) at (4.5,-0.005)
    {\includegraphics[width=.33\textwidth]{fig4.png}}; 
    
\node[inner sep=0pt] (figfive) at (9,0)
    {\includegraphics[width=.33\textwidth]{fig5.png}};      
    
\node[inner sep=0pt] (figone) at (1.2,2.5)
    {\includegraphics[width=.33\textwidth]{fig1.png}};     
    
\node[inner sep=0pt] (figtwo) at (7.2,2.22)
    {\includegraphics[width=.33\textwidth]{fig2.png}}; 
    
\draw[thick] (7.2,1.3) node {\scriptsize \textbf{(b)} Capacity profile};
\draw[thick] (1.2,1.45) node {\scriptsize \textbf{(a)} A set of 7 jobs (numbers};
\draw[thick] (1.2,1.2) node {\scriptsize represent the demands)};       

\draw[thick] (0,-0.75) node {\scriptsize \textbf{(i)}};
\draw[thick] (4.5,-0.75) node {\scriptsize \textbf{(ii)}};
\draw[thick] (2.25,-1.1) node {\scriptsize \textbf{(c)} Any optimal ROUND-SAP packing must use at least 2 rounds};
\draw[thick] (9,-0.85) node {\scriptsize \textbf{(d)} An optimal ROUND-UFPP packing};
\draw[thick] (9,-1.15) node {\scriptsize using only 1 round};
\end{tikzpicture} \caption{\rsap\ and \rufp\ packings}
\label{fig:roundsapandroundufp} 
\end{figure}

\fi

\begin{figure}
\captionsetup{justification=centering} \captionsetup[subfigure]{justification=centering}
\begin{subfigure}[b]{.5\textwidth} \centering \resizebox{4.4cm}{1.9cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick, color=pink, pattern=north east lines, pattern color = pink] (5,0.25) rectangle (8,1.25);			
			\draw[thick, color=brown, pattern=north east lines, pattern color = brown] (11,0.25) rectangle (13,2.25);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (2,1.5) rectangle (10,2);
			\draw[thick, color=blue, pattern=north east lines, pattern color = blue] (1,2.25) rectangle (3,4.25);
			\draw[thick, color=yellow, pattern=north east lines, pattern color = yellow] (4,2.25) rectangle (6,3.25);
			\draw[thick, color=violet, pattern=north east lines, pattern color = violet] (9,2.5) rectangle (12,3);
			\draw[thick, color=green, pattern=north east lines, pattern color = green] (7,3.25) rectangle (11,4.25);
			
			\draw[thick] (8.25,0.75) node {\Large \textbf{2}};
			\draw[thick] (13.25,1.25) node {\Large \textbf{4}};
			\draw[thick] (10.25,1.75) node {\Large \textbf{1}};
			\draw[thick] (3.25,3.25) node {\Large \textbf{4}};
			\draw[thick] (6.25,2.75) node {\Large \textbf{2}};
			\draw[thick] (12.25,2.75) node {\Large \textbf{1}};
			\draw[thick] (11.25,3.75) node {\Large \textbf{2}};
	
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure} \begin{subfigure}[b]{.5\textwidth}
\centering \resizebox{4.4cm}{1.3cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick] (1,0) -- (1,2.5) -- (3,2.5) -- (3,0.5) -- (4,0.5) -- (4,1.5) -- (5,1.5) -- (5,2.5) -- (6,2.5) -- (6,2) -- (7,2) -- (7,2.5) -- (8,2.5) -- (8,1.5) -- (9,1.5) -- (9,2) -- (10,2) -- (10,1.5) -- (11,1.5) -- (11,2.5) -- (13,2.5) -- (13,0);
			
			\foreach \x in {1,...,5}
				\draw[dashed] (0.8,\x/2) -- (13.2,\x/2);
			\foreach \x in {1,...,5}
				\draw[thick] (13.4,\x/2) node {\Large \textbf{\x}};
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure}

\vspace{0.5cm}
 %\hspace*{-0.5in}
 \centering \begin{subfigure}[b]{.3\textwidth} %\centering
 \resizebox{4.35cm}{1.2cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick] (1,0) -- (1,2.5) -- (3,2.5) -- (3,0.5) -- (4,0.5) -- (4,1.5) -- (5,1.5) -- (5,2.5) -- (6,2.5) -- (6,2) -- (7,2) -- (7,2.5) -- (8,2.5) -- (8,1.5) -- (9,1.5) -- (9,2) -- (10,2) -- (10,1.5) -- (11,1.5) -- (11,2.5) -- (13,2.5) -- (13,0);
			
		\draw[thick, color=red, pattern=north east lines, pattern color = red] (2,0) rectangle (10,0.5);
		\draw[thick, color=blue, pattern=north east lines, pattern color = blue] (1,0.5) rectangle (3,2.5);
		\draw[thick, color=green, pattern=north east lines, pattern color = green] (7,0.5) rectangle (11,1.5);	
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure} %\hspace{0.5cm}
 \begin{subfigure}[b]{.3\textwidth} \centering \resizebox{4.35cm}{1.2cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick] (1,0) -- (1,2.5) -- (3,2.5) -- (3,0.5) -- (4,0.5) -- (4,1.5) -- (5,1.5) -- (5,2.5) -- (6,2.5) -- (6,2) -- (7,2) -- (7,2.5) -- (8,2.5) -- (8,1.5) -- (9,1.5) -- (9,2) -- (10,2) -- (10,1.5) -- (11,1.5) -- (11,2.5) -- (13,2.5) -- (13,0);
			
			\draw[thick, color=yellow, pattern=north east lines, pattern color = yellow] (4,0) rectangle (6,1);
			\draw[thick, color=pink, pattern=north east lines, pattern color = pink] (5,1) rectangle (8,2);
			\draw[thick, color=violet, pattern=north east lines, pattern color = violet] (9,0) rectangle (12,0.5);
			\draw[thick, color=brown, pattern=north east lines, pattern color = brown] (11,0.5) rectangle (13,2.5);
	
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure} %\hspace{0.5cm}
 \begin{subfigure}[b]{.3\textwidth} \centering \resizebox{4.35cm}{1.2cm}{ \begin{tikzpicture}
			\draw[thick] (1,0) -- (13,0);
			\foreach \x in {1,...,13}
				\draw[thick] (\x,0.1) -- (\x,-0.1);
			\foreach \x in {0,...,12}
				\draw[thick] (\x+1,-0.45) node {\Large \textbf{\x}};
			\draw[thick] (1,0) -- (1,2.5) -- (3,2.5) -- (3,0.5) -- (4,0.5) -- (4,1.5) -- (5,1.5) -- (5,2.5) -- (6,2.5) -- (6,2) -- (7,2) -- (7,2.5) -- (8,2.5) -- (8,1.5) -- (9,1.5) -- (9,2) -- (10,2) -- (10,1.5) -- (11,1.5) -- (11,2.5) -- (13,2.5) -- (13,0);
			
			\draw[thick, color=blue, pattern=north east lines, pattern color = blue] (1,0) rectangle (3,2);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (2,2) rectangle (3,2.5);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (3,0) rectangle (4,0.5);
			\draw[thick, color=yellow, pattern=north east lines, pattern color = yellow] (4,0) rectangle (6,1);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (4,1) rectangle (5,1.5);
			\draw[thick, color=pink, pattern=north east lines, pattern color = pink] (5,1) rectangle (7,2);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (5,2) rectangle (6,2.5);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (6,0.25) rectangle (7,0.75);
			\draw[thick, color=pink, pattern=north east lines, pattern color = pink] (7,0) rectangle (8,1);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (7,1) rectangle (8,1.5);
			\draw[thick, color=green, pattern=north east lines, pattern color = green] (7,1.5) rectangle (8,2.5);
			\draw[thick, color=red, pattern=north east lines, pattern color = red] (8,0) rectangle (10,0.5);
			\draw[thick, color=green, pattern=north east lines, pattern color = green] (8,0.5) rectangle (11,1.5);
			\draw[thick, color=violet, pattern=north east lines, pattern color = violet] (9,1.5) rectangle (10,2);
			\draw[thick, color=violet, pattern=north east lines, pattern color = violet] (10,0) rectangle (12,0.5);
			\draw[thick, color=brown, pattern=north east lines, pattern color = brown] (11,0.5) -- (11,2.5) -- (12,2.5) -- (12,2) -- (13,2) -- (13,0) -- (12,0) -- (12,0.5) -- (11,0.5);
	
		\end{tikzpicture}} \caption{}
\label{fig:zbend1} \end{subfigure} \caption{\textbf{(a)} A set of 7 jobs with demands written beside; \textbf{(b)}
The capacity profile; \protect \\
 \textbf{(c),(d)} Any valid \rsap\ packing requires at least 2 rounds;
\protect \\
 \textbf{(e)} A valid \rufp\ packing using only 1 round.}
\label{closedcor2} 
\end{figure}

\rufp and \rsap arise naturally in the setting of resource allocation
 with connections to many fundamental optimization problems,
e.g., wavelength division multiplexing (WDM) and optical
fiber minimization (see \cite{andrews2005bounds,winkler2003wavelength}
for more details and practical motivations). The path can represent
a network with a chain of communication links in which we need to
send some required transmissions in a few rounds so that they obey the
given edge capacities. The edges can also correspond to discrete time
slots, each slot models a job that we might want to execute, and the
edge capacities model the available amount of a resource shared by
the jobs like energy or machines. \rufp\ models routing in optical
networks, where each copy of the resource corresponds to a distinct
frequency. As the number of available distinct frequencies is limited,
minimizing the number of rounds for a given set of requests is a natural
objective. \rsap\ is motivated by settings in which jobs need a
contiguous portion of an available resource, e.g., a consecutive portion
of the computer memory or a frequency bandwidth. Another application
is ad-placement, where each job is an advertisement that requires
a contiguous portion of the banner \cite{MomkeW15}.

\begin{comment}
In \ursap\ and \urufp, all edges of $G_{\text{path}}$ have the
same capacity $\cs$. The \rtree~problem is a generalization of
\rufp\, where the input graph $G_{\text{tree}}$ is a tree. Each
job $\js\in J$ spans the unique path between vertices $v_{s_{\js}}$
and $v_{t_{\js}}$ of $G_{\text{tree}}$. The objective is to pack
$J$ using the minimum number of \textit{tree-rounds} of the capacity
profile. In \urtree, all edges of $G_{\text{tree}}$ have the same
capacity $\cs$. %In the \orufp\ problem, the jobs arrive one-by-one in an online fashion, and we need to pack them immediately in an irrevocable manner, without the complete knowledge of the future. %The objective is again to pack all jobs using minimum number of rounds.
Throughout this paper, we assume that maximum demand of a job is at
most the minimum capacity of an edge. This is called the No Bottleneck
Assumption (NBA), a standard assumption \cite{BonsmaSW11} in this
setting.
\end{comment}

\rufp and \rsap are APX-hard as they contain the
classical \textsc{Bin Packing} problem as a special case when $G$
has only one single edge. However, while for \textsc{Bin Packing}
there exists an asymptotic polynomial time approximation scheme (APTAS)\footnote{For formal definitions of notions like asymptotic approximation ratio, (asymptotic) polynomial time approximation scheme, etc. we refer to Appendix \ref{sec:approx}.}, it is open whether such an
algorithm exists for \rufp\ or \rsap. The best known approximation
algorithm for \rufp\ is a $O(\min\{\log n,\log m,\log\log c_{\max}\})$-approximation~\cite{JahanjouKR17}.
For the special case of \rufp~of uniform edge capacities, Pal~\cite{pal2014approximation} gave a 3-approximation. Elbassioni et al.~\cite{ElbassioniGGKN12} gave a 24-approximation algorithm for the problem under the no-bottleneck
assumption (NBA) which states that the maximum task demand is upper-bounded
by the minimum edge capacity. A result in (the full version of)~\cite{MomkeW15}
states that any solution to an instance of UFP can be partitioned
into at most 80 sets of tasks such that each of them is a solution
to the corresponding SAP instance. This immediately yields approximation algorithms
for \rsap: a 240-approximation for the case of uniform capacities, 
a 1920-approximation under the NBA, and a $O(\min\{\log n,\log m,\log\log c_{\max}\})$-approximation for the general case. These are the best known results
for~\rsap. 

%Bartal and Leonardi \cite{bartal1997line} have given a tight $O(\log n)$-competitive algorithms for the online setting when the graph is a $n \times n$ grid, and all capacities and demands are 1. 

\subsection{Our Contributions}

\label{subsec:ourwork} %We give asymptotic $(2+\eps)$-approximation algorithms for both \ursap\ and \urufp. This  improves   upon the previous 3-approximation for \urufp\ \cite{ElbassioniGGKN12}. We are not aware of any previous constant approximation algorithms for \ursap. We bootstrap our algorithm to get an asymptotic $(16+\eps)$-approximation algorithm for \rsap. Elbassioni et al. \cite{ElbassioniGGKN12} gave 24- and 64-approximation algorithms for the \rufp\ and \rtree\ problems, respectively. We do a refined analysis of their algorithm and improve its approximation ratio to 16 and 49, resp.
%For the hardness, we show that both \rsap\ and \rufp, unlike classical bin packing problem,  do not admit an asymptotic polynomial-time approximation scheme (APTAS), even in the uniform capacity case. 

First, we show that both \rsap\ and \rufp, unlike the classical
\textsc{Bin Packing} problem, do not admit an APTAS, even in the uniform
capacity case. We achieve this via a gap preserving reduction from
the 3D matching problem. We create a numeric version of the problem
and define a set of hard instances for both \rsap\ and \rufp. Together
with a result of Chlebik and Chlebikova \cite{chlebik2006complexity},
we derive an explicit lower bound on the asymptotic approximation
ratio for both problems. Our hardness result holds even for the case in which
in the optimal packing no round contains more than $O(1)$ jobs, i.e., a case in which
we can even enumerate all possible packings in polynomial time.

For the case of uniform edge capacities, we give asymptotic $(2+\eps)$-approximation
algorithms for both \rufp\ and \rsap, and absolute $(2.5+\eps)$ and 3-approximation algorithms for the two problems, respectively. 
This improves upon the previous absolute
3- and 240-approximation algorithms mentioned above. Note that for
both problems our factor of 2 is a natural threshold: in many algorithms
for UFP and SAP \cite{BonsmaSW11, AnagnostopoulosGLW14, GrandoniMW017, GMWZ018, MomkeW15, MomkeW20}, 
the input tasks are partitioned 
into tasks that are relatively small and relatively
large (compared to the edge capacities). Then, both sets
are handled separately with very different sets of techniques. This
inherently loses a factor of 2. Our algorithms are based on a connection
of our problems to the dynamic storage allocation (DSA) problem and
we show how to use some known deep results for DSA~\cite{BuchsbaumKKRT03} in our
setting. In DSA the goal is to place some given tasks
as non-overlapping rectangles, minimizing the height of the resulting packing. Hence, it is somewhat surprising
that also for \rufp (where we do not have this requirement) it yields
the needed techniques for an improved approximation.

For the general cases of \rufp and \rsap\, we give an $O(\log\log \min\{m, n\})$-approximation
algorithm. Depending on the concrete values of $n,m,$ and $c_{\max}$,
this constitutes an up to exponential improvement compared to the
best known result for \rufp~\cite{JahanjouKR17} and for \rsap\ (by the reasoning via~\cite{MomkeW15} above). We divide the
input tasks into two sets: tasks that use a relatively large portion
of the capacity of \emph{at least one} of their edges (large tasks) and tasks
that use a relatively small portion of the capacity of \emph{all} of their
edges (small tasks). For each large task, we fix a corresponding rectangle
that is drawn at the maximum possible height underneath the capacity curve
(even for \rufp~for which we do not need to represent the given
tasks as rectangles) and we seek a solution in which in each round
these corresponding rectangles are non-overlapping. It follows from
known results that this loses at most a factor of~$O(1)$~\cite{BonsmaSW11, JahanjouKR17}.
% Then, we show that we can reduce the given instance to the setting
% in which each input point overlaps at most $O(\log m)$ of these rectangles.
Then, we solve a configuration-LP for our problem which we solve via a separation oracle. We take the integral parts of
its solution and show that the fractional parts yield several instances of our original problem 
in which each point overlaps at most $O(\log m)$ rectangles.
Using a recent result by Chalermsook and Walczak \cite{parinbar} 
on the coloring
number of rectangle intersection graphs, 
we obtain an $O(\log\log m)$-approximation.
For the small tasks of a given \rufp instance, a result in~\cite{ElbassioniGGKN12}
yields an $O(1)$-approximation, which yields our $O(\log\log m)$-approximation
for \rufp. Finally, we use the result in~\cite{MomkeW15} mentioned above in order to turn this algorithm even into a $O(\log\log m)$-approximate
solution for \rsap. Then we study the setting of resource augmentation,
i.e., where we can increase the edge capacities by a factor of $1+\delta$
while the compared optimal solution does not have this privilege.
In this case, we show that we can reduce the given problem to the
setting in which the edge capacites are in the range $[1,1/\delta)$.
Applying the algorithm from~\cite{JahanjouKR17} then yields a $O(\log\log\frac{1}{\delta})$-approximation
for this case for \rufp, and with a similar argumentation as before
also for \rsap.

Furthermore, for the case of the NBA we improve the absolute approximation
ratio from 24 to 12 for \rufp, and from 1920 to 24 for
\rsap, and we obtain even an asymptotic $(16+\eps)$-approximation for \rsap. For \rsap~we show that we can reduce the general case to the
case of uniform edge capacities, losing only a factor of~8. Thus,
future improvements for the case of uniform edge capacities will directly yield improvements 
for the case of the NBA. For \rufp~we partition the input jobs
into several sets. For some of them we reduce the given setting
to the case of unit job demands and integral edge capacities and invoke
an algorithm from \cite{NomikosPZ01} for this case. For the others, we show that 
a simple greedy routine works sufficiently well. 

If in \rufp we are given a tree instead of a path, we obtain the \rtree~problem. The best known result for it under the NBA
is a 64-approximation \cite{ElbassioniGGKN12}. We are not aware of any better result for
uniform edge capacities.
We improve the best
known approximation ratio under the NBA to 55 and also provide a 5.5-approximation algorithm for the case of uniform edge capacities.

%?? {[}?{]} to $5.5$ for
%uniform edge capacities and from $64$ to 55 under the NBA. 



See Table~\ref{table:results} for an overview of our results.
Due to space limitations, many proofs had to be moved to the appendix.

\begin{table}[h!]
\centering{}%
\begin{tabular}{|l|l|l|l|}
\hline 
\textbf{Problem}  & \textbf{Edge capacites} & \textbf{Previous approximation}  & \textbf{Improved approximation} \tabularnewline
\hline 
\rufp  & uniform  & 3 \cite{pal2014approximation}  & asymp. $2+\eps$, abs. 2.5$+\eps$  \tabularnewline
\rsap  & uniform  & $240$  \cite{pal2014approximation, MomkeW15} & asymp. $2+\eps$, abs. 3 \tabularnewline
\rufp  & NBA & 24  \cite{ElbassioniGGKN12} & abs. 12 \tabularnewline
\rsap  & NBA & 1920   \cite{ElbassioniGGKN12, MomkeW15} & asymp. $16+\eps$, abs. 24\tabularnewline
\rufp  & general & $O(\log\min\{n,m,\log c_{\max}\})$ \cite{JahanjouKR17}& abs. $O(\log\log \min\{n,m\})$\tabularnewline
\rsap  & general & $O(\log\min\{n,m,\log c_{\max}\})$ \cite{JahanjouKR17}& abs. $O(\log\log \min\{n,m\})$ \tabularnewline
\rufp  & general with r.a. & $O(\log\min\{n,m,\log c_{\max}\})$ \cite{JahanjouKR17}& abs. $O(\log\log(1/\delta))$\tabularnewline
\rsap  & general with r.a. & $O(\log\min\{n,m,\log c_{\max}\})$ \cite{JahanjouKR17}& abs. $O(\log\log(1/\delta))$\tabularnewline
\rtree  & uniform & 64  \cite{ElbassioniGGKN12}& asymp. 5.1, abs. $5.5$\tabularnewline
\rtree  & NBA & 64  \cite{ElbassioniGGKN12}& asymp. 49, abs. 55\tabularnewline
\hline 
\end{tabular}
\vspace{0.4cm}
\caption{Overview of our results. We distinguish the settings according to uniform edge capacities, the no-bottleneck-assumption (NBA), general edge capacities, and general edge capacities with $(1+\delta)$-resource augmentation (r.a.). Also, we distinguish
between absolute approximation ratios and asymptotic approximation ratios. All listed previous results are absolute approximation ratios.
}
\label{table:results} 
\end{table}

\subsection{Other Related Work\label{subsec:relwork}}
% If all job demands and edge capacities are same, then \rufp and \rsap reduce
% to the interval-coloring problem on paths \cite{epstein2009online}.
Adamy and Erlebach~\cite{adamy2003online}
studied \rufp~for uniform edge capacities in the online setting and gave a 195-approximation
algorithm, which was subsequently improved to 10 \cite{narayanaswamy2004dynamic,azar2006improved}.
% Elbassioni et al.~\cite{ElbassioniGGKN12} gave a 3-approximation
% algorithm for \urufp~and a 24-approximation for \rufp, under NBA.
%For \orufp, the best competitive ratio known for this
%problem is 78 \cite{epstein2009online} and a lower bound of slightly greater than 3 is known \cite{kierstead1988linearity}.
Without the NBA, Epstein et al.~\cite{epstein2009online} showed that
no deterministic online algorithm can achieve a competitive ratio better
than $\Omega(\log\log n)$ or $\Omega(\log\log\log(c_{\max}/c_{\min}))$.
They also gave a $O(\log c_{\max}$)-competitive algorithm, where
$c_{\max}$ is the largest edge capacity. Without the NBA, recently Jahanjou
et al.~\cite{JahanjouKR17} gave 
% an offline $O(\min(\log n,\log m,\log\log c_{\max}))$-approximation
% algorithm and 
a $O(\min(\log m,\log\log c_{\max}))$-competitive
algorithm. 
% They also studied a restricted class of \rufp\ instances
% called $\alpha$-small, where the size of each task is at most $\alpha$
% times the capacity of its bottleneck edge (i.e., the edge of minimum capacity of the path of the task), and presented an $O(\log(1/(1-\alpha)))$-approximation
% algorithm.


\rufp\ and \rsap\ are related to many fundamental optimization
problems. For example, \rsap~can be interpreted as an intermediate
problem between two-dimensional bin packing (2BP) and the rectangle coloring
problem (RC). In 2BP, the goal is to find an axis-parallel nonoverlapping
packing of a given set of rectangles (which we can translate in both
dimensions) into minimum number of unit square bins. If all edges
have the same capacity then \rsap~can be seen as a variant of 2BP
in which the horizontal coordinate of each item is fixed and we can
choose only the vertical coordinate. For 2BP, the present best asymptotic
approximation guarantee is 1.406 \cite{bansal2014binpacking}. On
the other hand, in RC, all rectangles are fixed and the goal is to
color the rectangles using a minimum number of colors such that no two
rectangles of the same color intersect. For RC, recently Chalermsook
and Walczak~\cite{parinbar} have given a polynomial-time algorithm that uses
only $O(\omega\log\omega)$ colors, where $\omega$ is the clique number of the corresponding
intersection graph (and hence a lower bound on the number of needed colors). Another related problem is Dynamic Storage Allocation
(DSA), where the objective is to pack the given tasks (with fixed
horizontal location) such that the maximum vertical height, $\max_{\js}(h_{\js}+d_{\js})$
(called the \textit{makespan}) is minimized. The current best known approximation ratio 
for DSA is $(2+\eps)$ \cite{BuchsbaumKKRT03}.

In a sense \rufp and \rsap~are `{\sc{Bin Packing}}-type' problems, and their corresponding
`{\sc{Knapsack}}-type' problems are UFP and SAP, respectively, where each
task has an associated profit and the goal is to select a subset of
tasks which can be packed into one single round satisfying the corresponding
valid packing constraints. There is a series of work \cite{GrandoniMW017,bansal2014logarithmic,BatraG0MW15,AnagnostopoulosGLW14,GMWZ018, GMW22a}
in UFP, culminating in a PTAS~\cite{GMW22b}. It is maybe surprising that
\rufp~does not admit an APTAS, even though  UFP admits a PTAS. 
For SAP, the currently best polynomial time approximation ratio is
$2+\eps$ \cite{MomkeW15}, which has been recently improved to $1.969+\eps$
\cite{MomkeW20} for the case of uniform capacities, and also a quasi-polynomial time
$(1.997+\eps)$-approximation is known for quasi-polynomially bounded input data.

%\awr{the PTAS was accepted at STOC now, but the list of accepted papers is not out yet}
% the present best $(\frac{e+2}{e+1}+\eps)$-approximation
% \cite{GMW22a}. 
% Very recently, a PTAS for UFP has been claimed \cite{GMW22b}. 


There are many other related problems, such as two-dimensional knapsack
\cite{GalvezGHI0W17,Jansen2004, Galvez00RW21}, strip packing \cite{GGIK16,Galvez0AJ0R20, DeppertJ0RT21},
maximum independent set of rectangles \cite{AHW19,parinbar,mitchellFocs, Galvez22}, guillotine
separability of rectangles \cite{KMR20, khan2021guillotine, KS21}, weighted bipartite edge
coloring \cite{KhanS15}, maximum edge disjoint paths \cite{chuzhoy2016polylogarithmic},
etc. We refer the readers to \cite{khan2015approximation,CKPT17}
for an overview of these problems.

\section{Preliminaries}

\label{sec:prelim} 
% Now we introduce some definitions and notations.
Let $\opt_{UFP}$ and $\opt_{SAP}$ denote the optimal number of rounds required to
pack all jobs of a given instance of \rufp and \rsap, respectively. By simple preprocessing, we can assume that each vertex
in $V$ corresponds to endpoint(s) of some job(s) in $J$, and hence $m\le2n-1$.
% The \textit{bottleneck edge} of a job $\js$ is defined as $\arg\min\{c_{e}:e\in P_{\js}\}$.
For each job $\js$ denote by $\mathfrak{b}_{\js}$ the minimum capacity of 
the edges in $P_{\js}$, i.e., $\min\{c_{e}:e\in P_{\js}\}$ which we denote as the \textit{bottleneck
capacity} of $\js$. Job $\js$
is said to \textit{pass through} edge $e$ if $e\in P_{\js}$. The \textit{load} on edge $e$ is defined as $l_{e}:=\sum_{e\in P_{\js}}d_{\js}$,
the total sum of demands of all jobs passing through $e$. Let $L:=\max_{e}l_{e}$
denote the maximum \textit{load}. The \textit{congestion} $r_{e}$
of edge $e$ is defined as $r_{e}:=\lceil l_{e}/c_{e}\rceil$, and
$r:=\max_{e}r_{e}$ denotes the maximum \textit{congestion}.
Clearly, $r$ is a lower bound on $\opt_{UFP}$ and $\opt_{SAP}$. 

%\awr{how about $R$ instead of $r$ like $L$ and $l$? Maybe too late at this stage}

%Let $c_{\max}$ and $c_{\min}$ denote the maximum and minimum edge capacities, respectively, and $d_{\max}$ and $d_{\min}$ denote the maximum and minimum job demands, respectively. 
%\arir{Debajyoti, shift definitions to local places, as needed.}
% Throughout this paper, we assume that $d_{\max}\le c_{\min}$.
% This is called the No Bottleneck Assumption (NBA).

% A \textit{slicing line} is defined as a horizontal line spanning between
% the leftmost and rightmost vertices of $G_{\text{path}}$. A \textit{slicing
% line} located at height $h$ from the $x$-axis will be denoted by
% $\ell_{h}$. Let $\Ls_{h}$ denote the set of all slicing lines located
% at heights that are integral multiples of $h$, i.e., $\Ls_{h}:=\{\ell_{kh}\mid k\in\mathbb{N}\}$.
%  A job $\js$ is sliced by $\Ls_{h}$
% if there exists an $\ell\in\Ls_{h}$ such that $\js$ is \textit{sliced}
% by $\ell$. 



==> Arxiv submission/tree.tex <==
\section{\rufp\ on Trees}
\label{sec:roundufpontree}
\subsection{Uniform capacities}
\label{subsec:roundtreeuniform}
First, we consider the \rtree\ problem where all edges of $G_{\text{tree}}$ have the same capacity $\cs$. Let $\Zs_L := \{\js \in J\mid d_{\js} > \cs/2 \}$ and $\Zs_S := J\setminus \Zs_L$.

For the jobs in $\Zs_L$, any two jobs sharing at least one common edge must be placed in different \textit{tree-rounds}. Thus the problem reduces to the \pcolor\ problem on trees and we have the following result due to Erlebach and Jansen \cite{erlebach2001complexity} (for asymptotic approximation ratio) and Raghavan and Upfal \cite{raghavan1994efficient} (for absolute approximation ratio).

%\begin{lemma}
%\label{lemma:almostopt}
%\cite{erlebach2001complexity} There exists a polynomial-time algorithm that packs $\Zs_L$ into at most $11 \cdot \opt_{URT}/10 + 8/10$ tree-rounds. 
%\end{lemma}
%\arir{This is 1.5-absolute approximation, attained when OPT=2}

\begin{lemma}
\label{lemma:almostopt}
There exists a polynomial time asymptotic (resp. absolute) 1.1- (resp. 1.5-) approximation algorithm for packing jobs in $\Zs_L$.
\end{lemma}

Now we consider packing of jobs in  $\Zs_S$.  First, we fix any vertex $v_{\text{root}}$ as the root of $G_{\text{tree}}$. For any $\js \in J$, let $\theta_{\js}$ denote the least common ancestor of $v_{s_{\js}}$ and $v_{t_{\js}}$. For any two vertices $u,v \in V(G_{\text{tree}})$, let $P_{u-v}$ denote the unique path starting at $u$ and ending at $v$. The \textit{level} of a vertex $v\in G_{\text{tree}}$ is defined as the number of edges present in $P_{v_{\text{root}}-v}$. We sort the jobs in $\Zs_S$ in non-decreasing order of the levels of $\theta_{\js}$ and apply the \ff\ algorithm, i.e., we assign $\js$ to the first tree-round in which it can be placed without violating the edge-capacities. Let $\Gamma$ denote the set of tree-rounds used.

\begin{lemma}
\label{lemma:badfactorfour}
$|\Gamma| \le 4r$.
\end{lemma}
\begin{proof}
For any job $\js$, let $e^{1}_{\js}$ and $e^{2}_{\js}$ denote the first edges on the paths $P_{\theta_{\js}-v_{s_{\js}}}$ and $P_{\theta_{\js}-v_{t_{\js}}}$, respectively. For any tree-round $\Rs \in \Gamma$ and edge $e\in E(G_{\text{tree}})$, let $l^{\Rs}_e$ denote the sum of demands of all jobs assigned to $\Rs$ that pass through $e$.  

Let $\Rs^1, \Rs^2, \ldots \Rs^{|\Gamma|}$ be the tree-rounds used to pack $\Zs_S$. Observe that only $l^{\Rs^i}_{e^{1}_{\js}}$ and $l^{\Rs^i}_{e^{2}_{\js}}$, $\forall 1\le i \le |\Gamma|$, need to be considered while determining the tree-round for $\js$, as we are considering jobs in $\Zs_S$ in non-decreasing order of the levels of $\theta_{\js}$.
Let $\js_{\text{f}}$ be the first job for which $\Rs^{|\Gamma|}$ is opened for the first time. Clearly then at least one of $l^{\Rs^i}_{e^{1}_{\js_{\text{f}}}}$ or $l^{\Rs^i}_{e^{2}_{\js_{\text{f}}}}$ must exceed $\cs/2$, $\forall i = 1,2,\ldots,|\Gamma|-1$. Thus $\frac{\cs}{2} < l^{\Rs^i}_{e^{1}_{\js_{\text{f}}}} + l^{\Rs^i}_{e^{2}_{\js_{\text{f}}}}$. Summing over all $i$ from 1 to $|\Gamma| -1$, we get $\frac{\cs}{2}(|\Gamma| -1) < l_{e^{1}_{\js_{\text{f}}}} + l_{e^{2}_{\js_{\text{f}}}} \le 2L$. Thus, $|\Gamma| < 4r+1$. Since. $|\Gamma|$ is an integer, we get $|\Gamma| \le 4r$.     
\end{proof}

Combining \Cref{lemma:almostopt} and \Cref{lemma:badfactorfour}, we have the following theorem.

\begin{theorem}
There exists a polynomial-time asymptotic (resp. absolute) 5.1- (resp. 5.5-) approximation algorithm for \rtree~with uniform edge capacities.
\end{theorem}
%\arir{5.9 absolute approximation?}

\subsection{Arbitrary capacities (under NBA)}
\label{subsec:roundtreearbi}
We now consider the \rtree\ problem. Chekuri et al.~\cite{ChekuriMS07}  proved the following result.

\begin{theorem}
\label{theorem:Chekuristheorem}
\cite{ChekuriMS07} If all job demands are equal to 1, then they can be packed into at most $4r$ \textit{tree-rounds}.
\end{theorem}

We state the following result which enables us to obtain an improved approximation algorithm.

\begin{lemma}
\label{lemma:treelemma}
Let $\Hs := \{\js \in J\mid \frac{1}{\eta_1}c_{\min} < d_{\js} \le \frac{1}{\eta_2}c_{\min}\}$, for some $\eta_1 > \eta_2 \ge 1$. Then there exists a valid \rtree\ packing of $\Hs$ using less than $\frac{4\eta_1(\eta_2 +1)}{\eta^{2}_2}r + 4$ tree-rounds.
\end{lemma}
\begin{proof}
We scale up the demand of each job in $\Hs$ to $\frac{1}{\eta_2}c_{\min}$ and scale down the capacity of each edge in $E$ to the nearest integral multiple of $\frac{1}{\eta_2}c_{\min}$. Let $\Hs'$ denote the new set of identical demand (of $\frac{1}{\eta_2}c_{\min}$) jobs and let $I' = (c'_{e_1},\ldots,c'_{e_m})$ denote the new profile. For $e\in E$, let $l^{\Hs}_e$ and $r^{\Hs}_e$ denote the original load and congestion of edge $e$ due to the jobs in $\Hs$ and let $l^{\Hs'}_e$ and $r^{\Hs'}_e$ denote the new load and congestion, respectively. Then $l^{\Hs'}_e < \frac{\eta_1}{\eta_2}l^{\Hs}_e$ and $c'_e \ge \frac{\eta_2}{\eta_2 + 1}c_e$. Thus $r^{\Hs'}_e = \left \lceil \frac{l^{\Hs'}_e}{c'_e} \right \rceil \le \left \lceil \frac{\frac{\eta_1}{\eta_2}l^{\Hs}_e}{\frac{\eta_2}{\eta_2 + 1}c_e} \right \rceil < \frac{\eta_1 (\eta_2 + 1)}{\eta^2_2}\frac{l^{\Hs}}{c_e}+1 \le \frac{\eta_1 (\eta_2 + 1)}{\eta^2_2}r^{\Hs}_e + 1$.

Finally, we scale all demands and edge capacities by $\frac{1}{\eta_2}c_{\min}$ so that now all jobs have unit demands and all capacities are integers. Applying \Cref{theorem:Chekuristheorem} to this set of jobs, we obtain the number of tree-rounds used is at most $4r^{\Hs'} < \frac{4\eta_1(\eta_2 +1)}{\eta^{2}_2}r + 4$.
\end{proof}

Let $\Js_L := \{\js \in J\mid d_{\js} > \mathfrak{b}_{\js}/5\}$ and $\Js_s := J\setminus \Js_L$.

\begin{lemma}
\label{lemma:31approx}
The jobs in $\Js_L$ can be packed into at most $31r+6$ \textit{tree-rounds}.
\end{lemma}
\begin{proof}
Let $\Qs_M := \{\js \in \Js_L \mid \frac{1}{5}c_{\min} < d_{\js} \le \frac{1}{2}c_{\min}\}$ and $\Qs_L := \Js_L \setminus \Qs_M$. Apply \Cref{lemma:treelemma} to $\Qs_M$ with $\eta_1 = 5$ and $\eta_2 = 2$ and to $\Qs_L$ with $\eta_1 = 2$ and $\eta_2 = 1$. This yields valid packings of $\Qs_M$ and $\Qs_L$ using at most $15r+3$ and $16r+3$ tree-rounds, respectively (since the number of rounds is an integer and \Cref{lemma:treelemma} is strict). Thus the total number of tree-rounds used $\le 31r + 6$.
\end{proof}

\begin{lemma}
\label{lemma:18approx}
The jobs in $\Js_S$ can be packed into at most $18r$ \textit{tree-rounds}.
\end{lemma}
\begin{proof}
First, we introduce some terminologies. An edge $e\in E(G_{\text{tree}})$ is said to be of \textit{class} $k$ if $(5/2)^k \le c_e < (5/2)^{(k+1)}$ and we denote $\text{cl}(e):=k$. For any $u,v \in V(G_{\text{tree}})$, the \textit{critical edge} of $P_{u-v}$, denoted by $\text{crit}(P_{u-v})$ is defined as the first edge having the minimum class among all the edges of $P_{u-v}$. 

We again fix any vertex ($v_{\text{root}}$) as the root of $G_{\text{tree}}$.
As previously, for any $\js \in J$, let $\theta_{\js}$ denote the least common ancestor of $v_{s_{\js}}$ and $v_{t_{\js}}$.
 We maintain $18r$ tree-rounds, $\Rs^1, \Rs^2,\ldots,\Rs^{18r}$. For any job $\js \in \Js_S$, let $e_{\js}^1 := \text{crit}(P_{\theta_{\js}-v_{s_{\js}}})$ and $e_{\js}^2 := \text{crit}(P_{\theta_{\js}-v_{t_{\js}}})$. We consider the jobs in $\Js_S$ in non-decreasing order of the levels of $\theta_{\js}$ and place $\js$ in a tree-round $\Rs$ in which both the following conditions hold:
\begin{enumerate}[(i)]
\item The sum of demands of all jobs that have already been assigned to $\Rs$ and pass through $e_{\js}^{1}$ is at most $c_{e_{\js}^{1}}/9$.
\item The sum of demands of all jobs that have already been assigned to $\Rs$ and pass through $e_{\js}^{2}$ is at most $c_{e_{\js}^{2}}/9$. 
\end{enumerate}

First, we show that such a tree-round must always exist. Suppose to the contrary, there exists a job $\js$ that cannot be assigned by the above algorithm. Then in each of the $18r$ tree-rounds, either (i) or (ii) must fail. For any tree-round $\Rs$ and edge $e\in E(G_{\text{tree}})$, let $l_{e}^{\Rs}$ denote the sum of demands of jobs assigned to $\Rs$ that pass through $e$. Let $\chi$ be the number of tree-rounds in which $l_{e_{\js}^1}^{\Rs^i} > \frac{1}{9}c_{e_{\js}^1}$. Thus in at least $18r-\chi$ tree-rounds, $l_{e_{\js}^2}^{\Rs^i} > \frac{1}{9}c_{e_{\js}^2}$. So $l_{e_{\js}^1} \ge \sum \limits_{i=1}^{18r}l_{e_{\js}^1}^{\Rs^i} > \chi\cdot \frac{1}{9}c_{e_{\js}^1}$. Since $r \ge l_{e_{\js}^1}/c_{e_{\js}^1}$, we get $\chi < 9r$. Again $l_{e_{\js}^2} \ge \sum \limits_{i=1}^{18r}l_{e_{\js}^2}^{\Rs^i} > (18r-\chi)\cdot \frac{1}{9}c_{e_{\js}^2}$ and since $r \ge l_{e_{\js}^2} /c_{e_{\js}^2}$, we get $\chi > 9r$, a contradiction.

Now we show that the above algorithm produces a valid packing. Consider any tree-round $\Rs$ and edge $e = \{u,v\}$, such that $\text{level}(v)=\text{level}(u)+1$. Let $\Ss_e^{\Rs}$ denote the set of jobs assigned to $\Rs$ that pass through $e$. Let $\js_{\text{up}} \in \Ss_e^{\Rs}$ be the last job such that at least one of $e_{j_{\text{up}}}^{1}$ or $e_{j_{\text{up}}}^{2}$ lies on $P_{v_{\text{root}}-v}$. Thus the sum of demands of all such jobs such that at least one of $e_{j_{\text{up}}}^{1}$ or $e_{j_{\text{up}}}^{2}$ lies on $P_{v_{\text{root}}-v}$, including $\js_{\text{up}}$, is at most \[\frac{(5/2)^{\text{cl}(e)+1}}{9} + \frac{c_e}{5} \le \frac{43}{90}c_e.\]
       
All the remaining jobs must satisfy $\text{level}(\theta_{\js}) > \text{level}(u)$. 
So the critical edge is of lower level. 
Thus the sum of demands of all such jobs is at most \[\sum \limits_{i=0}^{\text{cl}(e)-1} \Big (\frac{(5/2)^{i+1}}{9} + \frac{(5/2)^{i+1}}{5}\Big ) \le \frac{14}{45}\sum \limits_{i=0}^{\text{cl}(e)-1} (5/2)^{i+1} \le \frac{14}{27}c_e.\]
    
Since ${43}/{90} + {14}/{27} < 1$, the total sum of demands of jobs in $\Ss_e^{\Rs}$ does not exceed $c_e$. Hence, the packing is valid.
\end{proof}

%Combining \Cref{lemma:31approx} and \Cref{lemma:18approx}, we have the following theorem.
Note that \Cref{lemma:31approx} yields a packing of $\Js_L$ using at most $31r+6 \le 37r$ tree-rounds. Together with \Cref{lemma:18approx}, we have the following theorem.

\begin{theorem}
There exists a polynomial time asymptotic (resp. absolute) 49- (resp. 55-) approximation algorithm for \rtree.
\end{theorem}
%\arir{absolute 57-approximtion?}

%\begin{theorem}
%There exists a polynomial time exact 55-approximation algorithm for \rtree.
%\end{theorem}

We note that with some careful choice of parameters, the asymptotic approximation ratio could be improved to 48.292, but it is unlikely to be improved further using the present technique.


==> Arxiv submission/uniform.tex <==
\section{Algorithms for Uniform Capacity Case}

\label{sec:Uniform_capacity} In this section, we provide asymptotic
$(2+\eps)$-approximation for \rsap\ and \rufp\ for the case of
uniform edge capacities. %
\begin{comment}
We will use the following few results related to DSA.

\begin{theorem} \label{theorem:dynamicProgramming} \cite{Gergov99}
There exists an algorithm for DSA that returns a feasible packing
with makespan at most $3L$. \end{theorem}

%\begin{theorem}
%\label{theorem:constantHeights}
%\cite{BuchsbaumKKRT03} For any $\eps > 0$, there is an algorithm that  (i)  if $L = O_{\eps}(1)$ then returns the optimal DSA solution (using dynamic programming), or (ii) it produces a feasible solution with makespan at most $(1+15\eps)L$ such that no job is sliced by $\Ls_{H}$, for some integer $H = O(d_{\max}/\eps)$. 
%\end{theorem}

%\subsection{Uniform capacity and arbitrary demands}
%\label{sec:Uniform_capacity_arbitrary}
Next we prove the following result for uniform capacity and arbitrary
demands.
\end{comment}
We distinguish two cases, depending on the value of $d_{\max} := \max_{\js \in J} d_{\js}$ compared to $L$.

\subsection{Case 1: $d_{\max}\le\eps^{7}L$.\label{subsubsec:easysubsec}}

First, we invoke an algorithm from \cite{BuchsbaumKKRT03} for the
dynamic storage allocation (DSA) problem. Recall that in DSA 
the input consists of a set of jobs like in \rsap\ and \rufp, but
without upper bounds of the edge capacities. Instead, we seek
to define a height $h_{\js}$ for each job $\js$ such that the resulting
rectangles for the jobs are non-overlapping and the \emph{makespan}
$\max_{\js} (h_{\js}+d_{\js})$ is minimized. The maximum load $L$ is
defined as in our setting. 

We invoke the following theorem on our input jobs $J$ with $\delta:=\eps$.

\begin{theorem} [\cite{BuchsbaumKKRT03}]\label{theorem:thorrup}
Assume that we are given a set of jobs $J'$ such that $d_{\js}\le\delta^{7}L$
for each job $\js\in J'$. Then there exists an algorithm that produces
a DSA packing of $J'$ with makespan at most $(1+\kappa \delta)L$, where $\kappa >0$ is some global constant independent of $\delta$. \end{theorem}

Let $\xi$ denote the makespan of the resulting solution to DSA and
let $\cs$ denote the (uniform) edge capacity. 
For each $h\in \mathbb{R}$, we define the horizontal line $\ell_h:=\mathbb{R}\times\{h\}$. 
A job $\js$ is said to be \textit{sliced} by $\ell_{h}$ if for the computed packing
of the jobs it holds that
$h_{\js}<h<h_{\js}+d_{\js}$.
Now we will transform this into \rsap~or \rufp~packing. 
% (we will use this for \rsap\ and DSA packings).

We define a set of
rounds $\Gamma_{1}$. The set $\Gamma_{1}$ contains a round for each integer $i$
with $0\le i\le\lfloor\xi/\cs\rfloor$ and this round contains all
jobs lying between $\ell_{i\cs}$ and $\ell_{(i+1)\cs}$. Thus, 
$|\Gamma_{1}|\le\lfloor(1+\kappa\eps)L/\cs)\rfloor+1\le(1+\kappa\eps)r+1$.
There are two subcases.

{\em Subcase A: Assume that $r > {1}/{(2\kappa \eps)}$}. In this case $|\Gamma_1| \le (1+3\kappa\eps)r$. We define a set of rounds $\Gamma_{2}$ as follows. 
For each
integer $i$ with $1\le i\le\lfloor\xi/\cs\rfloor$,  $\Gamma_{2}$ has a round containing
all jobs that are sliced by $\ell_{i\cs}$. Thus $|\Gamma_2|\le \lfloor (1+\kappa \eps)L/c^* \rfloor \le (1+\kappa\eps)r$. Hence, the total number of rounds is bounded by $(2+4\kappa\eps)r \le (2+O(\eps))\opt_{UFP}\le (2+O(\eps))\opt_{SAP}$.

{\em Subcase B: Assume that $r\le {1}/{(2\kappa \eps)}$}. Now $\xi \le (1+\kappa\eps)L$, and therefore $\xi -L \le \kappa\eps L \le c^*/2$. Hence, we have $|\Gamma_1|\le r+1$ and the $(r+1)^{\text{th}}$ round is filled up to a capacity of at most $c^*/2$ on each edge. Now the total load of the set of jobs that are sliced by $(\ell_{ic^*})_{1\le i\le r}$ is at most $r\cdot \eps^7L$. We now invoke the following result on DSA to this set of jobs.

\begin{theorem}[\cite{Gergov99}]\label{thm:gergov'sdsaresult}
Let $J'$ be a set of jobs with load $L$. Then a DSA packing of $J'$ of makespan at most $3L$ can be computed in polynomial time.
\end{theorem}

Thus the makespan of the computed solution is at most $3r\cdot \eps^7L \le 3\cdot \frac{1}{2\kappa\eps}\cdot \eps^7\cdot \frac{c^*}{2\kappa\eps}\le c^*/2$, if $\eps$ is small enough. Hence these jobs can added to the $(r+1)^{\text{th}}$ round of $\Gamma_1$. Therefore, we get a packing of $J$ using at most $r+1\le \opt_{UFP}+1\le \opt_{SAP}+1$ rounds.
%Similarly, $|\Gamma_{2}|\le(1+O(\eps))r$.
%Hence the total number of rounds is bounded by $(2+O(\eps))r+1 \le (2+O(\eps))OPT_{UFP}+1\le (2+O(\eps))OPT_{SAP}+1$.

%\arir{added 2.5 and 3 absolute algos for UFP and SAP}

\begin{comment}
\begin{algorithm}
Apply \Cref{theorem:thorrup} to $J$ with $\delta=\eps$ to obtain
a DSA packing with makespan $\xi$.\\
 For each $0\le i\le\lfloor\xi/\cs\rfloor$, open a round $\Rs_{1}^{i}$
and pack the jobs completely lying between $\ell_{i\cs}$ and $\ell_{(i+1)\cs}$
into $\Rs_{1}^{i}$.\\
 For each $1\le i\le\lfloor\xi/\cs\rfloor$, open a round $\Rs_{2}^{i}$
and pack the jobs sliced by $\ell_{i\cs}$ into it. \caption{}
\label{algo:UniformRoundSapArbitrary_new} 
\end{algorithm}
\end{comment}


\subsection{Case 2: $d_{\max}>\eps^{7}L$\label{subsubsec:hardsubsubsec} }

%\ari{Observe that in this case in particular $\cs\ge d_{\max}>\eps^{7}L$
%and one can show that $OPT_{UFP}\le OPT_{SAP}\le O(1/\eps^7)$ (even though we do
%not use this fact directly).} \arir{may not be correct}
For this case, we have $c^* \ge d_{\max}> \eps^7 L$ and therefore $r = \lceil L/c^* \rceil \le 1/\eps^7$. We partition the input jobs into \emph{large }and \emph{small} jobs
by defining $J_{\mathrm{large}}:=\{\js\in J|d_{\js}>\eps^{56}L\}$
and $J_{\mathrm{small}}:=\{\js\in J|d_{\js}\le\eps^{56}L\}$. 

%For these sets, we will compute solutions with at most $(1+\eps)OPT+O(1)$ rounds each, leading to a solution with $(2+\eps)OPT+O(1)$ rounds in total.

We start with the small jobs $J_{\mathrm{small}}$. First, we apply
Theorem~\ref{theorem:thorrup} to them with $\delta:=\eps^{56}$ and
obtain a DSA packing $\Ps$ for them. We transform it into a solution
to \rsap\ with at most $r+1$ rounds as follows: we introduce a set $\Gamma_1$ consisting of $r+1$ rounds exactly as in the previous case (when $r\le {1}/{(2\kappa \eps)}$). The $(r+1)^{\text{th}}$ round would be filled up to a capacity of at most $\kappa\eps^8 L \le \kappa\eps c^*$. Again applying \Cref{thm:gergov'sdsaresult} to the remaining jobs, we get a DSA packing of makespan at most $3r \cdot \eps^{56}L \le 3\cdot ({1}/{\eps^7})\cdot \eps^{56}\cdot ({c^*}/{\eps^7})\le c^*/2$, and therefore these jobs can be packed inside the $(r+1)^{\mathrm{th}}$ round. Hence, there exists a packing of $J_{\text{small}}$ using at most $r+1\le \opt_{UFP}+1\le \opt_{SAP}+1$ rounds.


\begin{comment}
first, we define the rounds $\Gamma_{1}$ and $\Gamma_{2}$ exacty
as above. Since our jobs are very small, we argue that we can combine
any set of $1/\eps$ rounds from $\Gamma_{2}$ to a single round,
and hence all jobs packed in the rounds $\Gamma_{2}$ can be packed
in $O(\eps)r$ rounds in total. This yields $(1+O(\eps))r+2$
rounds overall for the small jobs $J_{\mathrm{small}}$.

\begin{lemma} \label{lemma:sidelemma} We are given a DSA packing $\Ps$
with makespan $\xi$ for a set of jobs $\bar{J}\subseteq J$ such
that $d_{\js}\le\eps\cs$ for each $\js\in\bar{J}.$ Then
we can compute a valid \rsap\ packing of $\bar{J}$ using at most
$(1+O(\eps))r+2$ rounds with (uniform) edge capacity $\cs$.
\end{lemma}
\arir{add proof in appendix}
\end{comment}

Now we consider the large jobs $J_{\mathrm{large}}$. Our strategy
is to compute an optimal solution for them via dynamic programming
(DP). Intuitively, our DP orders the jobs in $J_{\mathrm{large}}$
non-decreasingly by their respective source vertices and assigns them
to the rounds in this order. Since the jobs are large, each edge is
used by at most $1/\eps^{56}$ large jobs, and using interval coloring one can
show easily that at most $1/\eps^{56}=O_{\eps}(1)$ rounds
suffice (e.g., we can color the jobs with $1/\eps^{56}$ colors such that 
no two jobs with intersecting paths have the same color). 
In our DP we have a cell for each combination of an edge $e$ and the assignment
of all jobs passing through $e$ to the rounds. Given this, the corresponding subproblem is to assign additionally 
all jobs to the rounds whose paths lie completely on the right of $e$.
% Using this, we can ensure that for our DP a polynomial number of DP-cells are sufficient.

For \rsap\ we additionally want to bound the number of
possible heights $h_{\js}$. To this end, we restrict ourselves to
packings that are normalized which intuitively means that all jobs
are pushed up as much as possible. Formally, we say that a packing
for a set of jobs $J'$ inside a round is \textit{normalized} if for every $\js\in J'$,
either $h_{\js}+d_{\js}=\cs$ or $h_{\js}+d_{\js}=h_{\js'}$ for some
$\js'\in J'$ such that $P_{\js}\cap P_{\js'}\neq\emptyset$ (see \Cref{fig:chain} in \Cref{sec:normalizedpacking}). 

\begin{lemma}
\label{lem:normal}
Consider a valid packing of a set of jobs $J'\subseteq J_{\mathrm{large}}$
inside one round. Then there is also a packing for $J'$ that is normalized.
\end{lemma}
%\arir{removed proof and figure to Appendix.}


Now the important insight is that in a normalized packing of large
jobs, the height $h_{\js}$ of a job $\js$ is the difference of (the
top height level) $\cs$ and the sum of at most $1/\eps^{56}$
jobs in $J_{\mathrm{large}}$. Thus, the number of possible heights
is bounded by $n^{O(1/\eps^{56})}$ and we can compute all these
possible heights before starting our DP. 
\begin{lemma}
\label{lemma:heights}Given $J_{\mathrm{large}}$ we can compute a set $\mathcal{H}$ of $n^{O(1/\eps^{56})}$
values such that in any normalized packing of a set $J'\subseteq J_{\mathrm{large}}$
inside one round, the height $h_{\js}$ of each job $\js\in J'$ is
contained in $\mathcal{H}$.
\end{lemma}

Now we can compute the optimal packing via a dynamic program as described
above, which yields the following lemma. 

\begin{lemma} \label{lemma:maindynamicprogramming} Consider an instance
of \rufp\ or \rsap\ with a set of jobs $J'$ satisfying the following
conditions: 
\begin{enumerate}[(i)] 
\item The number of jobs using any edge is bounded by $\omega$. 
\item In the case of \rsap\ there is a given set $\mathcal{H}'$ of allowed
heights for the jobs. 
\end{enumerate}
Then we can compute an optimal solution to the given instance in time $(n|\mathcal{H}'|)^{O(\omega)}$. \end{lemma}

\begin{comment}
Any packing can be converted to a normalized packing by pushing all
jobs up as much as possible. Formally, As we will show shortly, this
greatly reduces the number of distinct job positions that need to
be considered (to polynomial).

A subset $J'':=\{\js_{1},\js_{2},\ldots,\js_{k}\}\subseteq J'$ will
be called a \textit{chain} of size $k$ if 
\begin{itemize}
\item $h_{\js_{i}}+d_{\js_{i}}=h_{\js_{i+1}}$ and $P_{\js_{i}}\cap P_{\js_{i+1}}\neq\emptyset$,
$\forall i\in\{1,2,\ldots,k-1\}$; $h_{\js_{k}}+d_{\js_{k}}=\cs$, 
\item if there exists $\js\in\Ds$ such that $h_{\js}+d_{\js}=h_{\js_{1}}$,
then $P_{\js}\cap P_{\js_{1}}=\emptyset$. 
\end{itemize}
Intuitively, a set of jobs form a chain if each job touches the bottom
of the next job over at least one edge (see Fig. \ref{fig:chain}
in Appendix \ref{sec:appfig}). We now present two lemmas which will
be required for our main algorithm. The omitted proofs are given in
Appendix \ref{sec:applowb}.
\end{comment}

We invoke Lemma~\ref{lemma:maindynamicprogramming} with $J':=J_{\mathrm{large}}$,
$\omega=1/\eps^{56}$, and in the case of \rsap\ we define $\mathcal{H}'$
to be the set $\mathcal{H}$ due to Lemma~\ref{lemma:heights}. This
yields at most $OPT$ rounds in total for the large jobs $J_{\mathrm{large}}$. Hence,  we obtain a packing of $J$ using at most $2\cdot \opt +1$ rounds.

\begin{comment}
\begin{lemma} \label{lemma:mainDP} Let $\mathcal{W}\subseteq J$
be a set of jobs such that $d_{\js}\ge3\delta L$, $\forall\js\in\mathcal{W}$,
for some $\delta>0$. Then the optimal number of rounds required to
pack all jobs in $\mathcal{W}$ can be found in $n^{O(1/\delta^{2})}$
time. \end{lemma} 
\begin{proof}
Let $OPT_{\Ws}$ be the optimal number of rounds required. If $L<\cs/3$,
we apply \Cref{theorem:dynamicProgramming} to get a packing of
makespan $\le3L\le\cs$. Thus $OPT_{\Ws}=1$ in this case. Henceforth
we assume that $L\ge\cs/3$ so that all demands are $\ge\delta\cs$.
Thus in any round, maximum possible size of a chain is $1/\delta$.

Consider any job $\js\in\Ws$. Total number of possible chains that
$\js$ can be a part of including its position in the chain is at
most $\sum_{i=1}^{1/\delta}{|\Ws| \choose i}i!\le\sum_{i=1}^{1/\delta}n^{i}\le(1/\delta)n^{1/\delta}$.
Considering only normalized packings, this is the maximum possible
number of values that $h_{\js}$ can take (if we had allowed arbitrary
packings, $h_{\js}$ could have taken $\Omega(\cs)$ many values,
which can be exponential). Also since the demand of each job is at
least $3\delta L$, the number of jobs passing through any edge is
bounded by $1/(3\delta)$.

We apply \Cref{lemma:maindynamicprogramming} to $\mathcal{W}$
with $\omega=1/(3\delta)$ and $U=(1/\delta)n^{1/\delta}$. Thus the
running time is bounded by $(n\cdot(1/\delta)n^{1/\delta})^{1/(3\delta)}=n^{O(1/\delta^{2})}$. 
\end{proof}
\end{comment}

%\textbf{If} $d_{\max} \le \eps^7 L$, apply \Cref{theorem:thorrup} to get a feasible DSA packing $\Ps$.\\
%Pack jobs in $J \setminus J^{\Ps}_{\Ls_{c}}$ lying between consecutive slicing lines into separate rounds.\\ 
%For each $\ell \in \Ls_c$, pack all jobs sliced by $\ell$ into separate rounds and halt.\\
\iffalse
\begin{algorithm}
Let $J_{\mathrm{large}}:=\{\js\in J|d_{\js}>\eps^{8}L\}$ and
$J_{\mathrm{small}}:=\{\js\in J|d_{\js}\le\eps^{8}L\}$\\
Apply \Cref{theorem:thorrup} to $J_{\mathrm{small}}$ with $\delta=\eps$
to obtain a DSA packing $\Ps$.\\
 Apply \Cref{lemma:sidelemma} to $\Ps$ %Pack jobs in $\Ys \setminus \Ys^{\Ps_1}_{\Ls_{c}}$ lying between consecutive slicing lines into separate rounds.\\
%Apply \Cref{theorem:dynamicProgramming} to $\Ys^{\Ps_1}_{\Ls_{c}}$. Let $\Ps_2$ be the packing generated.\\
\\
Apply \Cref{lemma:heights} to compute the set $\mathcal{H}$ 

Apply \Cref{lemma:maindynamicprogramming} to $J_{\mathrm{large}}$
with $\omega=1/\eps^{8}$ and $\mathcal{H}':=\mathcal{H}$ \\
 %Pack the jobs in $\Ys^{\Ps_1}_{\Ls_{c}} \setminus \Ys^{\Ps_2}_{\Ls_{c}}$ lying between consecutive slicing lines into separate rounds.\\
%For each slicing line $\ell \in \Ls_{c}$, pack the jobs in $\Ys^{\Ps_2}_{\Ls_{c}}$ sliced by $\ell$ in packing $\Ps_2$ into separate rounds. 
\caption{}
\label{algo:UniformRoundSapArbitrary} 
\end{algorithm}
\fi

%\begin{lemma}
%\label{lemma:approxroundSAP}
%\Cref{algo:UniformRoundSapArbitrary} packs the jobs into at most $(2+O(\eps))OPT_{URS} + 2$ rounds.
%\end{lemma}
%\begin{proof}
%If $d_{\max} \le \eps^7L$, from \Cref{theorem:thorrup}, the makespan of $\Ps$ is at most $(1+O(\eps))L$. Thus total number of rounds used in step 2 and 3 is bounded by $\lceil(1+O(\eps))L/c\rceil + \lfloor(1+O(\eps))L/c\rfloor \le (2+O(\eps))OPT_{URS} + 1$.\par
%Otherwise $c \ge d_{\max} > \mu ^6L$. Step 5 produces the optimal solution for the jobs in $\Xs$. Again by \Cref{theorem:thorrup}, the number of rounds used in step 7 is at most $\lceil(1+O(\mu))L/c\rceil$. Now maximum possible load on any edge in $\Ps_1$ is $\mu^{7}L \lfloor(1+O(\mu))L/c\rfloor \le \mu (1+O(\mu))L \le 2\mu L$ for sufficiently small $\mu$. Thus makespan of $\Ps_2$ is at most $6\mu L$. So number of additional rounds used in steps 9 and 10 is $\le \lceil 6\mu L/c\rceil + \lfloor 6\mu L/c\rfloor \le 12\mu L/c + 1$. Hence the total number of rounds required to pack all jobs in $\Ys$ is $\le (1+O(\eps))L/c + 2$ (as $\mu \le \eps$). Together with the rounds used in step 5, we see that the given claim holds.   
%\end{proof}

% \textbf{}%
\begin{comment}
\textbf{Analysis:} Step 2 produces the optimal solution for the jobs
in $\Xs$. Since all jobs in $\Ys$ have demand at most $\mu^{7}L$,
the makespan of the packing $\Ps$ produced in Step 3 is bounded by
$(1+O(\mu))L$, due to \Cref{theorem:thorrup}. Also note that here
$\vartheta=\mu^{6}L=\eps^{7}L<d_{\max}\le\cs$. Thus step 4 yields
a packing using at most $(1+O(\mu))r+2\le(1+O(\eps))\opt_{URS}+2$
rounds (as $\mu=\eps^{7/6}\le\eps$). Together with the rounds used
in step 2, we see that \Cref{theorem:twoasymptoticapprox} holds.

%Till now we were dealing with \ursap. We note that the dynamic programming algorithm presented in the proof of \Cref{lemma:mainDP} can be modified to work for \urufp\ as well. Here the vertical positions of the jobs inside any round does not matter. So we simply have a 2-cell DP, where each DP cell is defined by an edge $e\in E$ and a function $f_e$ that allocates the jobs passing through edge $e$ to the rounds. \Cref{algo:UniformRoundSapArbitrary} can be modified accordingly. Thus we have the following theorem. 
%\begin{theorem}
%\label{theorem:uniformroundsapandufp}
%For any $\eps > 0$, there exist asymptotic $(2+\eps)$-approximation algorithms for \ursap\ and \urufp.
%\end{theorem}

Till now, we were dealing with \ursap. For \urufp, we first propose
the following result, whose proof is given in Appendix \ref{sec:applowb}.

\begin{lemma} \label{lemma:corollaryofdp} Consider an instance of
\urufp\ such that the number of jobs passing through any edge is
bounded by $\omega$. Then the optimal number of rounds required to
pack $J$ can be determined in $n^{O(\omega)}$ time. \end{lemma}

Since the positions of jobs inside the rounds do not matter in the
case of \urufp, the optimal rounds required to pack $\Ws$ (as defined
in \Cref{lemma:mainDP}) can be determined in $n^{O(1/\delta)}$
time using the above lemma. Thus the algorithm is same as \Cref{algo:UniformRoundSapArbitrary}:
we find the optimal solution for $\Xs$ and a valid \urufp\ packing
for $\Ys$ using at most $(1+O(\eps))\opt_{URU}+2$ rounds. 
\end{comment}

Case 1 and 2 together yields our main theorem for the case of uniform edge capacities.

\begin{theorem} \label{theorem:twoasymptoticapprox} For any $\eps>0$,
there exist asymptotic $(2+\eps)$-approximation algorithms for \rsap\ and
\rufp, assuming uniform edge capacities. \end{theorem}

We now derive some bounds on the absolute approximation ratios. If $\opt_{SAP}= 1$, our algorithm would return a packing using at most $(2+\eps)\cdot 1 + 1$ rounds, and hence at most 3 rounds. If $\opt_{SAP}\ge 2$, then our algorithm uses at most $(2+\eps)\cdot OPT_{SAP}+ OPT_{SAP}/2 = (2.5+\eps)OPT_{SAP}$ rounds. Hence, we obain the following result.

\begin{theorem}
\label{thm:unisapabs}
There exists a polynomial time $3$-approximation algorithm for \rsap, assuming uniform edge capacities.
\end{theorem}

For \rufp, it is easy to check whether $\opt_{UFP}=1$ by checking whether $L \le c^*$. Otherwise, $\opt_{UFP}\ge 2$ and similar as above, the number of rounds used would be at most $(2.5+\eps)\cdot OPT_{UFP}$. This gives an improvement over the result of Pal \cite{pal2014approximation}.

\begin{theorem}
For any $\eps >0$, there exists a polynomial time $(2.5+\eps)$-approximation algorithm for \rufp, assuming uniform edge capacities.
\end{theorem}

\iffalse
Finally, we obtain APTASes if the maximum job demand is bounded by
a constant, see Appendix \ref{sec:Constant_Job_Heights} for the proof
of Theorem \ref{theorem:APTASforconstant}.

\begin{theorem} \label{theorem:APTASforconstant} There exist APTASes
for \rsap\ and \rufp\ when the maximum demand $d_{\max}$ is
constant and the edge capacities are uniform. \end{theorem}
\fi



==> Arxiv submission/uniform_new.tex <==
\section{Improved algorithms for uniform capacity case}
We repeatedly use the following results on DSA.

\begin{theorem}
\cite{BuchsbaumKKRT03}
\label{thm:dsamaintheorem}
If $d_{\max}\le \delta^7 L$, there exists a feasible solution to DSA with makespan at most $(1+\alpha \delta)L$, for some constant $\alpha > 0$.
\end{theorem}

\begin{theorem}
\cite{Gergov99}
\label{thm:dsagergovthm}
Given a set of jobs with load $L$, there exists a solution of DSA with makespan at most $3L$.
\end{theorem}

Now we divide our algorithm into 2 cases depending on the values of $d_{\max}$ and $L$.

\subsection{$d_{\max}\le \epsilon^7 L$}
We further divide into two subcases depending on the value of $r$.

\subsubsection{$r > \frac{1}{2\alpha \epsilon}$}
\label{sec:largecongestion}
We first apply \Cref{thm:dsamaintheorem} to $J$ to obtain a DSA packing with makespan $\zeta \le (1+\alpha \epsilon)L$. Now we open a set of rounds $\Gamma_1$ which contains a round for each integer $i$ with $0\le i \le \lfloor \zeta/c^{*}\rfloor$ and this round contains all jobs lying between $\ell_{ic^{*}}$ and $\ell_{(i+1)c^{*}}$. Thus $|\Gamma_1| \le \left \lceil \frac{(1+\alpha \epsilon)L}{c^*}\right \rceil \le (1+\alpha \epsilon)r + 1 \le (1+3\alpha \epsilon)r$. 

Now we define a set of rounds $\Gamma_2$ as follows. For each integer $i$ with $1\le i \le \lfloor \zeta/c^{*}\rfloor$, $\Gamma_2$ has a round containing all jobs sliced by $\ell_{ic^*}$. Thus $|\Gamma_2|\le \lfloor \frac{(1+\alpha \epsilon)L}{c^*}\rfloor \le (1+\alpha \epsilon)r$. Thus the total number of rounds used is at most $(2+O(\epsilon))r$.

\begin{theorem}
If $d_{\max}\le \epsilon^7 L$ and $r > \frac{1}{2\alpha \epsilon}$, there exists a packing of $J$ using $(2+O(\epsilon))r$ rounds.
\end{theorem}

\subsubsection{$r \le \frac{1}{2\alpha \epsilon}$}
Applying \Cref{thm:dsamaintheorem} to $J$, we get a DSA packing of makespan $\zeta \le (1+\alpha \epsilon)L$. Thus $\zeta - L \le \alpha \epsilon L \le c^*/2$. As in \Cref{sec:largecongestion}, we open a set of $r+1$ rounds, where the $i^{\text{th}}$ round contains all jobs lying between $\ell_{ic^{*}}$ and $\ell_{(i+1)c^{*}}$. Now since $\zeta - L \le c^*/2$, the $(r+1)^{\text{th}}$ round is filled to a capacity of at most $c^*/2$. Now the total load of the jobs sliced by the set of slicing lines $(\ell_{ic^*})_{1\le i \le r}$ is at most $r \cdot \epsilon^7 L$. Thus by applying \Cref{thm:dsagergovthm} to these jobs, we get a DSA packing of makespan at most $3r\cdot \epsilon^7 L \le 3\cdot \frac{1}{2\alpha \epsilon}\cdot \epsilon^7 \frac{c^*}{2\alpha \epsilon} \le \epsilon c^*$, for sufficiently small $\epsilon$. Hence all these jobs can be packed into the $(r+1)^{\text{th}}$ round, which will be filled up to at most $(\frac{1}{2}+\epsilon)c^*$. Hence we get a packing of $J$ using $r+1$ rounds.

\begin{theorem}
If $d_{\max}\le \epsilon^7 L$ and $r \le \frac{1}{2\alpha \epsilon}$, there exists a packing of $J$ using $r+1$ rounds.
\end{theorem}


\subsection{$d_{\max} > \epsilon^7 L$}
In this case, we have $c^* \ge d_{\max} > \epsilon^7 L$. Thus $r = \left \lceil L/c^* \right \rceil \le 1/\epsilon^7 $. We define $J_{\text{small}} := \{\js | d_{\js}\le \epsilon^{56}L \}$ and $J_{\text{large}} := \{\js | d_{\js}> \epsilon^{56}L \}$. For jobs in $J_{\text{large}}$, the optimal packing can be found in polynomial time using DP.

Applying \Cref{thm:dsamaintheorem} to $J_{\text{small}}$, we get a packing of makespan $\zeta \le (1+\alpha \epsilon^8)L$. Thus $\zeta - L \le \alpha \epsilon^8 L \le \alpha
\epsilon c^*$. As before, we open a set of $r+1$ rounds, where the $i^{\text{th}}$ round contains all jobs lying between $\ell_{ic^{*}}$ and $\ell_{(i+1)c^{*}}$. The $(r+1)^{\text{th}}$ round will be filled up to a capacity of at most $\alpha
\epsilon c^*$. Again the total load of the jobs sliced by the set of slicing lines $(\ell_{ic^*})_{1\le i \le r}$ is at most $r \cdot \epsilon^{56}L$. Thus \Cref{thm:dsagergovthm} would give a DSA packing of makespan at most $3r\cdot \epsilon^{56}L\le 3\cdot 1/\epsilon^7 \cdot \epsilon^{56}\cdot \frac{c^*}{\epsilon^7}\le \epsilon c^*$, for sufficiently small $\epsilon$. Thus all these jobs can be packed into the $(r+1)^{\text{th}}$ round. Hence we get a packing of $J_{\text{small}}$ using $r+1$ rounds.

Together with the optimal packing of $J_{\text{large}}$, we get a packing of $J$ using at most $2\cdot OPT +1$ rounds. 

\begin{theorem}
If $d_{\max} > \epsilon^7 L$, there exists a packing of $J$ using at most $2\cdot OPT + 1$ rounds.
\end{theorem}



==> constantdemand.tex <==
\section{Uniform Capacity and Constant Job Demands}
\label{sec:Constant_Job_Heights}
In this section, we prove Theorem \ref{theorem:APTASforconstant}.

\begin{theorem}
(Restatement of Theorem \ref{theorem:APTASforconstant})
There exist APTASes for \ursap\ and \urufp\ when the maximum demand $d_{\max}$ is constant.
\end{theorem}
%\arir{constant demand can be confused with same demand.}
%\arir{c is a poor notation as we already use it for capacity function as well.}
The proof is divided into two cases, depending on the value of $d_{\max}$.

\subsection{Case 1: $d_{\max}\ge \eps \cs$.}
\label{subsec:allconstant}
Intuitively, in this case $\cs$ is also a constant and thus we can use a dynamic program to find the optimal packing in polynomial-time. First, we consider \ursap. 
Consider a valid \ursap\ packing of a subset of $J$ inside one round of the uniform capacity profile of height $\cs$. We assume w.l.o.g.~that $h_{\js}$ is an integer, for all jobs $\js$ in the packing. This can be achieved by applying "gravity" to the packing, i.e., we consider the jobs in the non-decreasing order of $h_{\js}$'s and move them downwards till they touch the top of some other job or reach the $x$-axis. We define an encoding of the sequence of jobs present over any edge. The \textit{configuration} of edge $e$ is defined as an ordered $\cs$-tuple $(\zeta_1,\zeta_2,\dots,\zeta_{\cs})$. For all $i \in \{1,2,\ldots,\cs\}$, define $\zeta_i = 0$, if no job is present between the slicing lines $\ell_{i-1}$ and $\ell_i$ over $e$; and otherwise, define $\zeta_i = d_{\js}$, where $\js$ is the job present between $\ell_{i-1}$ and $\ell_i$. Thus each $\zeta_i$ can take $d_{\max}+1$ many values. Hence the number of possible configurations of an edge is $\nu := (d_{\max}+1)^{\cs} = O_{\eps}(1)$, since $d_{\max}$ is a constant and $\cs \le d_{\max}/\eps$.

Now consider any valid \ursap\ packing of $J$ using $\lambda$ rounds $\Rs^1, \Rs^2,\ldots,\Rs^\lambda$. The \textit{joint configuration} of an edge $e$ is defined as an \textbf{unordered} $\lambda$-tuple $(C^{e}_{1},C^{e}_{2},\ldots, C^{e}_{\lambda})$, where $C^{e}_i$ denotes the configuration of $e$ in round $\Rs^i$, $\forall i \in \{1,2,\dots,\lambda\}$. Since there are $\lambda$ rounds, such a joint configuration is said to be a $\lambda$-\textit{dimensional} joint configuration. Thus the number of possible $\lambda$-dimensional joint configurations of an edge is at most $\lambda^{\nu} = \lambda^{O_{\eps}(1)}$.

We define a procedure called \checkcomp\ (see \Cref{algo:Checkcompatibility}) that takes input a valid \ursap\ packing $\Ps$ of $J^{e_{i-1}}$ using $\lambda$ rounds and a $\lambda$-dimensional joint configuration $\Cs^{e_i}$, for some $i \in \{2, 3, \dots, m\}$. \checkcomp\  returns \textbf{false} if $\Ps$ and $\Cs^{e_i}$ cannot be feasibly packed together, otherwise, it returns the feasible packing. Let the $\lambda$ rounds in $\Ps$ be $\Rs^1$, $\Rs^2$,\ldots,$\Rs^\lambda$ and let $\Cs^{e_i} = (C^{e_i}_{1},C^{e_i}_{2},\ldots, C^{e_i}_{\lambda})$. 

\begin{algorithm}[H]
For each round $\Rs^j$, create a node $u_j$, and for each configuration $C^{e_i}_{k}$, create a node $v_k$, $1\le j,k \le \lambda$.\\
Add an edge between $u_j$ and $v_k$ if configuration $C^{e_i}_{k}$ can be feasibly placed with the packing inside the round $\Rs^j$, $\forall 1\le j,k \le \lambda$. Let $\Gs$ denote the resulting bipartite graph.\\   
%Create a bipartite graph $G=L\cup R$ where $L$ consists of the $k$ rounds in $\Ps$ and $R$ consists of the $k$ configurations in $C_e$.\\
%$\forall (l,r)\in L\cup R$, add an edge between $l$ and $r$ if configuration $r$ can be feasibly packed inside round $l$.\\
Compute the maximum matching $N$ in $\Gs$.\\
If $N$ is a perfect matching, return the packing corresponding to $N$, else return \textbf{false}.
\caption{\checkcomp$(\Ps,\Cs^{e_i})$}
\label{algo:Checkcompatibility}
\end{algorithm}

Equipped with the above procedure, we now propose a dynamic programming based algorithm. First, guess the value of $\opt_{URS}$ as $\kappa$ where $1\le \kappa \le n$. A DP cell consists of 
\begin{itemize}
\item an edge $e\in E$.
\item a $\kappa$-dimensional joint configuration $\Cs^e$ of $e$.
\end{itemize}

We define DP($e,\Cs^e$)=1 if and only if there exists a valid \ursap\ packing $\Ps$ of $J^e$ such that the joint configuration of $e$ in $\Ps$ is exactly $\Cs^e$. If DP($e,\Cs^e$)=1, we also store the corresponding packing $\Ps$ in another table $\Upsilon$ in the table entry $\Upsilon(e,\Cs^e)$. For all $i \in \{2,3,\ldots, m\}$,  the recurrence for the dynamic program is given by: DP($e_i,\Cs^{e_i}$)=1 if there exists a $\Cs^{e_{i-1}}$ such that DP($e_{i-1},\Cs^{e_{i-1}}$)=1 and \checkcomp$(\Upsilon(e_{i-1},\Cs^{e_{i-1}}),\Cs^{e_i})$ returns a valid packing; otherwise, DP($e_i,\Cs^{e_i}$)=0. Clearly, the number of DP cells is polynomially bounded and each DP entry can be computed in polynomial time. 

For \urufp\, the positions of jobs inside a round do not matter. Hence the configuration of an edge $e$ can simply be encoded as a $d_{\max}$-tuple $(\zeta_1,\zeta_2,\ldots,\zeta_{d_{\max}})$, where $\forall i \in \{1,2,\ldots, d_{\max}\}$, $\zeta_i$ denotes the number of jobs having demand $i$, present over $e$ inside a round of a valid packing. Clearly, each $\zeta_i \le \cs$ and therefore the number of possible edge configurations is bounded by ${\cs}^{d_{\max}} \le O_{\eps}(1)$. The definition of a joint configuration remains the same. Procedure \checkcomp\ and the dynamic program also stay the same. Thus we have the following theorem:

\begin{theorem}
\label{theorem:optimalsolnforrsap}
For any $\eps >0$, if $d_{\max}$ is constant, and $d_{\max}\ge \eps \cs$, then the optimal number of rounds required to pack $J$ can be computed in $n^{O_{\eps}(1)}$ time.
\end{theorem}

\subsection{Case 2: $d_{\max}<\eps \cs$.}
\label{subsubsec:someconstants}
We first show the following results.

\begin{lemma}
\label{corollary:maincorollary_new}
\ursap\ and \urufp\ can be solved optimally in polynomial time if $L$ is a constant.
\end{lemma}
\begin{proof}
If $\cs > 3L$, apply \Cref{theorem:dynamicProgramming} to obtain a DSA packing with makespan at most $3L < \cs$. Thus all jobs can be packed inside one round of the uniform capacity profile and hence $\opt_{URS} = \opt_{URU} = 1$. 

Suppose now that $\cs \le 3L$. Consider \ursap\ first. Apply \Cref{lemma:maindynamicprogramming} to $J$. Since all demands are integers, at most $L$ jobs pass through any edge. Thus $\omega = L$. Also for any job $\js$, $h_{\js}$ can take at most $\cs \le 3L$ distinct values and therefore $U = 3L$. Thus the running time of the dynamic program is bounded by $(n\cdot 3L)^{O(L)}$, which is polynomial in $n$.

Similarly for \urufp\, we apply \Cref{lemma:corollaryofdp} with $\omega = L$ as before. The running time is bounded by $n^{O(L)}$.
\end{proof}

\begin{lemma}
\label{lemma:abcdef}
There exists an algorithm that 
\begin{enumerate}[(i)]
\item if $L=O_{\eps}(1)$, returns the optimal \ursap\ or \urufp\ solution,
\item else, returns a DSA packing of makespan at most $(1+15\eps )L$.
\end{enumerate}
\end{lemma}
\begin{proof}
Our algorithm is very similar to the algorithm in section 4 in \cite{BuchsbaumKKRT03}. If $L \le C\frac{1}{\eps^4}\log ^2\frac{1}{\eps}$, we apply \Cref{corollary:maincorollary_new} to get the optimal \ursap\ or \urufp\ solution. Otherwise steps 2,3,4 of the algorithm generate a DSA packing of makespan at most $(1+15\eps )L$, as proved by the authors in Theorem 4.1.
\end{proof}

Now we present our main algorithm in \Cref{algo:UniformRoundSap1}.

\begin{algorithm}[H]
%\textbf{If} $d_{\max} \ge \eps c$, apply \Cref{theorem:constantHeights} with $H = c$. Pack the jobs lying between consecutive slicing lines of $\Ls_{c}$ into separate rounds, and halt.\\
%\textbf{Else} apply \Cref{theorem:constantHeights} with $H = d_{\max}\lceil1/\eps\rceil$ to generate a DSA packing $\Ps_1$.\\
%Pack jobs in $J \setminus J^{\Ps_1}_{\Ls_{c}}$ lying between consecutive slicing lines into separate rounds.\\
%Apply \Cref{theorem:dynamicProgramming} to $J^{\Ps_1}_{\Ls_{c}}$. Let $\Ps_2$ be the packing generated.\\
%Pack jobs in $J^{\Ps_1}_{\Ls_{c}} \setminus J^{\Ps_2}_{\Ls_{c}}$ lying between consecutive slicing lines in $\Ps_2$ into separate rounds.\\
%For each slicing line $\ell \in \Ls_{c}$, pack the jobs in $J^{\Ps_2}_{\Ls_{c}}$ sliced by $\ell$ in $\Ps_2$ into separate rounds.\\
Apply \Cref{lemma:abcdef} to $J$. If it returns an optimal solution (i.e. halts in step (i)), halt.\\
Else let $\Ps$ be the DSA packing returned. Apply \Cref{lemma:sidelemma} to $\Ps$ with parameters $\delta = \eps$ and $\vartheta=\cs$.    
\caption{}
\label{algo:UniformRoundSap1}
\end{algorithm}

\textbf{Analysis:} If the algorithm halts in step 1, we get an optimal solution for \ursap\ or \urufp. Otherwise, from \Cref{lemma:abcdef}, the makespan of $\Ps$ is at most $(1+15\eps)L$. Thus \Cref{lemma:sidelemma} implies the number of rounds used in step 2 is bounded by $(1+O(\eps))r+2$. Note that any valid \ursap\ packing is also a valid \urufp\ packing. Since $r$ is a lower bound for both $\opt_{URS}$ and $\opt_{URU}$, \Cref{theorem:APTASforconstant} holds.  





==> general.tex <==
\section{General case}

We present our $O(\log\log n)$-approximation algorithms for the general cases of \rufp and \rsap.

We consider \rufp\ first and describe later how to extend our algorithm
to \rsap. We split the input jobs into large and small
jobs. We define $J_{\mathrm{large}}:=\{\js\in J|d_{\js}>b_{\js}/4\}$
and $J_{\mathrm{small}}:=\{\js\in J|d_{\js}\le b_{\js}/4\}$.
For the small jobs, we invoke a result by Elbassioni et al. \cite{ElbassioniGGKN12}
that yields a 16-approximation.
\begin{theorem}[\cite{ElbassioniGGKN12}]
\label{thm:Elbassioni-small} Given an instance of \rufp\ with
a set of jobs $J'$ such that $d_{\js}\le\frac{1}{4}b_{\js}$ for
each job $\js\in J'$. There is a polynomial time algorithm that computes
a 16-approximate solution to $J'$. 
\end{theorem}

Now consider the large jobs $J_{\mathrm{large}}$. For each job $\js\in J_{\mathrm{large}}$, 
we define a rectangle $R_{\js}=(s_{\js},b_{\js}-d_{\js})\times(t_{\js},b_{\js})$.
Note that $R_{\js}$ corresponds to the rectangle for $\js$ in \rsap
if we assign $\js$ the maximum possible height $h_{\js}$ (which is $h_{\js}:=b_{\js}-d_{\js}$). We say
that a set of jobs $J'\subseteq J_{\mathrm{large}}$ is \emph{top-drawn}
(underneath the capacity profile), if their rectangles are pairwise
non-overlapping, i.e., if $R_{\js}\cap R_{\js'}=\emptyset$ for any
$\js,\js'\in R_{\js}$. If a set of jobs $J'$ is top-drawn, then
it clearly forms a feasible round in \rufp. 
However, not every feasible round of \rufp is top-drawn. Nevertheless, we look for a solution to \rufp in which the
jobs in each round are top-drawn. The following lemma implies that
this costs only a factor of 8 in our approximation ratio.

\begin{lemma}[\cite{BonsmaSW11}] \label{lemma:itspacking}  Let $J'$ 
be the set of jobs packed in  a feasible round for a given instance of \rufp. Then $J'$ can
be partitioned into at most 8 sets such that each of them is top-drawn.\end{lemma}

Let $\R_{\mathrm{large}}:=\{R_{\js}|\js\in J_{\mathrm{large}}\}$
denote the rectangles corresponding to the large jobs and let $\omega_{\mathrm{large}}$ be 
their clique number, i.e., the size of the largest set $\R'\subseteq\R_{\mathrm{large}}$
such that all rectangles in $\R'$ pairwise overlap. It is known that
for such a set of rectangles $\R'$ there must be a point in which all rectangles
in $\R'$ overlap\footnote{\ari{This is a simple consequence of Helly's theorem. See \cite{helly22} for details.}}. Note that we need at least $\omega_{\mathrm{large}}$
rounds since we seek a solution with only top-drawn jobs in
each round. Our strategy is to invoke the following theorem on $\R_{\mathrm{large}}$. 

\begin{theorem}[\cite{parinbar}] \label{thm:parinyathm}  Given a
set of rectangles $\R'$ with clique number $\omega$. In polynomial
time, we can compute a coloring of the rectangles using $O(\omega\log\omega)$
colors such that no two rectangles of the same color intersect. \end{theorem}

Thus, if $\omega_{\mathrm{large}}=O(\log n)$ then we obtain an $O(\log\log n)$-approximation
as desired. However, it might be that $\omega_{\mathrm{large}}$ is
larger. In that case, we partition $\R_{\mathrm{large}}$ into $\omega_{\mathrm{large}}/\log n$
sets, such that each of them has a clique size of $O(\log n)$.
\begin{lemma}
There is a randomized polynomial time algorithm that w.h.p.~computes
a partition $\R_{\mathrm{large}}=\R_{1}\dot{\cup}...\dot{\cup}\R_{\omega_{\mathrm{large}}/\log m}$
such that for each set $\R_{i}$, the corresponding clique size is
at most $O(\log n)$.
\end{lemma}
\arir{removed log m claim, adapted to log n. Please check.}
\begin{proof}
We split the rectangles $\R_{\mathrm{large}}$ uniformly at random
into $\omega/\log n$ sets $\R_{1},\ldots,\R_{\omega/\log n}$. Thus
the expected clique size in each set $\R_{i}$ at any point $p$ under
the profile is at most $\log n$. Using the Chernoff bound, the probability
that the clique size at $p$ is more than $6\log n$ is at most $2^{-6\log n}=1/n^{6}$.
For each vertex $v_{i}$, let $p_{v_{i}}$ denote the point $(v_{i},\min(c_{i-1},c_{i}))$.
We draw a horizontal and vertical line passing through $p_{v_{i}}$
inside the capacity profile. \deb{This divides the region below the capacity
profile into $m^2 \le 4 n^{2}$ rectangular regions. Inside any such region, the clique size is maximized at the top edge of the rectangular region (since the rectangles are top-drawn).} Thus the probability that there exists a point $p$ under the capacity
profile where the clique size is more than $6\log n$ is at most $4n^{2}/n^{6}\le1/n^{3}$.
Hence using union bound, probability that clique size is more than
$6\log n$ at some point in some set $\R_{i}$ is at most $1/n^{2}$.
\end{proof}
We apply Theorem~\ref{thm:parinyathm} to each set $\R_{i}$
separately and thus obtain a coloring with $O(\log n\log\log n)$
colors. Thus, for all sets $\R_{i}$ together we use at most $\frac{\omega_{\mathrm{large}}}{\log n}O(\log n\log\log n)=O(\omega_{\mathrm{large}}\log\log n)$
colors. We pack the jobs from each color class to a separate round
for our solution to \rufp. Due to Lemma~\ref{lemma:itspacking},
we have that $\omega_{\mathrm{large}}$ is  $O(\opt_{UFP})$, which thus yields
an $O(\log\log n)$-approximation for \rufp, together with Theorem~\ref{thm:Elbassioni-small}. 

\begin{theorem} There exists a randomized $O(\log\log n)$-approximation
algorithm for \rufp\ for general edge capacities. \end{theorem}

%Since $m\le 2n-1$, this also yields an $O(\log \log n)$-approximate algorithm.

In order to obtain an algorithm for \rsap, we invoke the following
lemma due to \cite{MomkeW15} to each round of the computed solution
to \rufp.
\begin{lemma}[\cite{MomkeW15}]
\label{lem:UFP2SAP}Let $J'$ be the set of jobs packed in a feasible round for a given instance
of \rufp. Then in polynomial time we can partition $J'$ into  $O(1)$ sets and compute a height $h_{\js}$ for each job $\js\in J'$
such that each set yields a feasible round of \rsap.
\end{lemma}

This yields a solution to \rsap~with only $O(OPT_{SAP}\log\log n)$
rounds.

\begin{theorem} There exists a randomized $O(\log\log n)$-approximation
algorithm for \rsap\ for general edge capacities.\end{theorem}

\begin{comment}
\begin{lemma} \label{lem:constantforsmalljobs-1} There exist $O(1)$-approximation
algorithms for \rufp\ and \rsap\ for packing jobs in $S$. \end{lemma} 
\begin{proof}
For \rufp, Elbassioni et al. \cite{ElbassioniGGKN12} gave a 16-approximation
algorithm for packing jobs in $S$. For \rsap, our algorithm in \Cref{sec:generalRoundSap}
gives an asymptiotic $(16+\eps)$-approximation algorithm. 
\end{proof}
\begin{lemma} \label{lem:loglognforlargejobs-1} There exists a randomized
$O(\log\log m)$-approximation for \rufp\ and \rsap\ for packing
jobs in $T$. \end{lemma} 
\begin{proof}
Let $OPT'$ denote the optimal number of rounds required to pack all
jobs in $T$ as top-drawn sets. Then from \Cref{thm:itspacking},
we have $OPT'\le8OPT_{RU}\le8OPT_{RS}$.

We draw all the jobs as rectangles in a top-drawn fashion inside one
bin, i.e each job $\js$ is placed in the region $R_{\js}$ (thus
the top edge of the rectangle touches the capacity profile over its
bottleneck edge). Let $\omega$ denote the clique size, i.e the maximum
number of rectangles that overlap at any point. Thus $\omega\le OPT'$.

If $\omega<\log n$, we apply \Cref{thm:parinyathm} to get a coloring
using at most $\omega O(\log\log n)$ colors. Otherwise 

We apply \Cref{thm:parinyathm} to each set $J_{i}$. Thus with
probability at least $1-\frac{1}{n^{2}}$, each set can be colored
using $O(\log n\log\log n)$ colors. Thus total number of colors used
is $\frac{\omega}{\log n}O(\log n\log\log n)\le\omega O(\log\log n)$.
We pack all rectangles having the same color inside one bin. Thus
the total number of bins used is at most $O(\log\log n)OPT'\le O(\log\log n)OPT_{RU}\le O(\log\log n)OPT_{RS}$
(since $OPT'\le8OPT_{RU}\le8OPT_{RS}$). 
\end{proof}
Note that the above algorithm works even if $n$ is replaced by $m$
everywhere. With probability at least $1-\frac{1}{m^{2}}$, we would
get a packing using at most $O(\log\log m)OPT_{RS}$ bins. Combining
\Cref{lem:constantforsmalljobs} and \Cref{lem:loglognforlargejobs},
we have the following theorem.

\begin{theorem} There exists a randomized $\min(O(\log\log n,\log\log m))$-approximation
algorithm for \rufp\ and \rsap\ without NBA. \end{theorem}
\end{comment}



==> improvements.tex <==
\section{Improvements}
\subsection{\rufp\ with NBA}
We assume that $c_{\min}=1$ and the demand of each job is at most 1. Let $S$ be the set of jobs whose demands are $\le 1/2$ and $T=J\setminus S$. Consider any job $\js\in S$ and let $i$ be such that $\frac{1}{2^{i+1}}< d_{\js} \le \frac{1}{2^i}$. We round up the demand of $\js$ to $\frac{1}{2^i}$. Let $J_i$ denote the set of jobs whose demands after rounding is $\frac{1}{2^i}$ and let $n_{e,i}=|\{\js \in J_i \mid e\in P_{\js}\}|$. Let $U_{e,i}=\{e\in E\mid n_{e,i}<2r\}$ and $J'_i = \{\js \in J_i\mid \exists e\in U_{e,i} \text{ such that } e\in P_{\js}\}$. Let $J''_i = J\setminus J'_i$. Let $n'_{e,i}=|\{\js \in J'_i \mid e\in P_{\js}\}|$ and $n''_{e,i}=|\{\js \in J''_i \mid e\in P_{\js}\}|$. Clearly $n'_{e,i} < 4r$.

\begin{lemma}
The jobs in $S$ can be packed into at most $8r$ bins.
\end{lemma}
\begin{proof}
For packing jobs in $\bigcup\limits_i J''_i$, we introduce a set $\Ss$ of $4r$ bins. Inside each of these bins, we create a profile $I_i$, such that the capacity of edge $e$ in $I_i$ equals $\frac{1}{2^i} \lfloor \frac{n_{e,i}}{2r} \rfloor$. Jobs in $J''_i$ shall be packed under these profiles $I_i$. The congestion of any edge having non-zero capacity in $I_i$ is $\frac{\frac{1}{2^i}n''_{e,i}}{\frac{1}{2^i}\lfloor \frac{n_{e,i}}{2r} \rfloor} \le \frac{\frac{n_{e,i}}{2r}}{\lfloor \frac{n_{e,i}}{2r} \rfloor}\cdot 2r \le 4r$. Also since each job in $J''_i$ has demand equal to $\frac{1}{2^i}$, the capacity of each edge in $I_i$ is an integral multiple of the demand. Thus using \Cref{theorem:nomikostheorem}, jobs in $J''_i$ can be packed under the $4r$ profiles $I_i$. The load on edge $e$ inside any bin is at most $\sum\limits_i \frac{1}{2^i} \lfloor \frac{n_{e,i}}{2r} \rfloor \le \sum\limits_i \frac{1}{2^{i+1}}\frac{n_{e,i}}{r} \le \frac{1}{r} \sum\limits_{\js \colon e\in P_j} d_j \le c_e$. Thus this is a valid packing.

For packing jobs in $\bigcup\limits_i J'_i$, we introduce a set $\Ts$ of $4r$ bins. For each $i$, we consider the jobs in $J'_i$ in non-decreasing order of their left endpoints and assign a job to the first bin in $\Ts$ where it does not overlap with any job from $J'_i$ that have been assigned till now. Since $n'_{e,i}\le 4r$, such an assignment is always possible. Thus over any edge $e$ inside any bin of $\Ts$, at most 1 job from each $J_i$ can be present. Thus the load on edge $e$ is at most $\sum\limits_i \frac{1}{2^i} \le 1 \le c_e$ and this is a valid packing. 

Hence all jobs in $S$ can be packed into $8r$ bins.
\end{proof}

\begin{lemma}
The jobs in $T$ can be packed into $4r$ bins.
\end{lemma}
\begin{proof}
We round up the demand of each job in $T$ to $1$ and round down the capacity of each edge to the nearest integer. Thus the congestion increases by at most a factor of 4. Hence by applying \Cref{theorem:nomikostheorem}, jobs in $T$ can be packed into at most $4r$ bins.
\end{proof}

Thus we get a packing of $J$ using at most $12r$ bins.

\subsection{Without NBA}
A set of jobs is said to form a top-drawn set if each job is placed in the rectangular region $R_{\js}=(s_{\js},b_{\js}-d_{\js})\times (t_{\js},b_{\js})$ under the capacity profile such that $R_{\js}\cap R_{\js'}=\phi$ for any two jobs $\js$ and $\js'$. We use the following results.

\begin{theorem}
\label{thm:itspacking}
\cite{BonsmaSW11} Let $F$ be a feasible UFPP packing of $1/k$-large jobs inside 1 bin. Then $F$ can be split into $2k$ top-drawn sets.
\end{theorem}

\begin{theorem}
\label{thm:parinyathm}
\cite{parinbar} Given a set of rectangles with clique number $\omega$, a coloring of the rectangles using $O(\omega \log \omega)$ colors such that no two rectangles of the same color intersect, can be computed in polynomial time.
\end{theorem}

Let $S=\{\js \in J\mid d_{\js}\le \frac{1}{4}b_{\js}\}$ and $T=J\setminus S$.

\begin{lemma}
\label{lem:constantforsmalljobs}
There exist $O(1)$-approximation algorithms for \rufp\ and \rsap\ for packing jobs in $S$.
\end{lemma}
\begin{proof}
For \rufp, Elbassioni et al. \cite{ElbassioniGGKN12} gave a 16-approximation algorithm for packing jobs in $S$. For \rsap, our algorithm in \Cref{sec:generalRoundSap} gives an asymptiotic $(16+\eps)$-approximation algorithm.
\end{proof}



\begin{lemma}
\label{lem:loglognforlargejobs}
There exists a randomized $O(\log \log n)$-approximation for \rufp\ and \rsap\ for packing jobs in $T$.
\end{lemma}
\begin{proof}
Let $OPT'$ denote the optimal number of rounds required to pack all jobs in $T$ as top-drawn sets. Then from \Cref{thm:itspacking}, we have $OPT' \le 8 OPT_{RU} \le 8 OPT_{RS}$. 

We draw all the jobs as rectangles in a top-drawn fashion inside one bin, i.e each job $\js$ is placed in the region $R_{\js}$ (thus the top edge of the rectangle touches the capacity profile over its bottleneck edge). Let $\omega$ denote the clique size, i.e the maximum number of rectangles that overlap at any point. Thus $\omega \le OPT'$. 

If $\omega < \log n$, we apply \Cref{thm:parinyathm} to get a coloring using at most $\omega O(\log \log n)$ colors. Otherwise we split the set of jobs uniformly at random into $\omega/\log n$ sets $J_1,\ldots,J_{\omega/\log n}$. Thus the expected clique size in each set $J_i$ at any point $p$ under the profile is $\le \log n$. Using Chernoff bound, the probability that the clique size at $p$ is more than $6\log n$ is at most $2^{-6\log n}=1/n^6$. For each vertex $v_i$, let $p_{v_i}$ denote the point $(v_i,\min (c_{i-1},c_i))$. We draw a horizontal and vertical line passing through $p_{v_i}$ inside the capacity profile. This divides the region below the capacity profile into $m^2\le 4n^2$ regions. Clearly inside each region, the clique size must be the same, since all rectangles are top-drawn. Thus the probability that there exists a point $p$ under the capacity profile where the clique size is more than $6\log n$ is at most $4n^2/n^6 \le 1/n^3$. Hence using union bound, probability that clique size is more than $6\log n$ at some point in some set $J_i$ is at most $1/n^2$. 

We apply \Cref{thm:parinyathm} to each set $J_i$. Thus with probability at least $1-\frac{1}{n^2}$, each set can be colored using $O(\log n\log \log n)$ colors. Thus total number of colors used is $\frac{\omega}{\log n}O(\log n\log \log n) \le \omega O(\log \log n)$. We pack all rectangles having the same color inside one bin. Thus the total number of bins used is at most $O(\log\log n)OPT'\le O(\log \log n)OPT_{RU}\le O(\log\log n)OPT_{RS}$ (since $OPT'\le 8OPT_{RU}\le 8OPT_{RS}$). 
\end{proof}

Note that the above algorithm works even if $n$ is replaced by $m$ everywhere. With probability at least $1-\frac{1}{m^2}$, we would get a packing using at most $O(\log\log m)OPT_{RS}$ bins. Combining \Cref{lem:constantforsmalljobs} and \Cref{lem:loglognforlargejobs}, we have the following theorem.

\begin{theorem}
There exists a randomized $\min (O(\log \log n, \log \log m))$-approximation algorithm for \rufp\ and \rsap\ without NBA.
\end{theorem}


\subsection{An $O(\log \log \frac{1}{\delta})$-approximation without NBA with $1+\delta$ resource augmentation}
We divide the jobs based on their bottleneck capacities: let $J_i$ be the set of jobs with bottleneck capacity in the range $(\frac{1}{\delta^i},\frac{1}{\delta^{i+1}})$, $i\ge 0$. Suppose we have a valid packing of $J_i$ using $x_i$ rounds. Using resource augmentation, we can combine the packings of $J_i$ in the following way. 

\begin{lemma}
Let $\Rs^i$ be a round containing only jobs from the set $J_i$. Then all jobs inside the rounds $\Rs^0,\Rs^2,\ldots$ can be packed inside one round $\Rs$ of the resource-augmented profile.
\end{lemma}
\begin{proof}
Suppose we are allowed a resource augmentation of $1+\gamma$, for some $\gamma > 0$. Now since the bottleneck capacity of any job in $J_i$ is at least $\frac{1}{\delta^i}$, on resource augmentation, the capacity of any such edge would increase by at least $\frac{\gamma}{\delta^i}$. Given the packing inside round $\Rs^i$, we shift up the position of each job by $\frac{\gamma}{\delta^i}$ and place it in $\Rs$.

Now the jobs from $J_{i-2}$ do not go above $\frac{1}{\delta^{i-1}}+\frac{\gamma}{\delta^{i-2}}$. We choose $\gamma$ such that $\frac{\gamma}{\delta^i} \ge \frac{1}{\delta^{i-1}}+\frac{\gamma}{\delta^{i-2}}$, from which we get $\gamma = \frac{\delta}{1-\delta^2}=O(\delta)$.
\end{proof}

Hence the total number of rounds used is $\max (x_0,x_2,\ldots) + \max (x_1,x_3,\ldots)$. We now show that each $x_i$ is at most $O(\log \log \frac{1}{\delta})OPT$. By scaling, we may assume all edges have capacity in the range $(1,1/\delta)$. For 1/4-small jobs, we already have 16-approximation algorithms for \rsap\ and \rufp. For 1/4-large jobs, Jahanjou et al. \cite{JahanjouKR17} gave an $O(\log \log c_{\text{max}})$-approximation algorithm. Since $c_{\text{max}}\le 1/\delta$ for our case, this yields an $O(\log \log \frac{1}{\delta})$-approximation algorithm. Hence we have the following result.






\iffalse
We now show that each $x_i$ is at most $O(\frac{1}{\delta})OPT$. By scaling, we may assume all edges have capacity in the range $(1,1/\delta)$. For 1/4-small jobs, we already have 16-approximation algorithms for \rsap\ and \rufp. So consider the 1/4-large jobs. We sort the jobs in $J_i$ in non-decreasing order of their left endpoints and apply the FF interval coloring algorithm. Hence in each round, at most 1 job is placed over each edge. 

\begin{lemma}
$x_i \le \frac{4}{\delta}OPT$.
\end{lemma}
\begin{proof}
Since the jobs are 1/4-large and the edge capacity is at most $1/\delta$, there are at most $4/\delta$ jobs over any edge inside any round of the optimal packing. Thus again by FF interval coloring, these can be split into at most $\frac{4}{\delta}$ sets such that each edge has at most 1 job over it. Thus the number of rounds used by our algorithm to pack $J_i$ is at most $\frac{4}{\delta}OPT$.
\end{proof}
\fi

\begin{corollary}
There exists an $O(\log \log \frac{1}{\delta})$-approximation algorithm for \rsap\ and \rufp\ without NBA when the edge capacities can be augmented by a factor $1+\delta$.
\end{corollary}




==> uniform_new.tex <==
\section{Improved algorithms for uniform capacity case}
We repeatedly use the following results on DSA.

\begin{theorem}
\cite{BuchsbaumKKRT03}
\label{thm:dsamaintheorem}
If $d_{\max}\le \delta^7 L$, there exists a feasible solution to DSA with makespan at most $(1+\alpha \delta)L$, for some constant $\alpha > 0$.
\end{theorem}

\begin{theorem}
\cite{Gergov99}
\label{thm:dsagergovthm}
Given a set of jobs with load $L$, there exists a solution of DSA with makespan at most $3L$.
\end{theorem}

Now we divide our algorithm into 2 cases depending on the values of $d_{\max}$ and $L$.

\subsection{$d_{\max}\le \epsilon^7 L$}
We further divide into two subcases depending on the value of $r$.

\subsubsection{$r > \frac{1}{2\alpha \epsilon}$}
\label{sec:largecongestion}
We first apply \Cref{thm:dsamaintheorem} to $J$ to obtain a DSA packing with makespan $\zeta \le (1+\alpha \epsilon)L$. Now we open a set of rounds $\Gamma_1$ which contains a round for each integer $i$ with $0\le i \le \lfloor \zeta/c^{*}\rfloor$ and this round contains all jobs lying between $\ell_{ic^{*}}$ and $\ell_{(i+1)c^{*}}$. Thus $|\Gamma_1| \le \left \lceil \frac{(1+\alpha \epsilon)L}{c^*}\right \rceil \le (1+\alpha \epsilon)r + 1 \le (1+3\alpha \epsilon)r$. 

Now we define a set of rounds $\Gamma_2$ as follows. For each integer $i$ with $1\le i \le \lfloor \zeta/c^{*}\rfloor$, $\Gamma_2$ has a round containing all jobs sliced by $\ell_{ic^*}$. Thus $|\Gamma_2|\le \lfloor \frac{(1+\alpha \epsilon)L}{c^*}\rfloor \le (1+\alpha \epsilon)r$. Thus the total number of rounds used is at most $(2+O(\epsilon))r$.

\begin{theorem}
If $d_{\max}\le \epsilon^7 L$ and $r > \frac{1}{2\alpha \epsilon}$, there exists a packing of $J$ using $(2+O(\epsilon))r$ rounds.
\end{theorem}

\subsubsection{$r \le \frac{1}{2\alpha \epsilon}$}
Applying \Cref{thm:dsamaintheorem} to $J$, we get a DSA packing of makespan $\zeta \le (1+\alpha \epsilon)L$. Thus $\zeta - L \le \alpha \epsilon L \le c^*/2$. As in \Cref{sec:largecongestion}, we open a set of $r+1$ rounds, where the $i^{\text{th}}$ round contains all jobs lying between $\ell_{ic^{*}}$ and $\ell_{(i+1)c^{*}}$. Now since $\zeta - L \le c^*/2$, the $(r+1)^{\text{th}}$ round is filled to a capacity of at most $c^*/2$. Now the total load of the jobs sliced by the set of slicing lines $(\ell_{ic^*})_{1\le i \le r}$ is at most $r \cdot \epsilon^7 L$. Thus by applying \Cref{thm:dsagergovthm} to these jobs, we get a DSA packing of makespan at most $3r\cdot \epsilon^7 L \le 3\cdot \frac{1}{2\alpha \epsilon}\cdot \epsilon^7 \frac{c^*}{2\alpha \epsilon} \le \epsilon c^*$, for sufficiently small $\epsilon$. Hence all these jobs can be packed into the $(r+1)^{\text{th}}$ round, which will be filled up to at most $(\frac{1}{2}+\epsilon)c^*$. Hence we get a packing of $J$ using $r+1$ rounds.

\begin{theorem}
If $d_{\max}\le \epsilon^7 L$ and $r \le \frac{1}{2\alpha \epsilon}$, there exists a packing of $J$ using $r+1$ rounds.
\end{theorem}


\subsection{$d_{\max} > \epsilon^7 L$}
In this case, we have $c^* \ge d_{\max} > \epsilon^7 L$. Thus $r = \left \lceil L/c^* \right \rceil \le 1/\epsilon^7 $. We define $J_{\text{small}} := \{\js | d_{\js}\le \epsilon^{56}L \}$ and $J_{\text{large}} := \{\js | d_{\js}> \epsilon^{56}L \}$. For jobs in $J_{\text{large}}$, the optimal packing can be found in polynomial time using DP.

Applying \Cref{thm:dsamaintheorem} to $J_{\text{small}}$, we get a packing of makespan $\zeta \le (1+\alpha \epsilon^8)L$. Thus $\zeta - L \le \alpha \epsilon^8 L \le \alpha
\epsilon c^*$. As before, we open a set of $r+1$ rounds, where the $i^{\text{th}}$ round contains all jobs lying between $\ell_{ic^{*}}$ and $\ell_{(i+1)c^{*}}$. The $(r+1)^{\text{th}}$ round will be filled up to a capacity of at most $\alpha
\epsilon c^*$. Again the total load of the jobs sliced by the set of slicing lines $(\ell_{ic^*})_{1\le i \le r}$ is at most $r \cdot \epsilon^{56}L$. Thus \Cref{thm:dsagergovthm} would give a DSA packing of makespan at most $3r\cdot \epsilon^{56}L\le 3\cdot 1/\epsilon^7 \cdot \epsilon^{56}\cdot \frac{c^*}{\epsilon^7}\le \epsilon c^*$, for sufficiently small $\epsilon$. Thus all these jobs can be packed into the $(r+1)^{\text{th}}$ round. Hence we get a packing of $J_{\text{small}}$ using $r+1$ rounds.

Together with the optimal packing of $J_{\text{large}}$, we get a packing of $J$ using at most $2\cdot OPT +1$ rounds. 

\begin{theorem}
If $d_{\max} > \epsilon^7 L$, there exists a packing of $J$ using at most $2\cdot OPT + 1$ rounds.
\end{theorem}


